BFT Protocol Forensics

Byzantine fault-tolerant (BFT) protocols allow a group of replicas to come to a consensus even when some of the replicas are Byzantine faulty. There exist multiple BFT protocols to securely tolerate an optimal number of faults $t$ under different network settings. However, if the number of faults $f$ exceeds $t$ then security could be violated. In this paper we mathematically formalize the study of forensic support of BFT protocols: we aim to identify (with cryptographic integrity) as many of the malicious replicas as possible and in as a distributed manner as possible. Our main result is that forensic support of BFT protocols depends heavily on minor implementation details that do not affect the protocol's security or complexity. Focusing on popular BFT protocols (PBFT, HotStuff, Algorand) we exactly characterize their forensic support, showing that there exist minor variants of each protocol for which the forensic supports vary widely. We show strong forensic support capability of LibraBFT, the consensus protocol of Diem cryptocurrency; our lightweight forensic module implemented on a Diem client is open-sourced and is under active consideration for deployment in Diem. Finally, we show that all secure BFT protocols designed for $2t+1$ replicas communicating over a synchronous network forensic support are inherently nonexistent; this impossibility result holds for all BFT protocols and even if one has access to the states of all replicas (including Byzantine ones).

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> [CCS21] BFT Protocol Forensics/0_abstract.tex <==
\begin{abstract}
Byzantine fault-tolerant (BFT) protocols allow a group of replicas to come to consensus even when some of the replicas are Byzantine faulty. There exist multiple BFT protocols to securely tolerate an optimal number of faults $t$ under different network settings. However, if the number of faults $f$ exceeds $t$ then security could be violated. In this paper we  mathematically formalize the study of  {\em forensic support} of BFT protocols: we aim to identify (with cryptographic integrity) as many of the malicious replicas as possible and in as distributed manner as possible. Our main result is that forensic support of BFT protocols depends heavily on minor implementation details that do not affect the protocol's security or complexity. Focusing on popular BFT protocols (PBFT, HotStuff, Algorand) we exactly characterize their forensic support, showing  that there exist minor variants of each protocol for which the forensic supports vary widely. %This result brings to focus a heretofore unexplored dimension, forensic support,  to  secure BFT protocol designs; this is in conjunction with the traditional performance metrics of latency and communication complexity. 
We show strong forensic support capability of LibraBFT, the consensus protocol of Diem cryptocurrency; our lightweight forensic module implemented on a Diem client is open-sourced  \cite{diemopensource} and is under active consideration for deployment in Diem.  Finally, we show that all secure BFT protocols designed for $2t+1$ replicas communicating over a synchronous network forensic support is inherently  nonexistent; this impossibility result holds for all BFT protocols and even if one has access to  the states of all replicas (including Byzantine ones). 
\end{abstract}

\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002978.10003006.10003013</concept_id>
<concept_desc>Security and privacy~Distributed systems security</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010520.10010575</concept_id>
<concept_desc>Computer systems organization~Dependable and fault-tolerant systems and networks</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Security and privacy~Distributed systems security}
\ccsdesc[500]{Computer systems organization~Dependable and fault-tolerant systems and networks}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{forensics; BFT protocols; blockchains}






\ignore{The one without comment/cite/etc, ready for copy and paste:
Byzantine fault-tolerant (BFT) protocols allow a group of replicas to come to consensus even when some of the replicas are Byzantine faulty. There exist multiple BFT protocols to securely tolerate an optimal number of faults $t$ under different network settings. However, if the number of faults $f$ exceeds $t$ then security could be violated. In this paper we  mathematically formalize the study of  {\em forensic support} of BFT protocols: we aim to identify (with cryptographic integrity) as many of the malicious replicas as possible and in as distributed manner as possible. Our main result is that forensic support of BFT protocols depends heavily on minor implementation details that do not affect the protocol's security or complexity. Focusing on popular BFT protocols (PBFT, HotStuff, Algorand) we exactly characterize their forensic support, showing that there exist minor variants of each protocol for which the forensic supports vary widely. We show strong forensic support capability of LibraBFT, the consensus protocol of Diem cryptocurrency; our lightweight forensic module implemented on a Diem client is open-sourced and is under active consideration for deployment in Diem. Finally, we show that all secure BFT protocols designed for $2t+1$ replicas communicating over a synchronous network forensic support is inherently nonexistent; this impossibility result holds for all BFT protocols and even if one has access to  the states of all replicas (including Byzantine ones). 
}

==> [CCS21] BFT Protocol Forensics/1_introduction.tex <==
\section{Introduction}

Byzantine Fault Tolerant (BFT) protocols, guaranteeing distributed consensus among parties that follow the protocol, are a corner stone of distributed system theory. In the relatively recent context of blockchains, BFT protocols have received renewed attention; new and efficient (state machine replication (SMR)) BFT protocols specifically designed for  blockchains  have been constructed (e.g., Algorand \cite{gilad2017algorand}, HotStuff \cite{yin2019hotstuff}, Streamlet \cite{chan2020streamlet}). The core theoretical security guarantee is that as long as a certain fraction of nodes are ``honest'', i.e., they follow the protocol, then these nodes achieve consensus with respect to (a time evolving) state machine regardless of the Byzantine actions of the remaining malicious nodes. When the malicious nodes are sufficiently numerous, e.g., strictly more than a $1/3$ fraction of nodes in a partially synchronous network, they can ``break security'', i.e., band together to create different views at the honest participants. 

In this paper, we are focused on ``the day after'' \cite{thedayafter}: events {\em after} malicious replicas have successfully mounted a security breach. Specifically, we focus on identifying which of the participating replicas acted maliciously; we refer to this action as ``forensics''. Successful BFT protocol forensics meets two goals:
\begin{itemize}
    \item identify as many of the nodes that acted maliciously as possible with an irrefutable cryptographic proof of culpability; 
    \item identification is conducted as distributedly as possible, e.g., by the individual nodes themselves, with no/limited communication between each other after the security breach.
\end{itemize}


\noindent {\bf Main contributions.} Our central finding is that the forensic possibilities crucially depend on minor implementation details of BFT protocols; the details themselves do not affect protocol  security or performance (latency and communication complexity); we demonstrate our findings  in the context of several popular BFT protocols for  Byzantine Agreement (BA). We present our  findings in the context of a mathematical  and systematic formulation of the  ``forensic support'' of BFT protocols. The forensic support of any BFT protocol is parameterized as a triplet  $(m,k,d)$, that represents the aforementioned  goals of forensic  analysis. The triplet $(m,k,d)$ along with traditional BFT protocol parameters of $(n,t,f)$ is summarized in Table~\ref{tab:notations}. We emphasize that each of the protocol variants is safe and live when $f \le t$ (here $n= 3t+1$  for all the protocols considered) but their forensic supports are quite different. % \sk{Highlight that all protocols are safe and live under the appropriate settings but their forensic support is quite different. Maybe by adding a security threshold column before forensic support? }

\begin{table}[t]
    \centering
    \begin{tabularx}{\columnwidth}{cX} \toprule
        Symbol & \makecell{Interpretation}\\
        \toprule
        $n$ & total number of replicas\\
        \midrule
        $t$ & maximum number of faults for obtaining agreement and termination \\
        \midrule
        $f$ & actual number of faults\\
        \midrule
        $m$ & maximum number of Byzantine replicas under which forensic support can be provided\\
        \midrule
        $k$ & the number of different honest replicas'  transcripts needed  to guarantee a proof of culpability \\
        \midrule
       $d$ & the number of Byzantine replicas that can be held culpable in case of an agreement violation\\\bottomrule
    \end{tabularx}
     \caption{Summary of notations.}
    \label{tab:notations}
\end{table}


% \begin{table}[]
% \centering
% \begin{tabular}{c|c|c|c|c}
% \toprule
% \multirow{2}{*}{\textbf{Protocols}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Forensic\\ Support\end{tabular}}} & \multicolumn{3}{c}{\textbf{Parameters}} \\ \cline{3-5} 
%                                     &                                                                                      & $m$       & $k$              & $d$       \\ \toprule
% PBFT-PK                             &                                                                                     &       &               &      \\ 
% \hsa                                 & Strong                                                                                    & $2t$      & $1$              & $t+1$     \\ 
% VABA                                &                                                                                     &       &               &      \\ \toprule
% \hsb                                 & Medium                                                                                    & $2t$      & $t+f+1$     & $t+1$     \\ \toprule
% PBFT-MAC                           &                                                                                     &         &               &         \\ 


% \hsc                                 & None                                                                                    & $t+1$         & $n$                &  0        \\ 


% Algorand                            &                                                                                     &         &                 &         \\ \bottomrule
% \end{tabular}
% \caption{Summary of Results.}
% \label{tab:results}
% \end{table}

\begin{table}[]
\centering
\begin{tabular}{c|c|ccc}
\toprule
\multirow{2}{*}{\textbf{Protocols}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Forensic\\ Support\end{tabular}}} & \multicolumn{3}{c}{\textbf{Parameters}} \\ \cline{3-5} 
                                    &                                                                                      & $m$       & $k$              & $d$       \\ \toprule
PBFT-PK                             &                                                                                     &       &               &      \\ 
\hsa                                 & Strong                                                                                    & $2t$      & $1$              & $t+1$     \\ 
VABA                                &                                                                                     &       &               &      \\ \midrule
\hsb                                 & Medium                                                                                    & $2t$      & $t+1$     & $t+1$     \\ \midrule
PBFT-MAC                           &                                                                                     &         &              &    $0$     \\ 


\hsc                                 & None                                                                                    & $t+1$         &          $2t$      &  $ 1$        \\ 


Algorand                            &                                                                                     &         &               &  $ 0$       \\ \bottomrule
\end{tabular}
\caption{Summary of results; the forensic support values of $d$ are the largest possible and $n=3t+1$ here.}
\label{tab:results}
\end{table}




Security attacks on BFT protocols can be far more subtle than simply double voting or overt equivocation (when the culpable replicas are readily identified), and the forensic analysis is correspondingly subtle. This paper brings to fore a new dimension for secure BFT protocol design  beyond performance (low latency and low communication complexity): forensic support capabilities. 

 We analyze the forensic support of classical and state-of-the-art BFT protocols for Byzantine Agreement. Our main findings, all in the settings of safety violation (agreement violation), are the following, summarized in Table~\ref{tab:results}. 
 \begin{itemize}[leftmargin=*]
     \item {\bf Parameter $\mathbf{d}$.} We show that %\kartik{when there is a safety violation} 
     the number of culpable replicas $d$ that can be identified is either 0 %\peiyao{in a special case, we can identify the malicious leader}%\kartik{Peiyao: verify, can we not even identify a leader?} 
     %\pramod{Peiyao and I discussed the point regarding identifying at least leader: the point of culpability of at least 1 is meant to cover all possible instances. It could be possible to identify 1 bad actor in some attaacks, but we are stating worst case guarantees}
     or as large as $t+1$. In other words,  
     %\kartik{for the variants we analyzed,} \pramod{we prefaced this list by saying that analysis is for specific classical and state of the art BFT protocols}
     if at least one replica can be identified then we can also identify the largest possible number,  $t+1$ replicas; the only exception is for \hsc,  where in a successful safety attack, we can identity the culpability of one malicious replica.
     
     
     \item {\bf Parameter $\mathbf{m}$.} We show that the maximum number of Byzantine replicas $m$ allowed for nontrivial forensic support (i.e., $d >0$) cannot be more than $2t$.  %\peiyao{do we need to exiplicitly say what is nontrivial} %\kartik{with chained hotstuff, it can be higher.} \pramod{Chained HotStuff is not part of BA, so we are taking it out of this list and out of Table 2.} 
     Furthermore, any forensic support  feasible with $m$ is also feasible with $m$ being its largest value $2t$, i.e., if $(m,k,d)$ forensic support is feasible, then $(2t, k,  d)$ is also feasible.% \peiyao{still have this question: $(t+1,t+1,1)$ is feasible for \hsc, but $(2t, t+1, 1)$ is not feasible. For $d=t+1$, the above claim is correct}
 %    \gerui{can we say any nontrivial forensic support with $d=t+1$}
     %\kartik{did not understand this statement} \pramod{added an English sentence to go along}
     \item {\bf Parameter $\mathbf{k}$.} Clearly at least one replica's transcript is needed for forensic analysis, so $k=1$ is the least possible value. This suffices for several of the BFT protocol variants. However for \hsb, $k$ needs to be at least  %\kartik{typo?} \pramod{yes, thanks for catching this}
     $t+1$ for any nontrivial forensic analysis. %\peiyao{should we say at most as much as $t+1$?}\gerui{I agree at most.}%\gerui{This is our new definition of $k=$N/A in impossible result}\gerui{For PBFT-MAC, \hsc, and Algorand,  it is impossible to detect $d$ culpable replicas, thus $k$ is not applicable.} \pramod{N/A doesnt make sense for any reviewer. I understand why you are doing this, but I am removing it.}
     
   
     \item \textbf{Strong forensic support.} The first three items above imply that the strongest possible forensic support is $(2t, 1, t+1)$. Further, the BFT protocols in Table~\ref{tab:results} that achieve any nontrivial forensic support automatically achieve the strongest possible forensics (the only exception is \hsb, for which the forensic support we identified is the best possible).
     
     \item {\bf Impossibility.} 
     For certain variants of BFT protocols (PBFT-MAC, \hsc, and Algorand), even with transcripts from all honest replicas, non-trivial forensics is simply not possible, i.e., $d=0$  even if $m$ is set to its smallest and $k$  set to its largest possible values ($t+1$ and $2t$ respectively);  again, \hsc allows the culpability of a single  malicious replica. %\kartik{typo?} %variants.  e.g.,  conflicting proofs in \hsc and silent (covert) attack in Algorand. 
     
     \item {\bf Practical impact.} Forensic support is of immediate interest to practical blockchain systems; we conduct a forensic support analysis of LibraBFT, the consensus protocol in the new cryptocurrency {\sf Diem}, and show  in-built strong forensic support. We have implemented the corresponding forensic analysis algorithm inside of a {\sf Diem} client and built an associated forensics dashboard; our reference implementation is available open-source \cite{diemopensource} and is under active consideration for deployment in {\sf Diem}.
     
      \item \textbf{BFT with $n=2t+1$.} For a secure BFT protocol operating on a synchronous network, the ideal setting is $n = 2t+1$. For {\em every} such protocol we show that at most one culpable replica can be identified (i.e., $d$ is at most 1) even if we have access to the state of all honest nodes, i.e, $k= t$. % \kartik{typo?}
     
     \end{itemize}
   
   
   \myparagraph{Outline.} We describe our results in the context of related work in \S\ref{sec:related}; to the best of our knowledge, this is the first paper to systematically study BFT protocol forensics. The formal forensic support problem statement and security model is in \S\ref{sec:model}. The forensic support of PBFT, HotStuff and Algorand (and variants) are explored in \S\ref{sec:pbft}, \S\ref{sec:basic-hotstuff}, \S\ref{sec:algorand}, respectively. 
   Our forensic study of LibraBFT and implementation of the corresponding forensic protocol is the focus of \S\ref{sec:impl}. In appendix \S\ref{sec:vaba}, we present the forensic support analysis for VABA, a state-of-the-art  efficient BFT for   asynchronous network conditions.  The impossibility of forensic support for all BFT protocols operating in the classical $n=2t+1$ synchronous network setting is shown in \S\ref{sec:lb}. Our choice of the 5  protocols studied here (PBFT, HotStuff, Algorand, LibraBFT, VABA) is made with the goal of  covering a variety of settings: (a) partially synchronous vs   asynchronous; (b) authenticated vs non-authenticated; (c) player replaceable vs irreplaceable;  (d) chained version vs single-shot version; (e) variants that communicate differing amounts of auxiliary information. Stitching the results across the 5 different protocols into a coherent theory of forensic support of abstract BFT protocols is an exciting direction of future work; this is discussed in \S\ref{sec:conclusion}. 



==> [CCS21] BFT Protocol Forensics/2_related_work.tex <==
\section{Related Work}
\label{sec:related}
\myparagraph{BFT protocols.} %The notion of Byzantine fault tolerance was first proposed in \cite{lamport1982byzantine} as Byzantine General Problem.
PBFT~\cite{castro1999practical,castro2002practical} is the first practical BFT SMR protocol in the partially synchronous setting, with quadratic communication complexity of view change. %Recently, new BFT protocols are pushing the state-of-the-art further. 
HotStuff~\cite{yin2019hotstuff} is the first partially synchronous SMR protocol that enjoys both a linear communication of view change and optimistic responsiveness. Streamlet~\cite{chan2020streamlet} is another SMR protocol known for its simplicity and textbook construction. Asynchronous Byzantine agreement  is solved by \cite{abraham2019asymptotically} with asymptotically optimal communication complexity and round number. Synchronous protocols such as \cite{abraham2019sync,abraham2020optimal} aim at optimal latency.  %Flexible BFT~\cite{malkhi2019flexible} discovers the case where clients have different beliefs in the number of Byzantine replicas and can act to confirm accordingly. \gerui{move flexible bft to next para?} 
Algorand~\cite{gilad2017algorand,chen2019algorand} designs a committee self-selection mechanism, and the Byzantine agreement protocol run by the committee decides the output for all replicas.

%\gerui{I added this paragraph.} \pramod{reads well. good work!}
\myparagraph{Beyond one-third faults.} The seminal work of   \cite{dwork1988consensus} shows that it is impossible to solve BA when the adversary corrupts one-third replicas for partially  synchronous communication (the same bound holds for SMR). In BFT2F~\cite{li2007beyond}, a weaker notion of safety is defined, and a protocol is proposed such that when the adversary corrupts more than one-third replicas, the weaker notion of safety remains secure whereas the original safety might be violated. However, the weaker notion of safety does not protect the system against common attacks, e.g., double-spending attack in distributed payment systems. Flexible BFT~\cite{malkhi2019flexible} considers the case where clients have different beliefs in the number of faulty replicas and can act to confirm accordingly. Its protocol works when the sum of Byzantine faults and alive-but-corrupt faults, a newly defined type of faults, are beyond one-third. Two recent works~\cite{xiang2021strengthened,kane2021highway} propose BFT SMR protocols that can tolerate more than one-third Byzantine faults after some specific optimistic period. The goal of these works is to mask the effects of faults, even when they are beyond one-third, quite  different from the goals of forensic analysis. 

%\gerui{In the follow section also talk breifly about liveness violation and crash fault detectors? As a review pointed out.} \sk{I think we should talk about liveness violation and say that since we impose irrefutable proof, we cannot provide it for liveness violation. Obtaining other forms of proofs should be pointed out in the discussion section. }

\myparagraph{Distributed system forensics.} Accountability has been discussed in seminal works~\cite{haeberlen2007peerreview,haeberlen2009fault} for distributed systems in general. In the lens of BFT consensus protocols,  accountability is defined as the ability for a replica to prove the culpability of a certain number of Byzantine replicas in \cite{civit2019polygraph}. Polygraph, a new BFT protocol with high communication complexity $O(n^4)$, is shown to attain this property in \cite{civit2019polygraph}. Reference  \cite{ranchal2020blockchain} extends Polygraph to an SMR protocol, and devises a finality layer to ``merge'' the disagreement. %and finalize to an agreement.
Finality and accountability are also discussed in other recent works; examples include Casper~\cite{casper}, GRANDPA~\cite{stewart2020grandpa}, and Ebb-and-flow~\cite{neu2020ebb}. Casper and GRANDPA identify accountability as a central problem and design their consensus protocols around this goal. Ebb-and-flow \cite{neu2020ebb} observes that accountability is immediate in BFT protocols for  safety violations via equivocating votes; however, as pointed out in  \cite{civit2019polygraph}, safety violations can happen during the view change process and this is the step where accountability is far more subtle.     %In these protocols, a BFT finality layer is put on top of an existing SMR (a BFT SMR or a nakamoto blockchain SMR) to ensure its safety. In case any safety violation happens, the protocol outputs the replicas who are accountable.

%\ignore{A subtle difference in the definition of forensic support in our paper  and accountability in \cite{civit2019polygraph} is our external perspective. Forensic support is defined in an external client's perspective, who would execute forensic protocol and return the Byzantine identities. Since a replica can also execute this protocol as a client, forensic support is a more general definition than accountability.}

Reference \cite{civit2019polygraph} argues that PBFT is not accountable and cannot be modified to be accountable without significant change/cost. We point out that the definition of accountability in \cite{civit2019polygraph} is rather narrow:   two replicas with differing views have  to themselves be able to identify culpability of malicious replicas.  On the other hand, in forensic support, we study the number of honest replicas (not necessarily restricted to the specific two replicas which have identified a security breach) that can identify the culpable malicious replicas. Thus the definition of forensic support   is more flexible than the one on accountability. Moreover, our work shows that we can achieve forensic support for protocols such as PBFT and HotStuff without incurring additional communication complexity other than (i) sending a proof of culpability to the client in case of a safety violation, and (ii) the need to use aggregate signatures instead of threshold signatures. %In comparison, Polygraph achieves this with a high communication complexity of $O(n^4)$. 

==> [CCS21] BFT Protocol Forensics/3_model.tex <==


\section{Problem Statement and Model}
\label{sec:model}
The goal of state machine replication (SMR) is to build a replicated service that takes requests from clients and provides the clients with the interface of a single non-faulty server, i.e., each client receives the same totally ordered sequence of values. To achieve this, the replicated service uses multiple servers, also called replicas, some of which may be Byzantine, where a faulty replica can behave arbitrarily. A secure  state machine replication protocol  satisfies two guarantees.
    %
%\peiyao{We may need a more elaborate definition of BFT SMR -- a reviewer's comment}
%\begin{itemize}[leftmargin=*, topsep=0pt]
%    \item[-] 
    \textbf{Safety}: Any two honest replicas cannot output different sequences of values.
 %   \item[-] 
 \textbf{Liveness}: A value sent by a client will eventually be output by honest replicas. % Honest replicas keep outputting non-duplicated valid values.
%\end{itemize}

SMR setting also has external validity, i.e., replicas only output non-duplicated values sent by clients. These values are eventually learned by the clients. Depending on the context, a replica may be interested in learning about outputs too. Hence, whenever we refer to a client for learning purposes, it can be an external entity or a server replica. %We use $n$ to denote the total number of replicas and consider protocols that achieve safety and liveness when the actual number of Byzantine faults $f$ is less than or equal to an upper bound $t$. 
A table of notations is in Table~\ref{tab:notations}.  

In this paper, for simplicity, we focus on the setting of  outputting a {\em single value} instead of a sequence of values. The safety and liveness properties of SMR can then be expressed using the following definition:
\begin{definition}[Validated Byzantine Agreement]
\label{defn:vba}
A protocol solves validated Byzantine agreement among $n$ replicas tolerating a maximum of $t$ faults, if it satisfies the following properties:
\begin{enumerate}[leftmargin=*, topsep=0pt]
    \item[] (Agreement) Any two honest replicas output values $v$ and $v'$, then $v = v'$.
    \item[] (Validity)  If an honest replica outputs $v$, $v$ is an externally valid value, i.e., $v$ is signed by a client. %\kartik{something does not seem right here. How does this get around a simple protocol where we always output $v_\bot$?} \peiyao{I think for single-shot VBA we do not need to consider a sequence of outputs. If all honest nodes receive $v_\bot$, they should output $v_\bot$.(this case is for Algorand)}
    \item[] (Termination) All honest replicas start with externally valid values, and all messages sent among them have been delivered, then honest replicas will output a value.
\end{enumerate}
\end{definition}
% \gerui{Hereafter we use agreement violation and safety violation interchangeably. (We never talk about validity violation since it's trivial to avoid.)}

\myparagraph{Forensic support.} 
Traditionally, consensus protocols provide guarantees only when $f \leq t$. When $f > t$, there can be a safety or liveness violation; this is the setting of study throughout this paper. Our goal is to provide \emph{forensic support} whenever there is a safety violation (or agreement violation) and the number of Byzantine replicas in the system are not too high. In particular, if the actual number of Byzantine faults are bounded by $m$ (for some $m > t$) and there is a safety violation, we can detect $d$ Byzantine replicas using a \emph{forensic protocol}. The protocol takes as input, the transcripts of honest parties, and outputs and \emph{irrefutable} proof of $d$ culprits. With the irrefutable proof, any party (not necessarily in the BFT system) can be convinced of the culprits' identities \emph{without} any assumption on the number of honest replicas. However, if even with transcripts from all honest replicas, no forensic protocol can output such a proof, the consensus protocol has no forensic support (denoted as ``None'' in Table~\ref{tab:results}). Note that when we say a protocol has no forensic support, we are referring to an impossibility w.r.t.\ providing irrefutable proof for $d$ culprits (more precisely, in the context of Definition~\ref{defn:forensic-support}). In a general sense, there are other ways to provide forensics related to hardware, software, and network except for non-repudiation in the protocol.

% \gerui{we can detect $d$ Byzantine replicas by a \emph{forensic protocol} that takes a set of transcripts as input and output an \emph{irrefutable} proof of $d$ culprits with soundness 1. With the irrefutable proof, any party (not necessarily in the BFT system) can be convinced of the culprits' identities \emph{without} any assumption on the number of honest replicas. } 
% TODO \gerui{remove below, and redefine k}
% \gerui{However, if even with transcripts from all honest replicas no forensic protocol can output such a proof, the consensus protocol has no forensic support and we denote it as None in Table~\ref{tab:results}.}\peiyao{Since we can not expect to get transcripts from the Byzantine replicas.} \Sk{irrefutable proof should hold *without* any assumption on the number of honest nodes.}


To provide forensic support, we consider a setting where a client observes the existence of outputs for two conflicting (unequal)  
values.\footnote{We assume all the (honest) replica outputs are eventually learned by the client. In practice, the client may monitor the outputs by periodically communicating with all replicas.} By running a forensic protocol, the client sends (possibly a subset of) these conflicting outputs to all replicas and waits for their replies. Some of these replicas may be ``witnesses'' and may have (partial) information required to construct the irrefutable proof. After receiving responses from the replicas, the client constructs the proof. We denote by $k$ the total number of transcripts from different honest replicas that are stored by the client to construct the proof.  %\peiyao{ For any reply the client receives, it can choose whether to store the transcript or ignore it. If the transcript sent by some replica has been stored by the client (even if it is finally discarded), the replica will be counted in $k$. Moreover, some (even all) of the replicas in $k$ can be Byzantine and they can send arbitrary transcripts (but can not forge others signed messages). Byzantine replicas can also keep silent in the forensic phase. For forensic support, with the transcripts received by $k$ replicas, the client can eventually obtain an irrefutable proof for the culpability of $d$ Byzantine replicas.
\begin{definition}
\label{defn:forensic-support}
$(\mathbf{m},\mathbf{k},\mathbf{d})$-{\bf Forensic Support}.  If $t < f \leq m$ and two honest replicas output conflicting values, then using the transcripts of all messages received from $k$ honest replicas during the protocol, a client can provide an irrefutable proof of culpability of at least $d$ Byzantine replicas.
\end{definition}
% \kartik{deleted a long comment here}%\gerui{k means kmax, so do we say at most $k$?} \Sk{the quantifier on $k$ is not clear.  There seem to be three things: (1) for any execution, it is $ \leq k$ (that is why Gerui is saying $k_{max}$), (2) but it has to be a specific $k$ nodes (3) who knows who are those k nodes. all three attributes need to be specified.Is this accurate: "then, in any execution, there exist $k$ nodes (who can self-identify based on the conflicting values) such that the transcripts..." } \gerui{exist k doesn't fit, since \hsb exist a set of 2 nodes rather than t+1}




%\begin{itemize}
%    \item Does the def need to specify ``with the transcripts'' means ``the transcripts have been stored''?
%    \item discuss what m means
 %   \item discuss d is either 0 or t+1
 %   \item discuss k means the distributed level of collaboration
%\end{itemize}

% With the irrefutable proof, any party (not necessarily in the SMR system) can be convinced of the culprits' identities without extra communication with the SMR system. }Note that forensic support is an additional property provided to SMR/validated Byzantine agreement protocols, and hence, the notations $f$ and $t$ refer to the notations in those definitions. In addition to an external client, a replica can also request for forensic support.

\myparagraph{Other assumptions.}
We consider forensic support for multiple protocols each with their own network assumptions. For PBFT and HotStuff, we assume a partially synchronous network~\cite{dwork1988consensus}. For VABA~\cite{abraham2019asymptotically} and Algorand~\cite{chen2019algorand}, we suppose  asynchronous and synchronous networks respectively.
%\peiyao{For different protocols, we assume different network settings. For PBFT and HotStuff, we assume a partially synchronous network where there is an unknown time bound GST until which messages sent between replicas are only eventually delivered. After GST, all messages will arrive within a bounded delay $\Delta$ after they are sent. For VABA, we assume an asynchronous network with unbounded delivery time. For Algorand, we assume a synchronous settings where the bound of message delivery time is known.}

We assume all messages are digitally signed except for one variant of PBFT (\S\ref{sec:pbft-mac}) that sometimes relies on the use of Message Authenticated Codes (MACs). Some protocols, e.g., HotStuff, VABA, use threshold signatures. For forensic purposes, we assume  multi-signatures~\cite{bls} instead (possibly worsening the communication complexity in the process). Whenever the number of signatures exceeds a threshold, the resulting aggregate signature is denoted by a pair $\sigma = (\sigma_{agg}, \epsilon)$, where $\epsilon$ %\gerui{a review say $b_0,..b_{n-1}$ and replica identity is not clear. I suggest we remove $[b_0,\cdots,b_{n-1}]$, and just say $\epsilon$ is a bitmap.} 
is a bitmap indicating whose signatures are included in $\sigma_{agg}$. 
We define the intersection of two aggregated messages to be the set of replicas who sign both messages, i.e., $\sigma \cap \sigma' := \{i|\sigma.\epsilon[i]\land \sigma'.\epsilon[i] = 1\}$. An aggregate signature serves as a quorum certificate (QC) in our protocols, and we will use the two terms interchangeably. We assume a collision resistant cryptographic hash function. % \gerui{We assume we have a preimage resistant, collision resistant cryptographic hash function~\cite{menezes2018handbook}.}

==> [CCS21] BFT Protocol Forensics/4_pbft_mac.tex <==
\section{Forensic Support for PBFT}\label{sec:pbft}

PBFT is a classical partially synchronous consensus protocol that provides an optimal resilience of $t$ Byzantine faults out of $n = 3t+1$ replicas. However, when the actual number of faults $f$ exceeds $t$, it does not provide any safety or liveness. In this section, we  show that when $f > t$ and in case of a safety violation,  the variant of the PBFT protocol (referred to as PBFT-PK) where all messages sent by parties are signed, has the \emph{strongest forensic support}. Further, we  show that for an alternative variant where parties sometimes only use MACs (referred to as PBFT-MAC), forensic support is impossible.

\subsection{Overview} 
\label{subsec:pbft-overview}
We start with an overview  focusing on  a single-shot version of PBFT, i.e., a protocol for consensus on a single value. The protocol described here uses digital signatures to authenticate all messages and routes messages through leaders as shown in \cite{ramasamy2005parsimonious}; however we note that our arguments  for PBFT-PK also apply to the original protocol in \cite{castro1999practical}. % \kartik{when signatures are used, our analysis should hold for original PBFT too, right?}\peiyao{Yes, if all messages are signed} %(which is different from the original protocol in \cite{castro1999practical}).}\gerui{The protocol described below is the variant adapted from Ramasamy and Cachin~\cite{ramasamy2005parsimonious} and is different from the original protocol~\cite{castro1999practical,castro2002practical}. Comparing with the original one, it uses digital signatures to authenticate all messages and routes messages through leaders. The original PBFT is discussed in section~\ref{sec:pbft-mac}.} 

The protocol proceeds in a sequence of consecutive views denoted as view number $e = 1, 2, \cdots$. A higher view is a view with a larger view number. Each view has a unique leader. Each view of PBFT progresses as follows:

\begin{itemize}[leftmargin=*, topsep=0pt]
    \item[-] \textbf{\ppr.} The leader proposes a \nv message containing a proposal $v$ and a status certificate $M$ (explained later) to all replicas.
    \item[-] \textbf{\vone.} On receiving the first \nv message containing a valid value $v$ in a view $e$, a replica sends \vone for $v$ if it is \emph{safe} to vote based on a locking mechanism (explained later). It sends this vote to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qctwo. The leader sends \qctwo to all replicas.
    \item[-] \textbf{\commit.} On receiving a \qctwo in view $e$ containing message $v$, a replica locks on $(v, e)$ and sends \commit to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qcthree. The leader sends \qcthree to all replicas.
    \item[-] \textbf{\reply.} On receiving \qcthree from the leader, replicas output $v$ and send a \reply (along with \qcthree) to the client.
\end{itemize}

Once a replica locks on a value $v$ in view $e$, we call $(v, e)$ is the current lock of this replica. And a higher lock is a lock formed in a higher view. With lock $(v,e)$, the replica only votes for the value $v$ in subsequent views. The only scenario in which it votes for a value $v' \neq v$ is when the status certificate $M$ provides sufficient information stating that $2t+1$ replicas are not locked on $v$. At the end of a view, every replica sends its lock to the leader of the next view. The next view leader collects $2t+1$ such values as a status certificate $M$.

The safety of PBFT follows from two key quorum intersection arguments:

\myparagraph{Uniqueness within a view.} Within a view, safety is ensured by votes in either round. Since a replica only votes once for the first valid value it receives, by a quorum intersection argument, two conflicting values cannot both obtain \qcthree when $f \leq t$. 

\myparagraph{Safety across views.} Safety across views is ensured by the use of locks and the status certificate. First, observe that if a replica $r$ outputs a value $v$ in view $e$, then a quorum of replicas lock on $(v, e)$. When $f \le t$, this quorum includes a set $H$ of at least $t+1$ honest replicas. For any replica in $H$ to update to a higher lock, they need a \qctwo in a higher view $e' > e$, which in turn requires a vote from at least one of these honest replicas in view $e'$. 
However, replicas in $H$ will vote for a conflicting value $v'$ in a higher view only if it is accompanied by a status certificate $M$ containing $2t+1$ locks that are not on value $v$. When $f \le t$, honest replicas in $M$ intersect with honest replicas in $H$  at least one replica -- this honest replica will not vote for a conflicting value $v'$.

%\peiyao{\myparagraph{Variants of PBFT} In terms of the methods to authenticate messages, there are two versions of PBFT. The first variant is based on \cite{castro1999practical} and described above (called PBFT-PK), where leaders route all messages in \prepare and \commit phases. It uses public key to verify signatures of all messages. The second variant is based on \cite{castro2002practical} (called PBFT-MAC) and uses all to all communication in \prepare and \commit phases, it utilizes shared secret to establish authenticated communications between any two replicas, .} \kartik{can we delete this paragraph? does the content at start of the section suffice?} \peiyao{yes, let me move the variant name to the start of the section too.}


\subsection{Forensic Analysis for PBFT-PK}

The agreement property for PBFT holds only when $f \leq t$. When the number of faults are higher, this agreement property (and even termination) can be violated. In this section, we show how to provide forensic support for PBFT when the agreement property is violated. We show that, if two honest replicas output conflicting values $v$ and $v'$ due to the presence of $t<f \le m$ Byzantine replicas, our forensic protocol can detect $t+1$ Byzantine replicas with an irrefutable proof. For each of the possible scenarios in which safety can be violated, the proof shows exactly what property of PBFT was not respected by the Byzantine replicas. The irrefutable proof explicitly uses messages signed by the Byzantine parties, and is thus only applicable to the variant PBFT-PK where all messages are signed. % \peiyao{And since the irrefutable proof should be able to convince a third party, it is supposed to be publicly verifiable. We will discuss how PBFT-PK finds such proof and how PBFT-MAC fails to do the same thing.} 


\myparagraph{Intuition.} In order to build intuition, let us assume $n = 3t+1$ and $f = t+1$ and start with a simple scenario: two honest replicas output values $v$ and $v'$ in the same view. It must then be the case that a \qcthree is formed for both $v$ and $v'$. Due to a quorum intersection argument, it must be the case that all replicas in the intersection have voted for two conflicting values to break the uniqueness property. Thus, all the replicas in the intersection are culpable. For PBFT-PK, the \qcthree (as well as \qctwo) for the two conflicting values act as the irrefutable proof for detecting $t+1$ Byzantine replicas. 


\begin{figure}[htbp]
    \centering
    %\vspace{-20pt}
    \includegraphics[width=\columnwidth]{figures/pbft.pdf}
    \caption{\textbf{An example sequence of events in the PBFT-PK protocol that leads to replicas $i$ and $j$ outputting different values. }}
    \label{fig:pbft-disagree}
   % \vspace{-20pt}
\end{figure}

When two honest replicas output conflicting values in different views, there are many different sequences of events that could lead to such a disagreement. One such sequence is described in Figure~\ref{fig:pbft-disagree}. The replicas are split into three sets: the blue set and the green set are honest replicas each of size $t$  and the red replicas are Byzantine replicas of size $t+1$. 

\begin{itemize}[leftmargin=*, topsep=0pt]
    \item In view $e$, replica $i$ outputs $v$ due to $\qcthree$ formed with the $\commit$ from the honest blue set and the Byzantine red set. At the end of the view, replicas in the blue and red set hold locks $(v, e)$ whereas the green set holds a lower lock for a different value. 
    \item In the next few views, no higher locks are formed. Thus, the blue and the red set still hold locks $(v, e)$.
    \item Suppose $e^*$ is the first view where a higher lock is formed. At the start of this view, the leader receives locks from the honest green set who hold lower-ranked locks and the Byzantine red set who maliciously send lower-ranked locks. The set of locks received by the leader is denoted by $M$ and suppose the highest lock was received  for $v'$. The leader proposes $v'$ along with $M$. This can make any honest replica ``unlock'' and vote for $v'$ and form quorum certificates in this view.
    \item In some later view $e'$, replica $j$ outputs $v'$.
\end{itemize}

With this sequence of events, consider the following questions: (1) Is this an admissible sequence of events? (2) How do we find the culpable Byzantine replicas? What does the irrefutable proof consist of? (3) How many replica transcripts do we need to construct the proof?

To answer the first question, the only nontrivial part in our example is the existence of a view $e^*$ where a higher lock is formed. However, such a view $e < e^* \leq e'$ must exist because replica $j$ outputs in view $e'$ and a higher lock must be formed at the latest in view $e'$. 

For the second question, observe that both the red replicas as well as the green replicas sent locks lower than $(v, e)$ to the leader in $e^*$. However, only the red replicas also sent \commit messages for value $v$ in view $e$. Thus, by intersecting the set of \commit messages for value $v$ in view $e$ and the messages forming the status certificate sent to the leader of $e^*$, we can obtain a culpable set of $t+1$ Byzantine replicas. So the proof for PBFT-PK consists of the \qcthree in $e$ and the status certificate in $e^*$, which indicates that the replicas sent a lower lock in view $e^*$ despite having access to a higher lock in a lower view $e$. 

For the third question, the \nv message containing the status certificate $M$ in view $e^*$ can act as the proof, so only one transcript needs to be stored. 

\begin{algorithm}[htbp]
\begin{algorithmic}[1]
\As{a replica running PBFT-PK}
    \State $Q\gets $ all \nv messages in transcript\label{alg:pbft-3}
    \Upon{$\lr{\conflictacross, e, v, e'}$ from a client}
        \For{$m \in Q$}
            \State $(v'',e'')\gets$ the highest lock in $m.M$
            \If{$(m.e \in(e, e'])\land(v''\neq v)\land(e'' \le e)$} 
                \State send $\lr{\nv, m}$ to the client\label{alg:pbft-13}
            \EndIf
        \EndFor
    \EndUpon
\EndAs{}

\As{a client}
    \Upon{two conflicting \reply messages}\label{alg:pbft-18}
        \If{the two messages are from different views}
            \State $\lr{\reply,e,v,\sigma}\gets$ the message from lower view
            \State $e'\gets$ the view number of \reply from higher view
            \State broadcast $\lr{\conflictacross, e, v, e'}$ \label{alg:pbft-21}
            \State wait for: $\lr{\nv, m}$ s.t. $m.e\in(e,e']\land(v''\neq v)\land(e'' \le e)$ where $(v'',e'')$ is the highest lock in $m.M$. \label{alg:pbft-message-com-1}
            \If{in $m.M$ there are two locks $(e'',v_1,\sigma_1)$ and $(e'',v_2,\sigma_2)$ s.t. $v_1\neq v_2$} \label{alg:pbft-20-withinM}
            \State \textbf{output} $\sigma_1\cap \sigma_2$ 
            \Else
            \State \textbf{output} the intersection of senders in $m.M$ and signers of $\sigma$.\label{alg:pbft-23} 
            \EndIf
        \Else\label{alg:pbft-25}
            \ignore{\State $v, v',e\gets$ two output values and the view number
            \State broadcast $\lr{\conflictwithin, e, v, v'}$
            \State wait for: $qc, qc'\gets$ two \qctwo of output values from possibly different replicas in view $e$.
            \State \textbf{output} $qc.\sigma \cap qc'.\sigma$}
            \State $\lr{\reply,e,v,\sigma}\gets$ first \reply message
            \State $\lr{\reply,e,v',\sigma'}\gets$ second \reply message
            \State \textbf{output} $\sigma \cap \sigma'$\label{alg:pbft-28}
        \EndIf
    \EndUpon
\EndAs{}
\end{algorithmic}
\caption{Forensic protocol for PBFT-PK Byzantine agreement}
\label{alg:fa-pbft1}
\end{algorithm}

\myparagraph{Forensic protocol for PBFT-PK.}
Algorithm~\ref{alg:fa-pbft1} describes the entire protocol to obtain forensic support atop PBFT-PK. For completeness, we also provide a complete description of the PBFT-PK protocol in Algorithm~\ref{alg:single-pbft}. Each replica keeps all received messages as transcripts and maintains a set $Q$ containing all received \nv messages (line~\ref{alg:pbft-3}). If a client observes the replies of two conflicting values, it first checks if two values are output in the same view (line~\ref{alg:pbft-18}). If yes, then any two \qcthree for two different output values can provide a culpability proof for at least $t+1$ replicas (lines~\ref{alg:pbft-25}-\ref{alg:pbft-28}). Otherwise, the client  sends a request for a possible proof between two output views $e, e'$ (lines~\ref{alg:pbft-21}). Each replica looks through the set $Q$ for the \nv message in the smallest view $e^* > e$ such that the status certificate $M$ contains the highest lock $(e'', v'')$ where $v''\ne v$ and $e'' \le e$ and sends it to the client (line~\ref{alg:pbft-13}). If inside $M$ there are conflicting locks in the same view, the intersection of them proves at least $t+1$ culprits (line~\ref{alg:pbft-20-withinM}), otherwise the intersection of $M$ and the \qcthree proves at least $t+1$ culprits (line~\ref{alg:pbft-23}).

The following theorem sharply characterizes the forensic support capability of PBFT-PK. As long as $m\leq 2t$, the best possible forensic support is achieved (i.e., $k=1$ and $d=t+1$). Algorithm~\ref{alg:fa-pbft1} can be used to irrefutably detect $t+1$ Byzantine replicas.  Conversely, if $m > 2t$ then no forensic support is possible (i.e., $k=n-f$ (messages from all honest nodes) and $d=0$).    %The proof indicates the Byzantine action performed by a detected Byzantine replica. 

\begin{theorem}
\label{thm:pbft}
With $n=3t+1$, when $f>t$, if two honest replicas output conflicting values, PBFT-PK provides $(2t,\ 1,\ t+1)$-forensic support. Further $(2t+1, n-f, d)$-forensic support is impossible with $d>0$. 
\end{theorem}
\begin{proof} We prove the forward part of the theorem below. The converse (impossibility) is proved in \S\ref{sec:proofoftheorem4.1}. 
Suppose the values $v$ and $v'$ are output in views $e$ and $e'$ respectively. 

\myparagraph{Case $e=e'$.} 

\noindent\underline{Culpability.} The quorums \qcthree  for $v$ and \qcthree  for $v'$ intersect in $t+1$ replicas. These $t+1$ replicas should be Byzantine since the protocol requires a replica to vote for at most one value in a view. 


\noindent\underline{Witnesses.} Client can obtain the culpability proof based on two \qcthree. No additional communication is needed in this case ($k=0$).

\myparagraph{Case $e\neq e'$.}

\noindent\underline{Culpability.}
If $e \neq e'$, then WLOG, suppose $e < e'$. Since $v$ is output in view $e$, it must be the case that $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$ (if they are honest). Now consider the first view $e < e^* \leq e'$ in which a higher lock $(v'', e^*)$ is formed (not necessarily known to any honest party) where $v'' \neq v$ (possibly $v'' = v'$). Such a view must exist since $v'$ is output in view $e' > e$ and a lock will be formed in at least view $e'$. Consider the status certificate $M$ sent by the leader of view $e^*$ in its \nv message. $M$ must contain $2t+1$ locks; each of these locks must be from view $e'' \le e$, and a highest lock among them is $(v'', e'')$.  

We consider two cases based on whether the status certificate contains two different highest locks: (i) there exist two locks $(v'', e'')$ and $(v''', e'')$ s.t. $v'' \ne v'''$ in $M$. (ii) $(v'', e'')$ is the only highest lock in $M$. For the first case, since two locks are formed in the same view, the two quorums forming the two locks in view $e''$ intersect in $t+1$ replicas. These replicas are Byzantine since they voted for more than one value in view $e$.

For the second case, $(v'', e'')$ is the only highest lock in the status certificate $M$. $M$ intersects with the $2t+1$ signers of \qcthree in view $e$ at $t+1$ Byzantine replicas. These replicas are Byzantine because they had a lock on $v \ne v''$ in view $e \ge e''$ but sent a different lock to the leader of view $e^* > e$.
%We consider two cases based on whether the status message contains \peiyao{two different highest locks} lock $(v''', e)$ for a value $v''' \neq v''$. The two cases are (i) there does not exist such a lock $(v''', e)$, and (ii) there exists such a lock $(v''', e)$.  the first case, \gerui{a review say it's hard to follow and a figure helps. can we refer figure 1 here?} the status certificate $M$ with $2t+1$ locks intersect with the $2t+1$ signers of \qcthree in view $e$ at $t+1$ Byzantine replicas. These replicas are Byzantine because they had a lock in view $e$ that was different from, and at least as high as the one sent to the leader of view $e^* > e$.

%For the second case, since $v''$ is proposed in view $e^*$, it exists in the status certificate $M$ and is a highest lock in $M$. Moreover, in this case, $(v''', e)$ exists in $M$ too. \gerui{This means $M$ contains two different locks both formed in view $e$. (I think this is clearer than the next sentence.)} Both of these locks were formed in view $e$. The two quorums forming the two locks in view $e$ intersect in $t+1$ replicas. These replicas are Byzantine since they voted for more than one value in view $e$.

\noindent\underline{Witnesses.} Client can obtain the proof by storing the \nv message containing the status certificate $M$ in $e^{*}$. Only one witness is needed to provide the \nv message ($k=1$). The status certificate $M$ and the first \qcthree act as the irrefutable proof. %\kartik{transcripts/witnesses.}
\end{proof}

\myparagraph{Communication complexity.} In the first branch of the forensic protocol, Algorithm~\ref{alg:fa-pbft1}, the client needs to receive one message from $k=1$ replica and the message size is $(2t+1)(|v|+|sig|)$ where $|v|$ and $|sig|$ stand for the size of a value and an aggregate signature (line~\ref{alg:pbft-message-com-1}). In the second branch, the client doesn't need any message (line~\ref{alg:pbft-25}). Therefore the complexity of the client receiving messages is $O(n(|v|+|sig|))$. Notice that we exclude the communication for learning replica outputs (\reply messages) since that procedure happens \textit{before} the forensic protocol.



\subsection{Impossibility for PBFT-MAC}\label{sec:pbft-mac}
%\gerui{TODO: point out that Byzantine can refuse to answer during forensic. or point out it in the model section?}\peiyao{I added a sentence in the model section for this.}
%\gerui{Perhaps we can describe PBFT-MAC here and not describe it in previous sections?} \kartik{can we explain this as a diff from what is described in overview section? also need intuition for why this is impossible.}
We now show an impossibility for a variant of PBFT proposed in \cite[Section 5]{castro1999practical}. The arguments here also apply to the variant in \cite{castro2002practical}. Compared to \S\ref{subsec:pbft-overview}, the only difference in this variant is (i)  \prepare and \commit messages are authenticated using MACs instead of signatures, and (ii) these messages are broadcast instead of routing them through the leader.

% The variant PBFT-MAC is originally proposed in \cite[Section 5]{castro1999practical}, but the same argument works for the variant in \cite{castro2002practical}. PBFT-MAC authenticates messages such as \commit messages using MACs rather than signatures. And replicas broadcast \prepare and \commit messages rather than route it via a leader. As we will show, the use of MACs makes it impossible to provide forensic support.

\myparagraph{Intuition.} The key intuition behind the impossibility relies on the absence of digital signatures which were used to ``log'' the state of a replica when some replica $i$ outputs a value. In particular, if we consider the example in Figure~\ref{fig:pbft-disagree}, while $i$ receives $2t+1$ \commit messages for value $ v$, these messages are not signed. Thus, if  $t+1$ Byzantine replicas vote for a different value $v'$, $v'$ can be output by a different replica. % (signed) to the leader of the next view, $v'$ can be committed in a subsequent view. 
The absence of a verifiable proof stating the set of replicas that sent a \commit to replica $i$ prevents any forensic analysis. We formalize this intuition below.

\ignore{A broadcast message from replica $x$ carries a vector of MACs, which includes the MAC between $x,y$ for any $y\neq x$. When replica $y$ receives the message, it can only check the MAC between $x,y$ and not between $x,z$ for $z\neq y$. As a result, if $x$ is Byzantine, it can include invalid MACs between $x,z$ for all $z\neq y$ and still make $y$ accept such a {\it partially valid} message. And if $y$ is Byzantine, it can also create such a partially valid message. Therefore, given such a partially valid message, a client cannot distinguish whether $x$ or $y$ is Byzantine. We will use this property on \commit messages to construct two indistinguishable worlds. In one world a Byzantine replica $x$ does broadcast a partially valid \commit message, and in another world a Byzantine replica $y$ claims $x$ has broadcast the message therefore frames honest replica $x$.}

\begin{theorem}
With $n=3t+1$, when $f>t$, if two honest replicas output conflicting values, $(t+1, 2t, d)$-forensic support is impossible with $d>0$ for PBFT-MAC.
\end{theorem}

\begin{proof}
Suppose the protocol provides forensic support to detect $d \geq 1$ replicas with irrefutable proof. To prove this result, we construct two worlds where a different set of $t+1$ replicas are Byzantine in each world but a forensic protocol cannot be correct in both worlds. We fix $f = t+1$, although the arguments will apply for any $f > t$.

Let there be four replica partitions $P,Q,R,\{x\}$. $|P|=|Q|=|R|=t$, and $x$ is an individual replica. In both worlds, the conflicting outputs are presented in the same view $e$. Suppose the leader is a replica from set $R$.

\myparagraph{World~1.} Let $P$ and $x$ be Byzantine replicas in this world. The honest leader from set $R$ in view $e$ proposes $v'$. Parties in $R$, $x$ and $Q$ send \prepare and \commit messages (authenticated with MACs) for value $v'$. Due to partial synchrony, none of these messages arrive at $P$. At the end of view $e$, only $R$ and one replica $q$ in $Q$ receive enough \commit messages and send replies to the client. So the client receives the first set of $t+1$ replies for value $v'$, which contain the same quorum $R, x, Q$.

The Byzantine parties in $P$ and $x$ simulate a proposal from the leader for $v$, and the sending of \prepare and \commit messages within $R, P$ and $x$. The simulation is possible due to the absence of a PKI. At the end of view $e$, $P$ and $x$ obtain enough \commit messages and send replies to the client. Thus, the client receives the second set of $t+1$ replies for value $v$, which contain the same quorum $P, R, x$.% The Byzantine parties in $P$ and $x$ forge a proposal from the leader for $v$ and broadcast \prepare and \commit messages for value $v$ within $P$ and $x$. Besides, they forge the \prepare and \commit messages from the honest party $R$. At the end of view $e$, $P$ and $x$ get enough \commit messages and send replies to the client. So the client receives the second set of $t+1$ replies for value $v$, which contain the same quorum $P, R, x$. 
 Client starts the forensic protocol.

During the forensic protocol, Byzantine $P$ and $x$ only present the votes for $v$, forged votes from $R$ as their transcripts. Since $t+1$ parties have output each of $v$ and $v'$, there is a safety violation. Since the protocol has forensic support for $d\geq 1$, using these transcripts, the forensic protocol determines some subset of $P$ and $x$ are culpable.

\myparagraph{World~2.} Let $R$ and $q$ (one replica in $Q$) be Byzantine replicas in this world. The Byzantine leader in view $e$ proposes $v$ to $P, R$ and $x$. They send \prepare and \commit messages (authenticated with MACs) for value $v$. These messages do not arrive at $Q$. At the end of view $e$, parties in $P$ and $x$ output $v$. So the client receives the first set of $t+1$ replies for value $v$, which contain the same quorum $P, R, x$.

Similarly, the leader sends $v'$ to $Q, R$ and $x$. The proposal does not arrive at $x$. Only $Q$ and $R$ send \prepare and \commit messages (authenticated with MACs) for $v'$, these messages do not arrive at $P$. However, $R$ and $q$ forge \prepare and \commit messages from $x$. At the end of view $e$, $R$ and $q$ output $v'$. So the client receives the second set of $t+1$ replies for value $v'$, which contain the same quorum $R, x, Q$. Client starts the forensic protocol.
 
During the forensic protocol, Byzantine $R$ and $q$ sends the same transcripts as in World~1 by dropping votes for $v$ and forging votes from $x$. Again, since $t+1$ parties have output each of $v$ and $v'$, there is a safety violation. However, observe that the transcript presented to the forensic protocol is identical to that in World~1. Thus, the forensic protocol outputs some subset of $P$ and $x$ as culpable replicas. In World~2, this is incorrect since replicas in $P$ and $x$ are honest. This completes the proof.

\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ignore from here

\ignore{
\begin{theorem}
When $f > t$, there exists an execution of PBFT-MAC where a safety violation occurs and we cannot provide forensic support for $m > t$, $k = n$, and $d = t+1$.
\end{theorem}


\begin{table}[!htb]
\caption{World 1. ``$\Leftarrow$'' means receive and ``$\Rightarrow$'' means send/broadcast.}
\label{tab:pbft-mac-1}
\begin{footnotesize}
\begin{tabular}{|c|c|}\hline
  & View $e$  \\\hline
$P$ & \makecell{$\Rightarrow$\commit on $v$,\\form $\qcthree_1$ on $v$\\$\Leftarrow\qcthree_1$} \\\hline
$Q$ & \makecell{$\Rightarrow$\commit on $v'$,\\form $\qcthree_2$ on $v'$\\$\Leftarrow\qcthree_2$} \\\hline
\color{red}{$R$} & \makecell{$\Rightarrow$\commit on $v$ to $P$,\\$\Rightarrow$\commit on $v'$ to $Q$,\\form $\qcthree_1,\qcthree_2$\\$\Leftarrow\qcthree_1$} \\\hline
\color{red}{$x$} & same as above\\\hline
\end{tabular}
\end{footnotesize}
\end{table}

\begin{table}[!htb]
\caption{World 2. ``$\Leftarrow$'' means receive and ``$\Rightarrow$'' means send/broadcast.}
\label{tab:pbft-mac-2}
\begin{footnotesize}
\begin{tabular}{|c|c|}\hline
  & View $e$  \\\hline
\color{red}{$P$} & \makecell{$\Rightarrow$\commit on $v$,\\forge \commit from $R$\\form $\qcthree_1$ on $v$\\$\Leftarrow\qcthree_1$} \\\hline
$Q$ & \makecell{$\Rightarrow$\commit on $v'$,\\form $\qcthree_2$ on $v'$\\$\Leftarrow\qcthree_2$} \\\hline
$R$ & \makecell{$\Rightarrow$\commit on $v'$,\\form $\qcthree_2$ on $v'$\\$\Leftarrow\qcthree_2$} \\\hline
\color{red}{$x$} & \makecell{$\Rightarrow$\commit on $v$ to $P$,\\$\Rightarrow$\commit on $v'$ to $Q$,\\form $\qcthree_1,\qcthree_2$\\$\Leftarrow\qcthree_1$}\\\hline
\end{tabular}
\end{footnotesize}
\end{table}

\begin{proof}
Suppose the protocol provides forensic support to detect $d \geq t+1$ replicas with irrefutable proof. To prove this result, we construct two worlds where a different set of $t+1$ replicas are Byzantine in each world but a forensic protocol cannot be correct in both worlds. We fix $f = t+1$, although the arguments will apply for any $f > t$.

Let there be four replica partitions $P,Q,R,\{x\}$. $|Q|=|P|=|R|=t$, and $x$ is an individual replica. In both worlds, the conflicting outputs are presented in the same view $e$. Suppose the leader is a replica from set $R$.

\myparagraph{World~1.} Let $R$ and $x$ be Byzantine replicas in this world. The Byzantine leader in view $e$ proposes $v$ to $P, R$ and $x$. They send \prepare and \commit messages (authenticated with MACs) for value $v$. Parties in $P$ output $v$ in view $e$. Due to partial synchrony, none of these messages arrive at $Q$.
Similarly, the leader sends $v'$ to $Q, R$ and $x$. They send \prepare and \commit messages (authenticated with MACs) for $v'$; these messages do not arrive at $P$ but arrive at other parties. Parties in $Q$ output $v'$ in view $e$.

% Subsequently, all message are delayed. Thus, all parties except those in $P$ send (signed) \vc messages with a lock on $v'$. In view $e+1$, the leader proposed $v'$ with a supporting status certificate and honest replicas in $Q$ commit $v'$.

During the forensic protocol, $P$ and $Q$ send their transcripts and state that they have output $v$ and $v'$ respectively. Byzantine $R$ only presents its communication with $Q$ and states that it has committed $v'$. Byzantine $x$ only presents its communication with $P$ and $R$ and states that it has committed $v$. Since $\geq t+1$ parties have committed each of $v$ and $v'$, there is a safety violation. Since the protocol has forensic support, using these transcripts, the forensic protocol determines $R$ and $x$ are culpable.

% If this protocol has any forensic support, then it should be able to detect the $d = t+1$ Byzantine replicas with an irrefutable proof. The Byzantine replica $x$  Suppose given all honest transcripts, the protocol detects 

\myparagraph{World~2.} Let $P$ and $x$ be Byzantine replicas in this world. The honest leader from set $R$ in view $e$ proposes $v'$. Parties in $R$, $x$ and $Q$ send \prepare and \commit messages (authenticated with MACs) for value $v'$. These messages do not arrive at $P$. The Byzantine parties in $P$ and $x$ simulate the receipt of a proposal for $v$ and of \prepare and \commit messages for value $v$ from parties in $P, R$ and $x$.

During the forensic protocol, $Q$ and $R$ send their transcripts and state that they have committed $v'$. Byzantine $P$ and $x$ only present the simulated communication between $P, R$ and $x$ as their transcripts. Again, since $\geq t+1$ parties have committed each of $v$ and $v'$, there is a safety violation. However, observe that the transcript presented to the forensic protocol is identical to that in World~1. Thus, the forensic protocol outputs $R$ and $x$ as culpable replicas. In world 2, this is incorrect since replicas in $R$ are honest. This completes the proof.

\ignore{
\kartik{Gerui's proof below}
Suppose in the sense of contradiction that an irrefutable proof of culprits exists for any execution. We will construct two worlds of execution where different $t+1$ replicas are Byzantine in different worlds. We will fix the number of Byzantine replicas $f=t+1$, but the following argument works for any $f\ge t+1$.

Let there be five replica partitions $P,Q,R,\{x\},\{y\}$. $|Q|=t-1,|P|=|R|=t$, and $x,y$ are individual replicas. In worlds 1 and 2, the conflicting outputs are in views $e,e'$ and $e'=e+1$).

\myparagraph{World 1} World 1 is presented in table~\ref{tab:pbft-mac-1}. Let $R$ and $x$ be Byzantine replicas in this world. They, together with $P$, broadcast \commit on $v$ in view $e$. And they, together with $Q$ and $y$, send \vc on $v'$ to the next leader in the view change between $e$ and $e+1$. The MACs of \commit messages sent by Byzantine replica $x$ in view $e$ is partially valid, that is, suppose the recipient of the message is $z$, then only the MAC for $z$ is valid. Notice that replica $z$ cannot check the validity of MACs for other replicas, therefore it considers the message valid. Such partially valid MACs help the construction of world 2.  

Let the replicas in $R$ provide their true transcripts to the client. However, let Byzantine replica $x$ not provide any information. In this way, the irrefutable proof can and has to be computed from transcripts from all replicas but $x$. At last, suppose the irrefutable proof holds $R$ and $x$ as culprits which are the correct ones.

\myparagraph{World 2} World 2 is presented in table~\ref{tab:pbft-mac-2}. Let $R$ and $y$ be Byzantine replicas in this world. They, together with $P$, broadcast \commit on $v$ in view $e$. And they, together with $Q$ and $x$, send \vc on $v'$ in the view change between $e$ and $e+1$. Let replicas in $R$ forge $\qcthree_1$ as world 1, such that the quorum contains the vote from $x$ rather than $y$. Notice that the vote from $x$ is forgeable since the vote in world 1 is partially valid, and the recipient can forge its MAC. Replicas put the forged $\qcthree_1$ in the transcripts and provide it to the client. Let replica $y$ forge their transcripts as in world 1. And the transcripts from $P$ and $Q$ are indistinguishable from world 1. As a result, the transcripts from all replicas but $x$ are indistinguishable to world 1. Hence, the irrefutable proof can be computed from transcripts from all replicas but $x$, and it should hold $R$ and $x$ as culprits as in world 1, which is a contradiction.

By the proof of contradiction, there exists an execution of this PBFT variant such that there is no irrefutable proof of $t+1$ culprits.
}
\end{proof}
}
% \noindent\emph{Remark.} Observe that the proof did not rely on the 

==> [CCS21] BFT Protocol Forensics/5_hotstuff.tex <==
\section{Forensic Support for HotStuff}
\label{sec:basic-hotstuff}
HotStuff~\cite{yin2019hotstuff} is a partially synchronous consensus protocol that provides an optimal resiliency of $n = 3t+1$.  The HotStuff protocol is similar to PBFT but there are subtle differences which allow it to obtain a linear communication complexity for both its steady state and view change protocols (assuming the presence of threshold signatures). Looking ahead, these differences significantly change the way forensics is conducted if a safety violation happens.

\subsection{Overview}  We start with an overview of the protocol. For simplicity, we discuss a single-shot version of HotStuff. The protocol proceeds in a sequence of consecutive views where each view has a unique leader. Each view of HotStuff progresses as follows:\footnote{The description of HotStuff protocol is slightly different from the basic algorithm described in~\cite[Algorithm~2]{yin2019hotstuff} to be consistent with the description of PBFT in \S\ref{subsec:pbft-overview}.}
\begin{itemize}[leftmargin=*, topsep=0pt]
    \item[-] \textbf{\ppr.} The leader proposes a \nv message containing a proposal $v$ along with the \hqc (the highest \qctwo known to it) and sends it to all replicas.
    \item[-] \textbf{\prepare.} On receiving a \nv message containing a valid value $v$ in a view $e$ and a \hqc, a replica sends \prepare for $v$ if it is \emph{safe} to vote based on a locking mechanism (explained later). It sends this vote to the leader. The leader collects $2t+1$ votes to form an aggregate signature \qctwo in view $e$. The leader sends the view $e$ \qctwo to all replicas.
    \item[-] \textbf{\precommit.} On receiving a \qctwo in view $e$ containing message $v$, a replica updates its highest \qctwo to $(v, e)$ and sends \precommit to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qcprecom.
    \item[-] \textbf{\commit.} On receiving \qcprecom in view $e$ containing message $v$ from the leader, a replica locks on $(v, e)$ and sends \commit to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qcthree.
    \item[-] \textbf{\reply.} On receiving \qcthree from the leader, replicas output the value $v$ and send a \reply (along with \qcthree) to the client.%\kartik{along with \qcthree or entire transcript?}\peiyao{yes, along with \qcthree is added. They only send transcript upon receiving request for proof.}
\end{itemize}

Once a replica locks on a given value $v$, it only votes for the value $v$ in subsequent views. The only scenario in which it votes for a value $v' \neq v$ is when it observes a \hqc from a higher view in a \nv message. At the end of a view, every replica sends its highest \qctwo to the leader of the next view. The next view leader collects $2t+1$ such values and picks the highest \qctwo as \hqc. 
The safety and liveness of HotStuff when $f \leq t$ follows from the following:

\myparagraph{Uniqueness within a view.} Since replicas only vote once in each round, a \qcthree can be formed for only one value when $f \leq t$.


\myparagraph{Safety and liveness across views.} Safety across views is ensured using locks and the voting rule for a \nv message. Whenever a replica outputs a value, at least $2t+1$ other replicas are locked on the value in the view. Observe that compared to PBFT, there is no status certificate $M$ in the \nv message to ``unlock'' a replica. Thus, a replica only votes for the value it is locked on. The only scenario in which it votes for a conflicting value $v'$ is if the leader includes a \qctwo for $v'$ from a higher view in \nv message. This indicates that at least $2t+1$ replicas are not locked on $v$ in a higher view, and hence it should be safe to vote for it. The latter constraint of voting for $v'$ is not necessary for safety, but only for liveness of the protocol.

\myparagraph{Variants of HotStuff.}
In this paper, we study three variants of HotStuff, identical for the purposes of consensus but provide varied forensic support. The distinction among them is only in the information carried in \vone message. For all three versions, the message contains the message type \vone, the current view number $e$ and the proposed value $v$. In addition, \vone in \hsa contains $\eqc$, the view number of the \hqc in the \nv message. \hsb contains the hash of \hqc (cf. Table~\ref{tab:hotstuff_variants}). \hsb is equivalent to the basic algorithm described in~\cite[Algorithm 2]{yin2019hotstuff}. \hsc does not add additional information.

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
    \toprule
         & \hsa &\hsb&\hsc  \\
        \toprule
        \info & $\eqc$&$ \text{Hash}(\hqc)$&$\emptyset$\\
        %\midrule
        $m$ & $2t$ & $2t$ &  $t+1$\\

        $k$ & $1$ & $t+1$ & $2t$\\
        %\midrule
        %\midrule
        $d$ & $t+1$ & $t+1$ & $1$\\
        %\midrule
        \bottomrule
    \end{tabular}
    \caption{Comparison of different variants of HotStuff, the \prepare message is $\signed{\vone,e,v, \info}$}
    \label{tab:hotstuff_variants}
\end{table}



\subsection{Forensic Analysis for HotStuff}
% \myparagraph{Intuition.} 
If two conflicting values are output in the same view, Byzantine replicas can be detected using \qcthree  and using ideas similar to that in PBFT. However, when the conflicting outputs of replicas $i$ and $j$ are across views $e$ and $e'$ for $e < e'$, the same ideas do not hold anymore. To understand this, observe that the two key ingredients for proving the culpability of Byzantine replicas in PBFT were (i) a \qcthree  for the value output in a lower view (denoted by $\sigma$ for replica $i$'s reply in Figure~\ref{fig:pbft-disagree}) and (ii) a status certificate from the first view higher than $e$ containing the locks from $2t+1$ replicas (denoted by $M$ for view $e^* > e$ in Figure~\ref{fig:pbft-disagree}). In HotStuff, a \qcthree still exists. However, for communication efficiency reasons, HotStuff does not include a status certificate $M$ in its \nv message. The status certificate in PBFT provides us with the following:

\begin{itemize}[leftmargin=*, topsep=0pt]
    \item \textbf{Identifying a potential set of culpable replicas.} Depending on the contents of $M$ and knowing $\sigma$, we could identify a set of Byzantine replicas.
    \item \textbf{Determining whether the view is the first view where a higher lock for a conflicting value is formed.} By inspecting all locks in $M$, we can easily determine this. Ensuring first view with a higher lock is important; once a higher lock is formed, even honest replicas may update their locks and the proof of Byzantine behavior may not exist in the messages in subsequent views.
\end{itemize}




\begin{figure}[tbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/hotstuff-same.pdf}
    \caption{\textbf{Depiction of events in the \hsa protocol for the first view where a higher \qctwo for $v'$ is formed.} } 
    \label{fig:hotstuff-same}
\end{figure}

Let us try to understand this based on the first view $e^\#$ where a higher \qctwo is formed for $v'\ne v$ (see Figure~\ref{fig:hotstuff-same}).  The set of replicas who sent \vone (the red ellipse) in $e^\#$ and formed a \qctwo are our potential set of Byzantine replicas. Why? If $e^\#$ is indeed the first view in which a higher \qctwo is formed, then all of these replicas voted for a \nv message containing a \hqc from a lower or equal view $e''$ on a different value. If any of these replicas also held a lock $(v, e)$ (by voting for replica $i$'s output) then these replicas have output the culpable act of not respecting the voting rule. 

The only remaining part is to ensure that this is indeed the first view where a higher conflicting \qctwo is formed. The way to prove this is also the key difference among three variants of HotStuff. For \hsa, \qctwo contains $\eqc$, which explicitly states the view number of \hqc in the \nv message they vote for. If $\eqc < e$, \qctwo provides an irrefutable proof for culpable behavior. For \hsb, the hash information contained in \vone provides the necessary link to the \nv message they vote, so once the linked \nv message is accessible, the \qctwo and \nv together serve as the proof for culpable behavior. However for \hsc, even if we receive both \qctwo and \nv messages that are formed in the same view, no proof can be provided to show a connection between them. A Byzantine node vote for the first higher \qctwo can always refuse to provide the \nv message they receive.

Thus, to summarize, the red set of replicas in view $e^\#$ are a potential set of culpable nodes of size $t+1$. The irrefutable proof to hold them culpable constitutes two parts, (1) the first \qctwo containing their signed \vone messages, and (2) a proof to show this is indeed the first view. In the next two subsections we will introduce the forensic protocols for \hsa and \hsb to provide different forensic supports, and how it is impossible for \hsc to provide forensic support.

\subsection{Forensic Protocols for \hsa and \hsb}

\begin{algorithm}[htbp]
\begin{algorithmic}[1]
\As{a replica running \hsa}
    \State $P\gets $ all \qctwo in transcript \Comment{including \qctwo in \precommit message and \hqc in \nv message}\label{alg:hotstuffa-2}
    \Upon{$\lr{\conflictacross, e, v, e'}$ from a client}
        \For{$qc\in P$}
            \If{$(qc.v\neq v)\land (qc.e\in (e,e'])\land (qc.\eqc\le e)$} 
                \State send $\lr{\proofacross, qc}$ to the client\label{alg:hotstuffa-12}
            \EndIf
        \EndFor
    \EndUpon
\EndAs{}


\As{a client}
    \Upon{two conflicting \reply messages}
        \If{ two messages are from different views}\label{hotstuffa:28}
            \State $\lr{\reply,e,v,\sigma}\gets$ the message from lower view
            \State  $e'\gets$ the view number of message from higher view
            \State broadcast $\lr{\conflictacross, e, v, e'}$ \label{alg:hotstuffa-23}
            
            \State wait for  $\lr{\proofacross, qc}$ s.t.
            \begin{enumerate}[leftmargin=1in]
                \item[(1)] $e<qc.e\le e'$, and\label{alg:hotstuffa-24}
                \item[(2)] $(qc.v\neq v)\land (qc.\eqc\le e)$
            \end{enumerate}
            \State \textbf{output} $qc.\sigma \cap \sigma$\label{alg:hotstuffa-26}
        \Else \label{alg:hotstuffa-28}
            \State $\lr{\reply,e,v,\sigma}\gets$ first \reply message
            \State $\lr{\reply,e,v',\sigma'}\gets$ second \reply message
            \State \textbf{output} $\sigma \cap \sigma'$
        \EndIf
    \EndUpon
\EndAs{}
\end{algorithmic}
\caption{Forensic protocol for \hsa}
\label{alg:fa-hotstuff-a}
\end{algorithm}


\begin{algorithm}[htbp]
\begin{algorithmic}[1]
\As{a replica running \hsb}
    \State $P\gets $ all \qctwo in transcript\label{alg:hotstuffb-2}
    \State $Q\gets $ all \nv messages in transcript\label{alg:hotstuffb-3}
    \Upon{$\lr{\conflictacross, e, v, e'}$ from a client}
        \For{$qc\in P$}
            \If{$(qc.v\neq v)\land (qc.e\in (e,e'])$} 
                \State send $\lr{\proofacross, qc}$ to the client\label{alg:hotstuffb-12}
            \EndIf
        \EndFor
        \For{$m \in Q$}
            \If{$(m.v\neq v)\land(m.e\in (e,e'])\land(m.\hqc.e \le e)$} 
                \State send $\lr{\nv, m}$ to the client\label{alg:hotstuffb-13}
            \EndIf
        \EndFor
    \EndUpon
\EndAs{}

\As{a client}
    \State $NV\gets \{\}$
    \Upon{two conflicting \reply messages}
        \If{ two messages are from different views}\label{hotstuffb:28}
            \State $\lr{\reply,e,v,\sigma}\gets$ the message from lower view
            \State $e'\gets$ the view number of message from higher view
            \State broadcast $\lr{\conflictacross, e, v, e'}$ \label{alg:hotstuffb-23}
            \Upon{$\lr{\nv, m}$}
                \If{$(m.v\neq v)\land(m.e\in (e,e'])\land(m.\hqc.e \le e)$} 
                    \State $NV\gets NV\cup \{m\}$
                \EndIf
            \EndUpon
            \State wait for  $\lr{\proofacross, qc}$ s.t.
            \begin{enumerate}[leftmargin=1in]
                \item[(1)] $e<qc.e\le e'$, and\label{alg:hotstuffb-24}
                \item[(2)] $(qc.v\neq v)\land  (\exists m\in NV, \text{Hash}(m) = qc.hash)$
            \end{enumerate}
            \State \textbf{output} $qc.\sigma \cap \sigma$\label{alg:hotstuffb-26}
        \Else \label{alg:hotstuffb-28}
            \State $\lr{\reply,e,v,\sigma}\gets$ first \reply message
            \State $\lr{\reply,e,v',\sigma'}\gets$ second \reply message
            \State \textbf{output} $\sigma \cap \sigma'$
        \EndIf
    \EndUpon
\EndAs{}
\end{algorithmic}
\caption{Forensic protocol for \hsb}
\label{alg:fa-hotstuff-b}
\end{algorithm}

\myparagraph{Forensic protocol for \hsa.}
Algorithm~\ref{alg:fa-hotstuff-a} describes the protocol to obtain forensic support atop \hsa. A complete description of the general HotStuff protocol is also provided in Algorithm~\ref{alg:single-hotstuff-modified}. Each replica keeps all received messages as transcript and maintains a set $P$ containing all received \qctwo from \precommit messages and \hqc from \nv messages (line~\ref{alg:hotstuffa-2}). If a client observes outputs of two conflicting values in the same view, it can determine the culprits using the two \reply messages (line~\ref{alg:hotstuffa-28}).  Otherwise, the client sends a request to all replicas for a possible proof between two output views $e, e'$ for $e<e'$ (line~\ref{alg:hotstuffa-23}). Each replica looks through the set $P$  for \qctwo formed in views $e<e^\#\le e'$. If there exists a \qctwo whose value is different from the value $v$ output in $e$ and whose $\eqc$ is less than or equal to $e$, it sends a reply with this \qctwo to the client (line~\ref{alg:hotstuffa-12}). The client waits for a \qctwo (line~\ref{alg:hotstuffa-24}) formed between two output views. For \hsa, if it contains a different value from the first output value and an older view number $\eqc < e$, the intersection of this \qctwo and the \qcthree from the \reply message in the lower view proves at least $t+1$ culprits (line~\ref{alg:hotstuffa-26}). 


\myparagraph{Forensic protocol for \hsb.} % \kartik{this is a good candidate to move to appendix.} 
Algorithm~\ref{alg:fa-hotstuff-b} describes the protocol to obtain forensic support atop \hsb, which is similar to the protocol for \hsa. For replicas running \hsb, besides $P$, they also maintains the set $Q$ for received \nv messages (line~\ref{alg:hotstuffb-3}). When receiving a forensic request from clients, replicas look through $P$ for \qctwo formed in views $e<e^\#\le e'$ and send all \qctwo whose values are different from the value $v$ to the client (line~\ref{alg:hotstuffb-12}). Besides, they also look through $Q$ for a \nv message formed in views $e<e^\#\le e'$ and send all \nv proposing a value different from $v$ and containing a \hqc with view number $\le e$ (line~\ref{alg:hotstuffb-13}). For \hsb, when receiving such a \nv for different values, the message will be stored temporarily by the client until a \qctwo for the \nv message with a matching hash is received. The \nv and the \qctwo together form the desired proof; the intersection of the \qctwo and the \qcthree provides at least $t+1$ culprits.


\myparagraph{Forensic proofs.} The following theorems characterize the forensic support capability of \hsa and \hsb. As long as $m\leq 2t$, \hsa can achieve the best possible forensic support (i.e., $k=1$ and $d=t+1$). \hsb can achieve a medium forensic support (i.e., $k=t+1$ and $d=t+1$). Conversely, if $m > 2t$ then no forensic support is possible for both protocols (i.e., $k=n-f$ and $d=0$).

\begin{theorem}
\label{thm:hotstuff_a}
With $n=3t+1$, when $f>t$, if two honest replicas output conflicting values, \hsa provides $(2t,\ 1,\ t+1)$-forensic support. Further $(2t+1, n-f, d)$-forensic support is impossible with $d>0$.
\end{theorem}
\begin{proof}We prove the forward part of the theorem below. The proof of converse (impossibility) is the same as \S\ref{sec:proofoftheorem4.1}.
Suppose two conflicting values $v,\ v'$ are output in views $e$, $e'$ respectively. 

\myparagraph{Case $e=e'$.}

\noindent\underline{Culpability.} The \qcthree of $v$ and \qcthree of $v'$ intersect in $t+1$ replicas. These $t+1$ replicas should be Byzantine since the protocol requires a replica to vote for at most one value in a view. 

\noindent\underline{Witnesses.} Client can obtain a proof based on the two \reply messages, so additional witnesses are not necessary in this case.

\myparagraph{Case $e\neq e'$.}

\noindent\underline{Culpability.}
If $e \neq e'$, then WLOG, suppose $e < e'$. Since $v$ is output in view $e$, it must be the case that $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$. Now consider the first view $e < e^* \leq e'$ in which a higher lock $(v'', e^*)$ is formed where $v''\ne v$ (possibly $v''=v'$). Such a view must exist since $v'$ is output in view $e' > e$ and a lock will be formed in at least view $e'$. For a lock to be formed, a higher \qctwo must be formed too. Consider the first view $e<e^\# \leq e'$ in which the corresponding \qctwo for $v''$ is formed. The leader in $e^\#$ broadcasts the \nv message containing a \hqc on $(v'', e'')$. Since this is the first time a higher \qctwo is formed and there is no higher \qctwo for $v''$ formed between view $e$ and $e^\#$, we have $e''\le e$. The formation of the higher \qctwo indicates that $2t+1$ replicas received the \nv message proposing $v''$ with \hqc on $(v'', e'')$ and consider it a valid proposal, i.e., the view number $e''$ is larger than their locks because the value is different. 

 Recall that the output value $v$ indicates $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$. In this case, the $2t+1$ votes in \qctwo in view $e^\#$ intersect with the $2t+1$ votes in \qcthree in view $e$ at $t+1$ Byzantine replicas. These replicas should be Byzantine because they were locked on the value $v$ in view $e$ and vote for a value $v'' \neq v$ in a higher view $e^\#$ when the \nv message contained a \hqc from a  view $e'' \leq e$. Thus, they have violated the voting rule.

\noindent\underline{Witnesses.} Client can obtain a proof by storing a \qctwo formed between $e$ and $e'$, whose value is different from $v$ and whose $\eqc \le e$. So only one witness is needed ($k=1)$, the \qctwo and the first \qcthree act as the irrefutable proof.
\end{proof}

\begin{theorem}
\label{thm:hotstuff_b}
With $n=3t+1$, when $f>t$, if two honest replicas output conflicting values, \hsb provides $(2t,\ t+1,\ t+1)$-forensic support. Further $(2t+1, n-f, d)$-forensic support is impossible with $d>0$. 
\end{theorem}

\begin{proof}We prove the forward part of the theorem below. The proof of converse (impossibility) is the same as \S\ref{sec:proofoftheorem4.1}. Suppose two conflicting values $v,\ v'$ are output in views $e$, $e'$ respectively.

\myparagraph{Case $e=e'$.}
Same as Theorem~\ref{thm:hotstuff_a}.

\myparagraph{Case $e\neq e'$.}

\noindent\underline{Culpability.} 
Same as Theorem~\ref{thm:hotstuff_a}. 


\noindent\underline{Witnesses.}
Since \qctwo of \hsb only has the hash of \hqc, the irrefutable proof contains the \nv message that includes the \hqc and the corresponding \qctwo with the matching hash $\text{Hash}(\hqc)$. The client may need to store all \nv messages between $e$ and $e'$ whose value is different from $v$ and the whose $\hqc$ is formed in $\eqc \le e$, until receiving a \qctwo for some \nv message with a matching hash. In the best case, some replica sends both the \nv message and the corresponding \qctwo so the client only needs to store $k=1$ replica's transcript. In the worst case, we can prove that any $t+1$ messages of transcript are enough to get the proof. Consider the honest replicas who receive the first \qctwo and the \nv message. $2t+1$ replicas have access to the \qctwo and $2t+1$ replicas have access to the \nv message. Among them at least $t+1$ replicas have access to both messages, and we assume they are all Byzantine. Then at least $t$ honest replicas have the \qctwo and at least $t$ honest replicas have the \nv message. The total number of honest replicas $n-f \le 2t$. Thus among any $t+1$ honest replicas, at least one have \nv message and at least one have \qctwo. Therefore, $t+1$ transcripts from honest replicas ensure the access of both \nv message and \qctwo and thus guarantee the irrefutable proof. 

%formed in $e^*$, there are two possible cases: 1) If a \qcthree is also formed in $e^*$, then there are $2t+1$ replicas who receive \qctwo in $e^*$; 2) If no \qcprecom is formed $e^*$, there must exist a later view $e^{\#\#}$ where a higher \qctwo for $v''$ is formed, $2t+1$ replicas in this view receive the \nv message (containing the \hqc formed in $e^\#$). In both scenarios, there are at least $2t+1-f$ honest replicas who have received the first higher \qctwo, and in the worst case assume their messages are the last messages the client receives. Before hearing from those honest replicas, other honest replicas may send different \nv messages which also contain \hqc formed in some views $<e$. But the client can not determine which view of these \nv messages forms a higher \qctwo. Thus, the client needs to store $(n-f)-(2t+1-f)+1 = t+1$ messages of transcript to obtain a culpability proof containing the \nv message, \qctwo and the first \qcthree. 
\end{proof}

\myparagraph{Communication complexity.} In line~\ref{alg:hotstuffa-24} of Algorithm~\ref{alg:fa-hotstuff-a}, the client needs to receive one message from $k=1$ replica and the message size is $(|v|+|sig|)$ where $|v|$ and $|sig|$ stand for the size of a value and an aggregate signature. Therefore the complexity of the client receiving messages is $O(|v|+|sig|)$ for \hsa. As for \hsb, theorem~\ref{thm:hotstuff_b} shows that in the worst case, the client needs to receive messages from $k=t+1$ replicas. Each of those replicas sends one message of size $O(|v|+|sig|+|hash|)$ where $|hash|$ stands for the size of a hash value. Therefore the complexity of the client receiving messages is $O(n(|v|+|sig|+|hash|))$ for \hsb.

\subsection{Impossibility for \hsc}
Compared to the other two variants, in \hsc, \vone message and \qctwo are not linked to the \nv message. We show that this lack of information is sufficient to guarantee impossibility of forensics.
%Therefore, unlike \hsa or \hsb, given a \qctwo, there is no way to make sure it is in the first view higher than a view $e$ where a \qctwo is formed. Byzantine replicas may not respond or send a later \qctwo to the client and potentially avoid detection. % and make the client think it is the first \qctwo, such that they can avoid detection. 
% We discuss the intuition and formal theorem related to the impossibility below.

\myparagraph{Intuition.}
When $f=t+1$, from the forensic protocols of \hsa and \hsb, we know that given across-view $\qcthree_1$ and $\qcthree_2$ (ordered by view) and the first \qctwo higher than $\qcthree_1$, the intersection of \qctwo and $\qcthree_1$ contains at least $d=t+1$ Byzantine replicas. The intersection argument remains true for \hsc, however, it is impossible for a client to decide whether \qctwo is the first one only with the transcripts sent by $2t$ honest replicas (when $f=t+1$). In an execution where there are two \qctwo in view $e^*$ and $e'$ respectively ($e^*<e'$), % so that the \qctwo in view $e^*$ is the first one. 
the Byzantine replicas (say, set $P$) may not respond with the \qctwo in $e^*$. The lack of information disallows a client from separating this world from another world $P$ is indeed honest and sharing all the information available to them.  We formalize this intuition in the theorem below. % where these parties  and send the simulated transcripts (as if they are honest replicas in another execution) to the client so that a client may think \qctwo in $e'$ is the first one, and uses it to compute the intersection, holds wrong replicas as culpable, and misses Byzantine replicas. We formalize this intuition in the theorem below.

\begin{theorem}
With $n=3t+1$, when $f>t$, if two honest replicas output conflicting values, $(t+1,\ 2t,\ d)$-forensic support is impossible with $d>1$ for \hsc.
 Further, $(t+2,\ n-f,\ d)$-forensic support is impossible with $d>0$.
\label{thm:hotstuff-null}
\end{theorem}
The theorem is proved in \S\ref{proof:hotstuff-null}.
\ignore{
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/null1.pdf}
    \caption{World~1. TODO: explain who are P Q R etc. and red means Byzantine.}
    \label{fig:hotstuff-null-1}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/null2.pdf}
    \caption{World~2. TODO: explain who are P Q R etc. and red means Byzantine.}
    \label{fig:hotstuff-null-2}
\end{figure}
}
% \begin{table}[!htb]
% \caption{World~1. ``$\Leftarrow$'' means receive and ``$\Rightarrow$'' means send.}
% \label{tab:pf-hotstuff-v3-1}
% \begin{footnotesize}
% \begin{tabular}{|c|c|c|c|}\hline
%   & View $e$ & View $e^*$ & View $e'$ \\\hline
% $P$ &
%   \makecell{$\Rightarrow$\commit on $v$,\\form $\qcthree_1$} &
%   &
%   \\\hline
% \color{red}{$R\cup\{x\}$} &
% \makecell{$\Rightarrow$\commit on $v$,\\form $\qcthree_1$} &&
% \makecell{$\Leftarrow v'$ with $\qctwo_{old}$\\$\Rightarrow$ \vone on $v'$\\$\Leftarrow\qctwo$ on $v'$\\$\Rightarrow$ \precommit on $v'$\\$\Leftarrow$ \qcprecom on $v'$\\$\Rightarrow$ \commit on $v'$\\ form $\qcthree_2$}\\\hline
% $Q$ &&
% \makecell{$\Leftarrow v'$ with $\qctwo_{old}$\\$\Rightarrow$ \vone on $v'$}&
% same as above\\\hline
% \end{tabular}
% \end{footnotesize}
% \end{table}

% \begin{table}[!htb]
% \caption{World~2. ``$\Leftarrow$'' means receive and ``$\Rightarrow$'' means send.}
% \label{tab:pf-hotstuff-v3-2}
% \begin{footnotesize}
% \begin{tabular}{|c|c|c|c|}\hline
%   & View $e$ & View $e^*$ & View $e'$ \\\hline
% %$P-\{x\}$ &
% %  \makecell{$\Rightarrow$\commit on $v$,\\form $\qcthree_1$} &
% %   &
% %  \\\hline
% \color{red}{$P$} &
% \makecell{$\Rightarrow$\commit on $v$,\\form $\qcthree_1$} &
% \makecell{$\Leftarrow v'$ with $\qctwo_{old}$\\$\Rightarrow$ \vone on $v'$\\form $\qctwo^*$}&\\\hline
% $R$ & 
% \makecell{$\Rightarrow$\commit on $v$,\\form $\qcthree_1$}  & 
% &
% \makecell{$\Leftarrow v'$ with $\qctwo^*$\\$\Rightarrow$ \vone on $v'$\\$\Leftarrow\qctwo$ on $v'$\\$\Rightarrow$ \precommit on $v'$\\$\Leftarrow$ \qcprecom on $v'$\\$\Rightarrow$ \commit on $v'$\\ form $\qcthree_2$}\\\hline
% \color{red}{$x$} &
% \makecell{$\Rightarrow$\commit on $v$,\\form $\qcthree_1$} &
% \makecell{$\Leftarrow v'$ with $\qctwo_{old}$\\$\Rightarrow$ \vone on $v'$\\form $\qctwo^*$}&
% \makecell{$\Leftarrow v'$ with $\qctwo_{old}$\\then same as above}\\\hline
% $Q$ &&
% \makecell{$\Leftarrow v'$ with $\qctwo_{old}$\\$\Rightarrow$ \vone on $v'$\\form $\qctwo^*$}&
% same as above\\\hline
% \end{tabular}
% \end{footnotesize}
% \end{table}

% \begin{table}[!htb]
% \caption{World 3. ``$\Leftarrow$'' means receive and ``$\Rightarrow$'' means send. \gerui{TODO: didn't add to the proof yet}}
% \label{tab:pf-hotstuff-v3-3}
% \begin{footnotesize}
% \begin{tabular}{|c|c|c|c|}\hline
%   & View $e$ & View $e^*$ & View $e'$ \\\hline
% %$P-\{x\}$ &
% %  \makecell{$\Rightarrow$\commit on $v$,\\form $\qcthree_1$} &
% %   &
% %  \\\hline
% \color{red}{$P$} &
% \makecell{$\Rightarrow$\commit on $v$,\\form $\qcthree_1$} &
% \makecell{$\Leftarrow v'$ with $\qctwo_{old}$\\$\Rightarrow$ \vone on $v'$\\form $\qctwo^*$}&\\\hline
% $R-y+x$ & 
% \makecell{$\Rightarrow$\commit on $v$,\\form $\qcthree_1$}  & 
% &
% \makecell{$\Leftarrow v'$ with $\qctwo^*$\\$\Rightarrow$ \vone on $v'$\\$\Leftarrow\qctwo$ on $v'$\\$\Rightarrow$ \precommit on $v'$\\$\Leftarrow$ \qcprecom on $v'$\\$\Rightarrow$ \commit on $v'$\\ form $\qcthree_2$}\\\hline
% \color{red}{$y\in R$} &
% \makecell{$\Rightarrow$\commit on $v$,\\form $\qcthree_1$} &
% \makecell{$\Leftarrow v'$ with $\qctwo_{old}$\\$\Rightarrow$ \vone on $v'$\\form $\qctwo^*$}&
% \makecell{$\Leftarrow v'$ with $\qctwo_{old}$\\then same as above}\\\hline
% $Q$ &&
% \makecell{$\Leftarrow v'$ with $\qctwo_{old}$\\$\Rightarrow$ \vone on $v'$\\form $\qctwo^*$}&
% same as above\\\hline
% \end{tabular}
% \end{footnotesize}
% \end{table}

\ignore{
\begin{proof}
Suppose the protocol provides forensic support to detect $d>1$ Byzantine replicas with irrefutable proof and the proof can be constructed from the transcripts of all honest replicas.  To prove this result, we construct two worlds where a different set of replicas are Byzantine in each world. We will fix the number of Byzantine replicas $f=t+1$, but the following argument works for any $f\ge t+1$.

Let there be four replica partitions $P,Q,R,\{x\}$. $|Q|=|P|=|R|=t$, and $x$ is an individual replica. In both worlds, the conflicting outputs are presented in view $e,e'$ ($e+1<e'$) respectively. Let $\qcthree_1$ be on value $v$ in view $e$, and signed by $P,R,x$. And let $\qcthree_2$ (and a \qcprecom) be on value $v'$ in view $e'$, and signed by $Q,R,x$. Suppose the leader of view $e,e^*,e'$ ($e<e^*<e'$) is replica $x$.

\myparagraph{World~1} is presented in Figure~\ref{fig:hotstuff-null-1}. % Let $R$ and $x$ be Byzantine replicas in this world, and they sign \qctwo on $v'$ in $e'$ with $Q$, which is in the first view $>e$. In view $e^*$, the leader proposes value $v'$ and $Q$ sends \prepare on it, but it doesn't form a \qctwo. % \kartik{Write this as: 
Let $R$ and $x$ be Byzantine replicas in this world. In view $e^*$, the leader proposes value $v'$ and $Q$ sends \prepare on it, but a \qctwo is not formed. In view $e'$, the Byzantine parties, together with $Q$, sign \qctwo on $v'$. $e'$ is the first view where a \qctwo for $v'$ is formed.

During the forensic protocol, all honest replicas in $P$ and $Q$ send their transcripts. Byzantine $R$ and $x$ do not provide any information. Since the protocol has forensic support, the forensic protocol can output $d > 1$ replicas in $R$ and $x$ as culprits. 


\myparagraph{World~2} is presented in Figure~\ref{fig:hotstuff-null-2}. % Let $P$ and $x$ be Byzantine replicas in this world, and they sign the first \qctwo on $v'$ in $e^*$ with $Q$, which is the first view $> e$. \kartik{
Let $P$ and $x$ be Byzantine replicas in this world. Here, in view $e^* > e$, $P$ and $x$, together with $Q$ sign \qctwo on $v'$. In this world, $e^*$ is the first view where a \qctwo for $v'$ is formed. View $e' > e^*$ is similar to that of World~1 except that honest $R$ receives a \nv message with $\qctwo^*$ (rather than $\qctwo_{old}$).

During the forensic protocol, $Q$ sends their transcripts, which are identical to those in World~1. Byzantine $P$ can provide the same transcripts as those in World~1. Observe that the transcripts from $P$ and $Q$ presented to the forensic protocol are identical to those in World~1. Thus, the forensic protocol can also outputs $d>1$ replicas in $R$ and $x$ as culpable. In World~2, this is incorrect since replicas in $R$ are honest. 

Based on $2t$ transcripts, World~1 and World~2 are indistinguishable. To obtain an irrefutable proof of $d>1$ culprits, the client needs to collect more than $2t$ transcripts, more than the number of honest parties available. This completes the proof. % However, Byzantine replicas can always choose to stay silent during the forensic protocol and honest replicas can provide at most $2t$ transcripts. This complete the proof.}
\end{proof}

\paragraph{Remark.} The above proof can be easily modified to work with parameters $d > 0$ when $m = t+2$.
}
% \peiyao{add a remark say t+2 -> d>0; t+1 we can identify one}

%\subsection{Chained HotStuff}

%The aforementioned three variants of HotStuff are described under the Byzantine agreement setting to get consensus on a single value. The leader proposes a single value and waits for the replicas' votes to form quorum certificates. When the value is not large, it can be directly included in the vote message without violating the efficiency (as is show in Table~\ref{tab:ba_chain}, $v$ is contained in the \prepare message). In this setting, once a replica receives the \qcthree for the value, it will output the value and send reply to the clients, even if the \qcthree is the only message it receives in the current view. So when two honest replicas output conflicting values, it is possible that the client receives only the commit messages and extra information is needed. And when $m > 2f$, Byzantine replicas are able to form QCs by themselves so that no other honest replicas can get access to the first \qctwo. So the bound on $m$ for \hsa and \hsb is $2t$ and $k>0$.

%However, the setting is slightly different in practice, when the value $v$ is no longer a single value, but actually a block with more fields or a list of transactions/commands, e.g. chained HotStuff \cite[Algorithm~3]{yin2019hotstuff} and other blockchains. Taking single-shot chained HotStuff as an example, a block includes the command (value) and the \hqc. In this case, the block can not be directly included in a vote message, replicas will compute the hash of the block and vote (as is show in Table~\ref{tab:ba_chain}, $Hash(b=(v, \hqc))$ is contained in the \prepare message). And since only the \nv message has the block's preimage, replicas can not vote/output until receiving the original blocks. So when two honest replicas output conflicting values, client can get the full blockchain from one of them ($k=1$) and all \qctwo are part of the blocks. In this case, even if $m > 2t$ the client can still get forensic support.



==> [CCS21] BFT Protocol Forensics/6_algorand.tex <==
\section{Forensic Support for Algorand}
\label{sec:algorand}
Algorand~\cite{chen2019algorand} is a synchronous consensus protocol which tolerates up to one-third fraction of Byzantine users. At its core, it uses a BFT protocol from \cite{micali2018byzantine,chen2018algorand}. However, Algorand runs the protocol by selecting a small set of replicas, referred to as the committee, thereby achieving consensus with sub-quadratic communication. %  Algorand achieves consensus with sub-quadratic communication; it selects a small set of replicas, referred to as the committee, to participate in each step of the protocol. 
The protocol is also player replaceable, i.e., different steps of the protocol have different committees, thus tolerating an adaptive adversary. Each replica uses {\it cryptographic self-selection} using a verifiable random function (VRF)~\cite{micali1999verifiable} to privately decide whether it is selected in a committee. The VRF is known only to the replica until it has sent a message to other parties thus revealing and proving its selection in the committee. In this section, we present an overview of the BFT protocol and then show why it is impossible to achieve forensic support for this protocol. 
%\gerui{Looking ahead, Algorand allows the absence of messages in a synchronous step to switch state of honest parties, and Byzantine parties can utilize this to launch an attack without leaving a trail.}
% \kartik{Talk about identifying only bad committee members?} % until after it has sent some message revealing its selection result. \gerui{Maybe delete this sentence since it may not be true.}Looking ahead, the use of synchrony and self-selection makes it difficult to provide forensic support.\kartik{is this true? They play a role, but the fact that the underlying protocol makes decisions based on absence of messages is what makes it hard.}

\subsection{Overview}
We start with an overview of the single-shot version of Algorand~\cite{chen2019algorand}. The protocol assumes synchronous communication, where messages are delivered within a known bounded time. The protocol proceeds in consecutive steps, each of which lasts for a fixed amount of time that guarantees message delivery. Each step has a self-selected committee, and a replica can compute its VRF, a value that decides whether it is selected in the committee, and it is known only by the replica itself until it has sent the value. All messages sent by a committee member is accompanied by a VRF thus allowing other replicas to verify its inclusion in the committee. Parameters such as committee size $\kappa$ are chosen such that the number of honest parties in the committee is greater than a threshold $t_H \geq 2\kappa/3$ with overwhelming probability. % \kartik{Write this as the following. We provide an overview of the protocol from [cite, section]. The protocol is divided into two sub-protocols: \gradedconsensus and \bba. \gradedconsensus, which forms the first four steps of the protocol, allows us to ... Subsequently, the replicas engage in a \bba protocol to determine ... }
%We provide an overview of the protocol from \cite{chen2019algorand}. 

The BFT protocol is divided into two sub-protocols: \gradedconsensus and \bba. In \gradedconsensus, which forms the first three steps of the protocol, each replica $r$ inputs its value $v_r$. Each replica $r$ outputs a tuple containing a value $v^{\text{out}}_r$ and a grade $g_r$. In an execution where all replicas start with the same input $v$, $v^{\text{out}}_r = v$ and $g_r = 2$ for all replicas $r$. 
The replicas then enter the next sub-protocol, denoted \bba. If $g_r = 2$, replica $r$ inputs value $b_r = 0$, otherwise it inputs $b_r = 1$. At the end of \bba, the replicas agree on the tuple $(0, v)$ or $(1, v_\perp)$.\footnote{$v_\perp$ is considered external valid in Algorand.} The \bba sub-protocol also uses a random coin; for simplicity, we assume access to an ideal global random coin. Our forensic analysis in the next section only depends on \bba and thus, we only provide an overview for \bba here. The protocol proceeds in the following steps,

\begin{itemize}
    \item Steps 1-3 are \gradedconsensus. At the end of \gradedconsensus, each replica inputs a value $v_r$ and a binary value $b_r$ to \bba. % $b=0$ iff $v\neq v_\perp$ and $b=1$ iff $v=v_\perp$ where $v_\perp$ is a default ``empty'' value.
    \item Step 4. Each replica in the committee broadcasts its vote for $(b_r, v_r)$ along with its VRF.
    \item Step $s$ ($s \geq 5, s \equiv 2 \mod 3$) is the \coinfixtozero step of \bba. In this step, a replica checks {\it Ending Condition 0}: if it has received $\ge t_H$ valid votes on $(b,v)$ from the previous step, where $b=0$, it outputs $(b,v)$ and ends its execution. Otherwise, it updates $b_r$ as follows: 
    \[b_r\gets \left\{\begin{array}{lc}
         1,& \text{if}\ge t_H\text{ votes on $b=1$} \\
         0,& \text{otherwise}
    \end{array}\right.\]
    If the replica is in the committee based on its VRF, it broadcasts its vote for $(b_r,v_r)$ along with the VRF.
    \item Step $s$ ($s \geq 6, s \equiv 0 \mod 3$). Symmetric to the previous step but for bit $1$ instead of $0$. Also, the votes need not be for the same $v$ in the ending condition. 
    \item Steps $s$ ($s\ge7, s\equiv 1\mod 3$) is the \coingenuinelyflipped step of \bba. In this step, it updates its variable $b_r$ as follows:
    \[b_r\gets \left\{\begin{array}{l}
         0, \text{if}\ge t_H\text{ votes on $b=0$} \\
         1, \text{if}\ge t_H\text{ votes on $b=1$} \\
         \text{random coin of step }s,\quad \text{otherwise}
    \end{array}\right.\]
    If the replica is in the committee based on its VRF, it broadcasts its vote for $(b_r,v_r)$ along with the VRF.
\end{itemize}

%binary value $b$ and a multi-value $v$. as their inputs to \bba. Subsequently, the replicas engage in \bba, a binary Byzantine agreement protocol to reach agreement on the tuple $(b,v)$. \bba uses a random coin at some steps, and for simplicity we assume there is a magic random coin that appears in the sky for each step. The steps of the whole Algorand protocol are as follows:
%The first four steps of the protocol are the \gradedconsensus sub-protocol and steps starting from step 4 \kartik{you mean step 5? first 4 are for graded consensus.} are the binary Byzantine agreement sub-protocol, referred to as \bba. We assume \gradedconsensus works in good condition, \kartik{what does good condition mean?} and focus on the safety violation and forensics of \bba. In \bba, replicas reach agreement on a tuple $(b,v)$ where $b$ is a binary value and $v$ is a multi-value. \bba uses a random coin at some steps, and for simplicity we assume there is a magic random coin that appears in the sky for each step, since its implementation is irrelevant to forensics. The output of \gradedconsensus and details of \bba are as follows:
\ignore{
\begin{itemize}
    \item[-] Steps 1-4\gerui{3.5} are \gradedconsensus. The output of \gradedconsensus is that each replica has a value $v$ and a binary value $b$, which are the starting values for \bba. $b=0$ iff $v\neq v_\perp$ and $b=1$ iff $v=v_\perp$ where $v_\perp$ is a default ``empty'' value.
    \item[-] Step 4 (after \gradedconsensus) is the start of \bba. At step 4, after each replica in the committee has obtained tuple $(b,v)$ from \gradedconsensus, it broadcasts its vote for $(b,v)$.
    \item[-] Steps $s$ ($s\ge5, s\equiv 2\mod 3$) are \coinfixtozero step of \bba. In this step, a replica checks {\it Ending Condition 0}:\kartik{perhaps can explain terminating condition here}\gerui{done} if it has received $\ge t_H$ valid votes on $(b,v)$ from the previous step, where $b=0$ and the head of $v$ has been received in \gradedconsensus, it outputs $(b,v)$ and ends its execution. (The latter condition of the head of $v$ is irrelevant to forensics, so we will not mention it hereafter.) If it shouldn't end, it updates its variable $b$ according to the number of valid votes it has received from the previous step. It is as follows:
    \[b\gets \left\{\begin{array}{lc}
         1,& \text{if}\ge t_H\text{ votes on $b=1$ and the same $v$} \\
         0,& \text{otherwise}
    \end{array}\right.\]
    If the replica is in the committee based on its VRF, it broadcasts its vote for $(b,v)$ along with the VRF.
    \item[-] Steps $s$ ($s\ge6, s\equiv 0\mod 3$) are \coinfixtoone step of \bba. \kartik{just say symmetric to the previous step?}\gerui{This step is symmetric to \coinfixtozero step, where it may output $(b=1,v=v_\perp)$ by {\it Ending Condition 1}, or it may update $b$ as follows:}% If it shouldn't end, it updates its variable $b$ according to the number of valid votes it has received from the previous step. It is as follows:
    \[b\gets \left\{\begin{array}{lc}
         0,& \text{if}\ge t_H\text{ votes on $b=0$} \\
         1,& \text{otherwise}
    \end{array}\right.\]
    If the replica is in the committee based on its VRF, it broadcasts its vote for $(b,v)$ along with the VRF.
    \item[-] Steps $s$ ($s\ge7, s\equiv 1\mod 3$) are \coingenuinelyflipped step of \bba. In this step, it updates its variable $b$ as follows:
    \[b\gets \left\{\begin{array}{l}
         0, \text{if}\ge t_H\text{ votes on $b=0$ and the same $v$} \\
         1, \text{if}\ge t_H\text{ votes on $b=1$} \\
         \text{magic coin of step }s,\quad \text{otherwise}
    \end{array}\right.\]
    If the replica is in the committee based on its VRF, it broadcasts its vote for $(b,v)$ along with the VRF.
    %\item[-] Ending Condition 0. In a \coinfixtozero step, if a replica has received $\ge t_H$ valid votes on $(b,v)$ from the previous step, where $b=0$ and the head of $v$ has been received in \gradedconsensus, it outputs $(b,v)$ and ends its execution. Notice the latter condition of the head of $v$ is irrelevant to forensics, so we will not mention it hereafter. \gerui{Without loss of generality, assume a replica that has ended execution with this condition to vote for its output $(b,v)$ for all subsequent steps.}\kartik{did not understand this statement}
    %\item[-] Ending Condition 1. \kartik{remove this after ending condition 0 is inlined.} In a \coinfixtoone step, if a replica has received $\ge t_H$ valid votes on $(b,v)$ from the previous step, where $b=1$, it stops its execution and outputs $(b,v_\perp)$ where $v_\perp$ is a default value, and ends its execution. \gerui{Without loss of generality, assume a replica that has ended execution with this condition to vote for its output $(b,v_\perp)$ for all subsequent steps.}
    %\item[-] \gerui{Without loss of generality, if in any step, the number of valid votes is less than $t_H$, which means the honest committee members of the previous step is less than the threshold $t_H$, a replica ends without output since this scenario violates the assumption of honest-majority-of-user or synchrony.}\kartik{does algorand say this?}\gerui{no, original algorand doesn't say this. we can delete this.}
\end{itemize}
}

\myparagraph{Safety of \bba within a step.} If all honest replicas reach an agreement before any step, the agreement will hold after the step. If the agreement is on binary value 0 (1 resp.) then the opposite Ending Condition 1 (0 resp.) will not be satisfied during the step. This is because synchronous communication ensures the delivery of at least $t_H$ votes on the agreed value and there are not enough malicious votes on the other value. 

\myparagraph{Safety of \bba across steps.} For the step \coinfixtozero (1 resp.), if any honest replica ends due to Ending Condition 0 (1 resp.), all honest replicas will agree on binary value 0 and value $v$ (1 and $v_\perp$ resp.) at the end of the step, because there could only be less than $t_H$ votes on binary value 1 (0 resp.). Hence, together with safety within a step, binary value 1 and value $v_\perp$ (0 and $v$ resp.) will never be output.

\ignore{
Algorand assumes honest-majority-of-user, which ensures $f$ Byzantine members of any committee out of the $n$ committee members to satisfy the following inequalities with overwhelming probability~\cite{chen2019algorand} \gerui{I cite 2019 paper. what about 2017 paper?}\kartik{both should have the same bound, isn't it?}:
\[n-f>t_H,\text{ and }(n-f)+2f=n+f<2t_H.\]
(Notice that committee members $n$ and Byzantine members $f$ in Algorand are random variables.) 
Denote these inequalities as {\it honest-majority-of-committee}, and it ensures the safety of Algorand as follows.

\myparagraph{Safety of \gradedconsensus.} \gradedconsensus ensures that all honest replicas have the same output value $v$ or a default output value $v_\perp$. Due to {\it honest-majority-of-committee}, Byzantine replicas cannot create two conflicting values $v,v'$ ($v\neq v_\perp, v'\neq v_\perp$) that are honest replicas' output. %As mentioned before, we will not attack \gradedconsensus and assume it works in good condition.

\myparagraph{Safety of \bba within a step.} If all honest replicas reach an agreement before any step, the agreement will hold after the step. If the agreement is on binary value 0 (1 resp.) then the opposite Ending Condition 1 (0 resp.) will not be satisfied during the step. This is because synchronous communication ensures the delivery of at least $t_H$ votes on the agreed value and there is not enough malicious votes on the other value. 

\myparagraph{Safety of \bba across steps.} For the \coinfixtozero (1 resp.) step, if any honest replica ends due to Ending Condition 0 (1 resp.), all honest replicas will agree on binary value 0 and value $v$ (1 and $v_\perp$ resp.) at the end of the step, because there could only be less than $t_H$ votes on binary value 1 (0 resp.). Hence, together with safety within a step, binary value 1 and value $v_\perp$ (0 and $v$ resp.) will never be output.
}

\subsection{Impossibility of Forensics}
When the Byzantine fraction in the system is greater than one-third, with constant probability, a randomly chosen committee of size $\kappa < n$ will have $t_H < 2\kappa/3$. In such a situation, we can have a safety violation. Observe that since only $\kappa < n$ committee members send messages in a round, the number of culpable replicas may be bounded by $O(\kappa)$. However, we will show an execution where no Byzantine replica can be held culpable. % can construct an execution of Algorand with no forensic support. % When the assumption of honest-majority-of-user doesn't hold anymore, the honest-majority-of-committee inequalities don't hold with overwhelming probability. Thus, \gerui{Byzantine replicas can make a violation of agreement, and from there} we can construct an execution of Algorand such that there is no forensic support.

\myparagraph{Intuition.} The safety condition for \bba relies on the following: if some honest replica commits to a value $b$, say $b = 0$, in a step and terminates, then all honest replicas will set $b=0$ as their local value. In all subsequent steps, there will be sufficient ($> 2/3$ fraction) votes for $b=0$ due to which replicas will never set their local value $b=1$. Thus, independently of what Byzantine replicas send during the protocol execution, honest replicas will only commit on $b = 0$. On the other hand, if replicas do not receive $> 2/3$ fraction of votes for $b=0$, they may switch their local value to $b=1$ in the \coinfixtoone or \coingenuinelyflipped step. This can result in a safety violation. When the Byzantine fraction is greater than one-third, after some replicas have committed 0, the Byzantine replicas can achieve the above condition by selectively not sending votes to other replicas (say set $Q$), thereby making them switch their local value to $b=1$. There is no way for an external client to distinguish this world from another world where the set $Q$ is Byzantine and states that it did not receive these votes. We formalize this intuition in the theorem below. Observe that our arguments work for the \bba protocol with or without player-replaceability. %that the argument still holds even without player-replaceability, i.e., if a committee is fixed across rounds instead of selected differently each round.}

% Byzantine replicas can selectively send votes to some replicas and not to some other replicas. As a result, some honest replicas collect enough votes for Ending Condition 0 whereas others collect enough votes for Ending Condition 1. Those who don't receive votes cannot prove it.

\begin{theorem}
When the Byzantine fraction exceeds 1/3, if two honest replicas output conflicting values, $(t+1,\ 2t,\ d)$-forensic support is impossible with $d>0$ for Algorand.
\label{thm:algorand}
\end{theorem}
The theorem is proved in \S\ref{sec:algorand-proof}.
\ignore{
\begin{proof}
We construct two worlds where a different set of replicas are Byzantine in each world. Let replicas be split into three partitions $P$, $Q$, and $R$, and $|P|=(n-2\epsilon)/3,|Q|=|R|=(n+\epsilon)/3$ 
%where $N$\gerui{Is $n,N$ same here?} is the number of replicas 
and $\epsilon>0$ is a small constant. Denote the numbers of replicas from $P,Q,R$ in a committee by $p,q,r$. Let $\kappa$ denote the expected committee size; $t_H=2\kappa/3$. With constant probability, we will have $p < \kappa/3$, $q > \kappa/3$ and $r > \kappa/3$ and $p+q < 2\kappa/3$ in steps 4 to 8. % \kartik{Pramod, do we need to be more formal here?}

\myparagraph{World 1.} Replicas in $R$ are Byzantine in this world. We have $p+q < t_H$ and $q+r > t_H$. The Byzantine parties follow the protocol in \gradedconsensus. Thus, all replicas in step 4 hold the same tuple of $b=0$ and $v$ ($v\neq v_\perp$). Then, the following steps are executed.
\begin{itemize}
    \item[Step 4] Honest committee members that belong to $P$ and $Q$ broadcast their votes on $(b=0,v)$ whereas Byzantine committee members that belong to $R$ send votes to replicas in $P$ and not $Q$. %(Without loss of generality, suppose the honest replicas in committees for the next steps belong to $Q$).
    \item[Step 5] Replicas in $P$ satisfy Ending Condition 0, and output $b=0$ and the value $v$. Replicas in $Q$ do not receive votes from committee members in $R$, so they update $b=0$ and broadcast their votes on $(b=0, v)$. %Honest committee members that belong to $Q$ doesn't receive votes from committee members in $R$, so they update $b=0$ and broadcast their votes on $(b=0,v)$. 
    Byzantine committee members that belong to $R$ pretend not to receive votes from committee members in $Q$, and also update $b=0$. And they send votes to replicas in $P$ and not $Q$.
    \item[Step 6] Replicas in $Q$ update $b=1$ since they receive $p+q<t_H$ votes.  Replicas in $R$ pretend not to receive votes from committee members in $Q$, and also update $b=1$. Committee members in $Q$ and $R$ broadcast their votes.
    \item[Steps 7-8] Committee members that belong to $Q$ and $R$ receive $q+r>t_H$ votes, so they update $b=1$ and broadcast their votes.
    %Since $q+r>2/3 n$, there are more than $2/3 n$ such votes.
    \item[Step9] Replicas in $Q$ and $R$ satisfy Ending Condition 1, and output $b=1$ and $v_\perp$, a disagreement with replicas in $P$.
\end{itemize}
During the forensic protocol, replicas in $P$ send their transcripts and state that they have output $b=0$. $Q$ and $R$ send their transcripts claiming in steps 4 and 5 they do not hear from the other partition, and they state that output $b=1$. %\gerui{$|P|<1/3$, I think ALgorand doesn't care about 1/3 replicas commit a value, right?}\kartik{did not understand this comment.}\gerui{the question is that do we need $b=0$ to be committed by $>1/3$ replicas? I guess no.}

If this protocol has any forensic support, then it should be able to detect some replica in $R$ as Byzantine.

\myparagraph{World 2.} This world is identical to World 1 except (i) Replicas in $Q$ are Byzantine and replicas in $R$ are honest, and (ii) the Byzantine set $Q$ behaves exactly like set $R$ in World~1, i.e., replicas in $Q$ do not send any votes to $R$ in steps 4 and 5 and ignore their votes. % symmetrically to  Let replicas in $Q$ be Byzantine in this world. Similar to world 1, assume \gradedconsensus gives all committee members in step 4 $(b=0,v)$. Next, in steps 4-9, let $Q$ act symmetrically as if they are in world 1: $Q$ don't send to $R$ and ignore votes from $R$ in step 4 and 5. 
During the forensic protocol, $P$ send their transcripts and state that they have output $b=0$. $Q$ and $R$ send their transcripts claiming in steps 4 and 5 they do not hear from the other partition, and they state that output $b=1$. 

From an external client's perspective, World 2 is indistinguishable from World 1. In World~2, the client should detect some replica in $R$ as Byzantine as in World 1, but all replicas in $R$ are honest. % which is a contradiction.
\end{proof}
}
% Therefore, in this execution of world 1 or 2, there is no forensic support.

\ignore{
Suppose honest-majority-of-committee inequalities doesn't hold in steps 4 to 8, that is, suppose $|HSV|<t_H$ and $|HSV|/2+|MSV|\ge t_H$. The following execution can create a safety violation while Byzantine replicas avoid being held accountable. First, assume \gradedconsensus works fine and all committee members in step 4 have $b=0$ and the same $v$ ($v\neq v_\perp$). Let the honest replicas be evenly split into two partitions $P$ and $Q$. Next, the following happens:
\begin{itemize}
    \item[Step4] Honest committee members broadcast their votes whereas Byzantine committee members send votes to replicas in $P$ exclusively and not to $Q$. %(Without loss of generality, suppose the honest replicas in committees for the next steps belong to $Q$).
    \item[Step5] Replicas in $P$ satisfies Ending Condition 0, and output $b=0$ and the value $v$. Honest committee members in $Q$ don't end, and update $b=0$ and broadcast their votes. Byzantine committee members don't send vote, so that the total number of votes is less than $t_H$.
    \item[Step6-8] Committee members not in $P$ update $b=1$ and broadcast their votes. With high probability, honest committee members in $Q$ and Byzantine committee members are beyond $t_H$, hence there are $\ge t_H$ such votes.
    \item[Step9] Replicas in $Q$ satisfy Ending Condition 1, and output $b=1$ and value $v_\perp$.
\end{itemize}

\kartik{need another world to make this claim.} Therefore, a safety violation happens; values $v$ and $v_\perp$ are output by replicas in $P$ and $Q$ respectively. The behavior that causes this safety violation is in step 4 and 5. As for steps 6-9, all replicas (including Byzantine ones) follow the protocol. In step 4, Byzantine replicas selectively send votes whereas in step 5, Byzantine replicas stay silent. If a replica selectively sends votes to some replicas and not to some other replicas, it is difficult to provide irrefutable proof. \gerui{I'm not sure about the previous sentence. may change this sentence wrt definition of irrefutable proof. maybe only its own message can be the proof} If a replica stays silent in a step, it is difficult to provide irrefutable proof as well. Furthermore, it is difficult to identify the replica due to the property of self-selection; no replica other than itself knows it is in the committee. Since the protocol relies on the assumption that at least $t_H$ votes should be delivered in any step, Byzantine replicas being silent can cause a safety violation. %Furthermore, cryptographic self-selection makes it impossible to identify the silent replicas. 
Hence, it is impossible to detect any Byzantine replicas in this execution.
}

==> [CCS21] BFT Protocol Forensics/7_implementation.tex <==
\section{LibraBFT and {\sf Diem}}
\label{sec:impl}
In this paper, we have focused on forensics for single-shot consensus. Chained BFT protocols are natural candidates for consensus on a sequence with applications to  blockchains. LibraBFT is a chained version of Hotstuff and is the core consensus protocol in {\sf Diem}, a new cryptocurrency supported by Facebook~\cite{diem}. In this section, we show that LibraBFT has the strongest forensic support possible (as in Hotstuff-view). Further, we implement the corresponding forensic analysis protocol as a module on top of an open source {\sf Diem} client. We highlight the system innovations of our implementation and associated forensic dashboard; this has served as a reference implementation  presently under active consideration for deployment (due to anonymity imperativs we are unable to document this more concretely). 

\myparagraph{{\sf Diem} blockchain.}
{\sf Diem} Blockchain uses LibraBFT~\cite{librabft}, %\gerui{renamed to DiemBFT} \peiyao{Not sure about this, last time I used {\sf Diem}BFT in the draft and Dahlia revised it to LibraBFT}\pramod{agree with Peiyao. this is what Dahlia told us} 
 a variant of HotStuff protocol for consensus. In LibraBFT, the replicas are called validators, who receive transactions from clients and propose blocks of transactions in a sequence of rounds. 

\myparagraph{LibraBFT forensics.} The culpability analysis for LibraBFT is similar to Theorem~\ref{thm:hotstuff_b}. However, for the witnesses, the blockchain property of LibraBFT makes sure that any replica (validator) has access to the full blockchain and thus provides $(n-2, 1, t+1)$-forensic support. The formal result is below (proof in  \S\ref{sec:proof-diem}).
\begin{theorem}
\label{thm:diem}
For $n=3t+1$, when $f>t$, if two honest replicas output conflicting blocks, LibraBFT provides $(n-2,\ 1,\ t+1)$-forensic support.
\end{theorem}

The aforementioned three variants of HotStuff in \S\ref{sec:basic-hotstuff} are described under the VBA setting to reach consensus on a single value, and the value can be %\kartik{what can be?}\peiyao{the value} 
 directly included in the vote message (cf.\  Table~\ref{tab:ba_chain}, $v$ is contained in the \prepare message). In this setting, once a replica receives the \qcthree for the value, it will output the value and send a reply to the client, even if the \qcthree is the only message it receives in the current view so far. So when two honest replicas output conflicting values, it is possible that the client receives only the commit messages and extra communication is needed. And when $m > 2t$, Byzantine replicas are able to form QCs by themselves so that no other honest replicas can get access to the first \qctwo. Thus the bound on $m$ for \hsa and \hsb is $2t$.

However, the setting is slightly different in practice, when the value $v$ is no longer a single value, but actually a block with more fields and a list of transactions/commands, as in  LibraBFT. In single-shot consensus,   a block includes the transactions (value) and the \hqc. In this case, the block is too heavy to include directly in a vote message, %\gerui{I think "cannot" is not accurate. How about "is not"?} \peiyao{how about: the block is too heavy to be directly included in a vote message, so the replicas will compute the hash...} be directly included in a vote message, but 
so the replicas add the hash of the block  to the vote message (see  Table~\ref{tab:ba_chain}, Hash$(b=(v, \hqc))$ is contained in the \prepare message). And since only the \nv message has the block's preimage, replicas cannot vote/output until receiving the original blocks. Thus when two honest replicas output conflicting values, the client can obtain the full blockchain from one of them ($k=1$) and all \qctwo are part of the blocks. In this case, even if $m > 2t$ the client can still enjoy non-trivial forensic support. %\kartik{we only count replicas who send their full transcripts towards $k$? and that is why, $k=1$ for \hsa too, since the initial two parties showing equivocation do not send their full transcripts?} \peiyao{Yes, sending commitQC is part of the original protocol (along with the \reply message).
 %Only after the client observes a safety violation and sends a request, the forensic part begins. The messages sent and stored during the forensic protocol will be counted into $k$.}


\begin{table}[]
\begin{tabular}{c|c|c}
\toprule
     & \hsb  & LibraBFT  \\ \toprule
\vone                                                       & \begin{tabular}[c]{@{}c@{}}$\lr{\vone, e,v,$ \\ $ \text{Hash}(\hqc)}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\lr{\vone, e, $\\ $\text{Hash}(b=(v, \hqc))}$\end{tabular} \\ \midrule

$k$  & $t+1$    & $1$   \\ \midrule
$m$   & $2t$    & $n-2$     \\ \midrule
\begin{tabular}[c]{@{}c@{}}extra\\ condition\end{tabular} & - & \begin{tabular}[c]{@{}c@{}}must receive the\\ preimage of hash\end{tabular} \\ \bottomrule
\end{tabular}
    \caption{Comparison of \hsb and LibraBFT %\kartik{use the nicer table template}
    }
    \label{tab:ba_chain}
\end{table}





\myparagraph{Forensic module.} Our  prototype consists of two components, a database \fs used to store quorum certificates received by validators, which can be accessed by clients through JSON-RPC requests or consensus API; and an independent \detector run by clients to analyze the forensic information. 
\begin{itemize}
    \item \textbf{\fs} maintains a map from the view number to quorum certificates and its persistent storage. %\gerui{can we change and its persistent storage to "on persistent storage"/"and store it persistently".} 
    It is responsible for storing forensic information and allows access by other components,  % and
    including clients (via JSON-RPC requests or consensus API).  
    \item \textbf{\detector } is run by clients manually to send requests periodically to connected validators. It collates information received from validators, using it as the  input to the forensic analysis protocol.%[TODO: pseudo code for detector]
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/diem.pdf}
    \caption{Forensic module integrated with {\sf Diem}.}
    \label{fig:forensic_store}
\end{figure}

\myparagraph{Testing using Twins~\cite{bano2020twins}.}
To test the correctness of forensic protocols, we build a testbed to simulate Byzantine attacks and construct different types of safety violations. Ideally, for modularity purposes, our testbed should not require us to modify the underlying consensus protocol to obtain Byzantine behavior. We leverage Twins~\cite{bano2020twins}, an approach to emulate Byzantine behaviors by running two instances of a node (i.e. replica) with the same identity. Consider a simple example setting with four nodes (denoted by $node0\sim 3$), where $node0$ and $node1$ are Byzantine so they have twins called $twin0$ and $twin1$. The network is split into two partitions, the first partition $P_1$ includes nodes $\{node0, node1, node2\}$ and the second partition $P_2$ includes nodes $\{twin0, twin1, node3\}$. Nodes in one partition can only receive the messages sent from the same partition. The double voting attack can be simulated when Byzantine leader proposes different valid blocks in the same view, and within each partition, all nodes will vote for the proposed block. The network partition is used to drop all messages sent from a set of nodes. However, it can only help construct the safety violation within the view. To construct more complicated attacks, we further improve the framework and introduce another operation called ``detailed drop'', which drops selected messages with specific types.





\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/demo.pdf}
    \caption{Forensic module dashboard.  }
    \label{fig:demo}
\end{figure*}
\myparagraph{Visualization.} The \detector accepts the registration of different views to get notified once the data is updated. We built  a dashboard to display the  information received by the detector and the analysis results output by the forensic protocol.  Figure~\ref{fig:demo} shows a snapshot of the dashboard   which displays  information about the network topology, hashes of latest blocks received at different validators, conflicting blocks, detected culprit keys and raw logs. Interactions with end-users,  including {\sf Diem} core-devs, has guided our design of the dashboard. 




==> [CCS21] BFT Protocol Forensics/8_Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we have embarked on a systematic study of the forensic properties of BFT protocols, focusing on 4 canonical examples: PBFT (classical), Hotstuff and VABA   (state-of-the-art protocols on partially synchronous and asynchronous network settings) and Algorand (popular protocol that is adaptable to proof of stake blockchains). Our results show that minor variations in the BFT protocols can have outsized impact on their forensic support. 

We exactly characterize  the forensic support of each protocol, parameterized by the triplet $(m,k,d)$.
The forensic support characterizations are remarkably similar across the protocols: if any non-trivial support is possible (i.e., at least one culpable replica can be implicated; $d> 0$), then the largest possible forensic support, $(2t, 1, t+1)$, is also possible; the one exception to this result is the Hotstuff-hash variant. Although the proof of forensic support is conducted for each protocol and its variant individually, we observe common trends: %make the following interesting observations: %there is substantial overlap among the proof ingredients, both in the achievable forensic support as well as the converse (impossibility results):  
\begin{itemize}
    \item For each of the protocols with strong forensic support, as a part of the protocol execution, there exist witnesses who hold signed messages from Byzantine parties indicating that they have not followed some rule in the protocol. % \gerui{The reason that these protocols have strong forensic support is that, in order to create a security breach, Byzantine parties \textit{have to} leave irrefutable evidence (signed messages) that can be used to prove their deviation from the protocol.}
    \item On the other hand, for protocols with no forensic support, the Byzantine parties are able to break safety without  leaving any evidence, although the mechanism to achieve this is different for each of PBFT-MAC, Algorand, and HotStuff-null. With PBFT-MAC, Byzantine parties are able to construct arbitrary transcripts due to the absence of signatures. Hence, message transcripts cannot be used as evidence. With Algorand, they can utilize a rule which relies on the absence of messages (under synchrony) to set an incorrect protocol state without leaving a trail. With HotStuff-null, due to the lack of links between messages across views, Byzantine parties can present fake message transcripts and thus, pretend to be honest. % With PBFT-MAC, the Byzantine parties utilize  the ability to construct arbitrary transcript (due to absence of signatures). With Algorand, they utilize a rule which relies on absence of messages (under synchrony) to set an incorrect protocol state without leaving a trail. With HotStuff-null, \kartik{...}% \pramod{1-2 sentences on commonality of impossibility results}
\end{itemize}
Conceptually, the  burning question is whether these common ingredients can be stitched together to form an overarching theory of   forensic support  for abstract families of secure BFT protocols: First, from an impossibility standpoint, is there a relationship between the need to use synchrony or the absence of PKI in a protocol  and absence of  forensic support? Second, for the positive results, can one  argue strong forensic support for an ``information-complete'' variant of any BFT protocol?  This is an active area of research. %\kartik{Conceptually, there are two burning questions based on these observations. First, from an impossibility standpoint, is there a relationship between the need to use synchrony or the absence of PKI in a protocol directly related to its forensic support? Second, for the positive results, can the common ingredients be stitched together to form an overarching theory of   forensic supports for abstract families of secure BFT protocols? This is an active area of research.}  

From a practical stand point, forensic analysis for existing blockchain protocols is of great interest; our forensic protocol for LibraBFT and its reference implementation has made strong inroads towards practical deployment. However, one shortcoming of the approach  in this paper is that forensic analysis is conducted   only upon {\em fatal} safety breaches. It is of great interest to conduct forensics with other forms of attacks: liveness attacks, censorship, small number of misbehaving replicas that impact performance.  We note that liveness attacks do not  afford, at the outset, undeniable complicity of malicious replicas and an important research direction is in formalizing weaker notions of culpability  proofs (perhaps including assumptions involving external forms of trust). 
This is an active area of research. %\sk{should treat liveness attacks separately (liveness and censorship attacks are not mild). We should state that liveness attacks do not afford the ability to provide unforgeable proof so we want to look at a weaker version of proof, or maybe utilize some external trust assumption. }

==> [CCS21] BFT Protocol Forensics/9-ack.tex <==
\section{Acknowledgement}
This research was partly supported by US Army Research Office Grant W911NF-18-1-0332, National Science Foundation CCF-1705007 and the XDC network. Kartik Nayak was supported in part by Novi and VMware gift research grant.

We thank the {\sf Diem} team for  implementation advice and Jovan Komatovic for helpful discussions about a forensic attack on HotStuff.

==> [CCS21] BFT Protocol Forensics/A_vaba.tex <==
\section{VABA has Strong Forensic Support}
\label{sec:vaba}
Validated Asynchronous Byzantine Agreement (VABA) is a  state-of-the-art protocol~\cite{abraham2019asymptotically} in the asynchronous setting with asymptotically optimal $O(n^2)$ communication complexity and expected $O(1)$ latency for $n \geq 3t+1$. % and borrows the leader-based voting paradigm from HotStuff  adapting it to asynchronous network environments.

\begin{algorithm}[b]
\begin{algorithmic}[1]
\As{a replica running VABA}
    \ForInitialize{$e\ge 1$}
        \For{$j\in[n]$}
        \State $\pflock[e][j]\gets \{\}$
        \State $\coin[e]\gets \{\}$
        \EndFor
    \EndForInitialize
    \Upon{$\lr{i,\nv,e,v,L}$ in view $e$ in \pp instance $i$}
        \State $(e', v', \sigma, \eqc)\gets L $\algorithmiccomment{Note that $L$ has selectors $e,v,\sigma,\eqc$} 
        \State $\pflock[e'][i] \gets  \pflock[e'][i]\cup \{(v', \sigma, \eqc)\}$\label{alg:vaba-6}
    \EndUpon
    \Upon{$\lr{i,\prepare,e,v,\sigma,\eqc}$ in view $e$ in \pp instance $i$}
        \State $\pflock[e][i]\gets \pflock[e][i]\cup \{(v, \sigma,\eqc)\}$\label{alg:vaba-6-2}
    \EndUpon
    \If{$Leader[e]$ is elected}
    \State discard $\pflock[e][j]$ for $j\neq Leader[e]$\label{alg:vaba-12}
    \State $\coin[e]\gets$ inputs to $\threscoin$ for electing $Leader[e]$\label{alg:vaba-13}
    \EndIf
    \Upon{$\lr{\vc,e,\qctwo,$ $\qcprecom,\qcthree}$ in view $e$}
        \State $(e', v', \sigma, \eqc)\gets\qctwo$\algorithmiccomment{Note that \qctwo has selectors $e,v,\sigma,\eqc$} 
        \State $\pflock[e'][Leader[e']]\gets \pflock[e'][Leader[e']]\cup \{(v', \sigma,\eqc)\}$\label{alg:vaba-6-3}
    \EndUpon
    \Upon{$\lr{\requestproofleader, e, e'}$ from a client}
        \For{all $e\le e^*\le e'$}
            \State send $\lr{\coinmsg, e^*, Leader[e^*], \coin[e^*]}$ to client
        \EndFor
    \EndUpon
    \Upon{$\lr{\conflictacross, e, v, \sigma, e'}$ with a collection of $LeaderMsg$ from a client}
        \For{all $e<e^\#\le e'$}
            \If{$Leader[e^\#]$ is not elected yet}
            \State $\lr{\coinmsg, e^\#, leader, \coin}\gets LeaderMsg$ of view $e^\#$
            \State check $leader$ is the leader generated by $\coin$ in view $e^\#$ (otherwise don't reply to the client)
            \State $Leader[e^\#]\gets leader$
            \EndIf
            \For{$qc\in \pflock[e^\#][Leader[e^\#]]$}
            \If{$(qc.v\neq v)\land (qc.\eqc\le e)$}
                \State send $\lr{\proofacross, e^\#, Leader[e^\#], qc}$ to the client%\label{alg:vaba-12}
            \EndIf
            \EndFor
        \EndFor
    \EndUpon
\EndAs{}
\algstore{vaba}
\end{algorithmic}
\caption{Forensic protocol for VABA}
\label{alg:fa-vaba}
\end{algorithm}
\addtocounter{algorithm}{-1}
\begin{algorithm}[htbp]
\begin{algorithmic}[1]
\algrestore{vaba}
\As{a client}
    \Upon{two conflicting \reply messages}
        \State $e \gets$ the view number of \reply  from lower view
        \State $e'\gets$ the view number of \reply  from higher view
        \ForInitialize{all $e\le e^*\le e'$}
            \State $Leader[e^*]\gets \{\}$
            \State $LeaderMsg[e^*]\gets \{\}$
        \EndForInitialize
        \State send $\lr{\requestproofleader, e, e'}$  to the replica of \reply message from higher view\label{alg:vaba-request-proof-leader-1}
        \For{all $e\le e^*\le e'$}
        \State wait for $\lr{\coinmsg, e^*, leader, \coin}$ s.t. $leader$ is the leader generated by $\coin$ in view $e^*$ (otherwise the \reply message is not considered valid)
        \State $Leader[e^*]\gets leader$
        \State $LeaderMsg[e^*]\gets \lr{\coinmsg, e^*, leader, \coin}$
        \EndFor\label{alg:vaba-request-proof-leader-2}
        \If{the two \reply messages are from different views}\label{alg:vaba-28}
            \State $\lr{i,\reply,e,v,\sigma}\gets$ the message from lower view
            \State $\lr{i',\reply,e',v',\sigma'}\gets$ the message from higher view
            \State check $i=Leader[e]$ and $i'=Leader[e']$ (otherwise the \reply message is not considered valid)\label{alg:vaba-verify-leader-1}
            \State broadcast $\lr{\conflictacross, e, v, \sigma, e'}$ with $LeaderMsg[e^*]$ for all $e<e^*\le e'$ 
            \State wait for  $\lr{\proofacross, e^\#,leader, qc}$  s.t.
            \begin{enumerate}[leftmargin=1in]
                \item[(1)] $e<e^\#\le e'$, and
                \item[(2)] $(qc.v\neq v)\land (qc.\eqc\le e)$, and
                \item[(3)] $leader=Leader[e^\#]$\label{alg:vaba-verify-leader-2}% is the leader generated by $\coin$ in view $e^\#$
            \end{enumerate}
            \State \textbf{output} $qc.\sigma \cap \sigma$
        \Else
            \State $\lr{i,\reply,e,v,\sigma}\gets$ first \reply message
            \State $\lr{i',\reply,e,v',\sigma'}\gets$ second \reply message
            \State check $i=i'=Leader[e]$ (otherwise the \reply message is not considered valid)\label{alg:vaba-verify-leader-3}
            \State \textbf{output} $\sigma \cap \sigma'$
        \EndIf\label{alg:vaba-end}
    \EndUpon
\EndAs{}
\end{algorithmic}
\caption{Forensic protocol for VABA}
\label{alg:fa-vaba-second}
\end{algorithm}

\subsection{Overview}
At a high-level, the VABA protocol adapts HotStuff to the asynchronous setting. There are three phases in the protocol:
\begin{itemize}[leftmargin=*, topsep=0pt]
	\item[-] \textbf{Proposal promotion.} In this stage, each of the $n$ replicas run $n$ parallel HotStuff-like instances, where replica $i$ acts as the leader within instance $i$.
    \item[-] \textbf{Leader election.} 
		After finishing the previous stage, replicas run a leader election protocol using a \threscoin primitive \cite{cachin2005random} to randomly elect the leader of this view, denoted as $Leader[e]$ where $e$ is a view number. At the end of the view, replicas adopt the ``progress'' from $Leader[e]$’s proposal promotion instance, and discard values from other instances.
	\item[-] \textbf{View change.} Replicas broadcast quorum certificates from $Leader[e]$’s proposal promotion instance and update local variables and/or output value accordingly.
\end{itemize}

Within a proposal promotion stage, the guarantees provided are the same as that of HotStuff, and hence we do not repeat it here. The leader election phase elects a unique leader at random -- this stage guarantees (i) with $\geq 2/3$ probability, an honest leader is elected, and (ii) an adaptive adversary cannot stall progress (since a leader is elected in hindsight). Finally, in the view-change phase, every replica broadcasts the elected leader's quorum certificates to all replicas.


\subsection{Forensic Support for VABA}
The key difference between forensic support for HotStuff and VABA is the presence of the leader election stage -- every replica/client needs to know \emph{which} replica was elected as the leader in each view. Importantly, the \threscoin  primitive ensures that there is a unique leader elected for each view. % \kartik{check: for simplicity, we should just set the coin threshold to $k = 2t+1$? check Constantinople paper.}\gerui{if $f>t$, unpredictability doesn't hold. but unique (robustness) holds, according to Constantinople paper.} 
Thus, the forensic analysis boils down to performing an analysis similar to the HotStuff protocol, except that the leader of a view is described by the leader election phase.
 
We present the full forensic protocol in Algorithm~\ref{alg:fa-vaba} for completeness. We make the following changes to VABA:
\begin{itemize}
    \item \textbf{Storing information for forensics.} Each replica maintains a list of \emph{ledgers} for all instances, containing all received \qctwo from \prepare messages, \nv messages, and \vc messages (lines~\ref{alg:vaba-6},\ref{alg:vaba-6-2},\ref{alg:vaba-6-3}). When the leader of a view is elected, a replica keeps the \pflock from the leader's instance and discards others (line~\ref{alg:vaba-12}). A replica also stores the random coins from the leader election phase for client verification (line~\ref{alg:vaba-13}).
    \item \textbf{Bringing proposal promotion closer to \hsa.} There are minor differences in the proposal promotion phase of VABA~\cite{abraham2019asymptotically} to the description in HotStuff (\S\ref{sec:basic-hotstuff}). We make this phase similar to that in the description of our HotStuff protocol with forensic support. In particular: (i) the $LOCK$ variable stores both the view number and the value (denoted by $LOCK.e$ and $LOCK.v$), (ii) the voting rule in a proposal promotion phase is: vote if $KEY$ has view and value equal to $LOCK$, except when $KEY$'s view is strictly higher than $LOCK.e$, (iii) assume a replica's own \vc message arrives first so that others' \vc messages do not overwrite local variables $KEY$ and $LOCK$, and (iv) add $\eqc$ into \vone. % \kartik{add appropriate line numbers here if they are from forensic algorithm}
    % \kartik{if we use threshold $2t+1$, we need to mention that.}
\end{itemize}

A client first verifies leader election (lines~\ref{alg:vaba-request-proof-leader-1}-\ref{alg:vaba-request-proof-leader-2}). Then, it follows steps similar to the HotStuff forensic protocol (lines~\ref{alg:vaba-28}-\ref{alg:vaba-end}) except that there are added checks pertaining to leader elections (lines~\ref{alg:vaba-verify-leader-1},\ref{alg:vaba-verify-leader-2},\ref{alg:vaba-verify-leader-3}).

We prove the forensic support in Theorem~\ref{thm:vaba}.
\begin{theorem}
\label{thm:vaba}
For $n=3t+1$, when $f > t$, if two honest replicas output conflicting values, VABA protocol provides $(2t,\ 1,\ t+1)$-forensic support. Further $(2t+1,\ n-f,\ d)$-forensic support is impossible with $d>0$.
\end{theorem}
\begin{proof} We prove the forward part of the theorem below. The proof of converse (impossibility) is the same as \S\ref{sec:proofoftheorem4.1}.

The leader of a view is determined by the threshold coin-tossing primitive $\threscoin$ and Byzantine replicas cannot  forge the result of a leader election by the robustness property of the threshold coin. % \kartik{if we use Constantinople with k = 2t+1, then it is just a regular use of coin?} 
Suppose two conflicting outputs happen in view $e,e'$ with $e\le e'$. The replica who outputs in view $e'$ has access to the proof of leader election of all views $\le e'$. Therefore, a client can verify the leader election when it receives messages from this replica. Even if other replicas have not received messages corresponding to the elections in views $\le e'$, the client can send the proof of leader to them. The remaining forensic support proof follows from Theorem~\ref{thm:hotstuff_a} in a straightforward manner, where any witness will receive the proof of leader from the client (if leader is not elected) and send the proof of culprits to the client.
\end{proof}

\myparagraph{Communication complexity.} The client needs to first receive all leader election results from view $e$ to view $e'$, and each result is of size $|coin|$ (the size of the coin in the \threscoin primitive). Then, the client shares leader election results with all replicas. This step incurs receiving message complexity $O(l|coin|)$ where $l=e'-e$. Next, the client needs to receive one message from $k=1$ replica and the message size is $(|v|+|sig|)$. Therefore the complexity for the client receiving messages is $O(|v|+|sig|+l|coin|)$. However, the procedure of sharing leader election is irrelevant to forensic support, and we could assign it to replicas. (This procedure is included in the forensic protocol because we do not want to change the consensus protocol itself.) In that case, the client needs to receive just one leader election result, so the receiving message complexity is $O(|v|+|sig|+|coin|)$. % complexity one message from $k=1$ replica and the message size is $(|v|+|sig|)$ where $|v|$ and $|sig|$ stand for the size of a value and an aggregate signature. Therefore the complexity of the client receiving messages is $O(|v|+|sig|)$ for \hsa. As for \hsb, theorem~\ref{thm:hotstuff_b} shows that in the worst case, the client needs to receive messages from $k=t+1$ replicas. Each of those replicas sends one message of size $O(|v|+|sig|+|hash|)$ where $|hash|$ stands for the size of a hash value. Therefore the complexity of the client receiving messages is $O(n(|v|+|sig|+|hash|))$ for \hsb.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% from here is ignored

% \gerui{The threshold of coin tossing can be set to $k=n-t=2t+1$ (actually $t<k\le n-t$). Threshold coin tossing in Constantinople paper only works for $f<t$ for both robustness and unpredictability. Good news is that the robustness property still holds when $f>t$. Robustness: It is computationally infeasible for an adversary to produce k valid shares of an input $s$ such that the output of the coin tossing is not $F(s)$. The reason is: The robustness of the scheme follows from the soundness of the interactive proof of equality of discrete logarithms; and the assumption of the random oracle model.}
\ignore{
\subsection{Highlights}
The modification to original VABA protocol:
\begin{enumerate}
    \item $LOCK=(e)$ is changed to $LOCK=(e,v)$. ($e$ is view number, $v$ is value.)
    \item Voting rule is changed. Before: vote if proposal, a.k.a \qctwo or $KEY$ (in \nv) has view higher than or equal to $LOCK$. After: vote if $KEY$ has view and value equal to $LOCK$, except that $KEY$'s view is strictly higher than $LOCK.e$.
    \item Assume a replica's own \vc message arrives first so that others \vc message won't overwrite local variables.
    \item add $\eqc$ into \vone which is the same modification as HotStuff.
\end{enumerate}

Description in detail:
\begin{enumerate}
    \item $LOCK$ keeps the latest locked tuple of view and value
    \item \textbf{Voting rule.} Once a replica locks on view $e$ and value $v$, in subsequent views, it only votes when it observes a \qctwo on $(e,v)$  (same view and value as lock), or it observes a \qctwo from a higher view in a \nv message. In the latter case, it ``unlocks'' and vote for any value.
    \item Preference over its own \vc message: we assume the \vc message sent by itself arrives first among all messages. This preference prevents conflicting QCs created in the same view by Byzantine replicas from overwriting local variables.
\end{enumerate}
\subsection{Overview} %\gerui{VABA definition has two more properties: fairness and efficiency, but I think we don't need to mention them.} 
VABA  utilizes  two cryptographic techniques (besides multi-signatures): threshold signatures (\thressignature) and threshold coin-tossing (\threscoin). 
Similar to HotStuff, the protocol proceeds in a sequence of consecutive views. Each view progresses as follows:
\begin{itemize}[leftmargin=*, topsep=0pt]
	\item[-] \textbf{\pp.} In this stage, $n$ replicas run $n$ parallel HotStuff-like instances (explained later), where replica $i$ acts as the leader within instance $i$.
    \item[-] \textbf{Leader-Election.} 
		After finishing the previous stage, replicas use the outputs with \threscoin primitive to randomly elect the {\it leader of this view}, denoted as $Leader[e]$ ($e$ is view nunber). Replicas adopt $Leader[e]$’s instance from \pp stage, and discard other instances.
	\item[-] \textbf{\vdashc.} Replicas broadcast quorum certificates (QCs) from $Leader[e]$’s \pp instance and update local variables and/or output value accordingly (explained below).
\end{itemize}

Replicas keep two important local variables, $LOCK$ and $KEY$. Their roles are similar to $LOCK$ and $\qctwo$ in HotStuff: $LOCK$ keeps the latest locked tuple of view and value whereas $KEY$ records the latest $\qctwo$ a replica has received. The rule to updating these variables will be explained later. 

Each instance of \pp is similar to a HotStuff instance within one view, except that (a) there is one more round of voting, and (b) replicas hold QCs and defer local variable updating and committing until \vdashc stage. Each instance progresses as follows, where replica $i$ acts as the leader within instance $i$:
\begin{itemize}[leftmargin=*, topsep=0pt]
    \item[-] \textbf{Propose.} The leader proposes a \nv message containing its local variable $KEY$ and sends it to all replicas.
    \item[-] \textbf{\vone.} On receiving a \nv message containing $KEY$ and parsing its value $v$ and view $e'$, a replica sends \vone for $(v,e')$ if it is \emph{safe} to vote based on a locking mechanism (explained later). It sends this vote to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qctwo in view $e$. The leader sends the view $e$ \qctwo to all replicas.
    \item[-] \textbf{\vtwo.} On receiving a \qctwo in view $e$ containing message $v$, a replica sends \vtwo to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qcprecom and send it to all replicas.
    \item[-] \textbf{\vthree.} On receiving \qcprecom in view $e$ containing message $v$ from the leader, a replica sends \vthree to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qcthree and send it to all replicas.
    \item[-] \textbf{\vfour and Output.} On receiving \qcthree from the leader, a replica  sends \vfour to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qcfour, which is the leader's output.
\end{itemize}

The output for the leader $i$ of a \pp instance is \qcfour, which is broadcast upon entering Leader-Election stage. In Leader-Election stage, a replica collects $2t+1$ such \qcfour, and broadcasts a signed \skipshare message to imply that it has collected $2t+1$ \qcfour. A replica collects $2t+1$ \skipshare messages and broadcast a \skipmsg message containing the threshold signature created from those \skipshare messages. When a replica receives a \skipmsg message, it broadcast a \skipmsg message if it has not done so. It abandons all $n$ \pp instances it participates, and broadcasts a signed \coinshare message.  Again, a replica collects $2t+1$\gerui{$t+1$ written in VABA paper} \coinshare messages, and uses them with \threscoin primitive to randomly elect the leader of this view, denoted as $Leader[e]$ where $e$ is the view number.

In \vdashc stage, a replica collects three type of QCs: \qctwo, \qcprecom, and \qcthree from $Leader[e]$'s \pp instance (if any), and broadcast them. Then, a replica collects view change messages from  $2t+1$ distinct replicas and update its local variables and commit value as follows:
\begin{itemize}[leftmargin=*, topsep=0pt]
    \item[-] On receiving \qctwo: if \qctwo is in a view higher than $KEY$, update local variable $KEY\gets \qctwo$.
	\item[-] On receiving \qcprecom: if \qcprecom is in a view higher than $LOCK$, update local variable $LOCK\gets (\qcprecom.e,\qcprecom.v)$, i.e., the view and value of \qcprecom.
	\item[-] On receiving \qcthree: commit to its value $\qcthree.v$.
	\item[-] Preference over it own QCs: we assume the QCs sent by itself arrives first among all QCs.\ignore{On receiving a \qctwo/\qcprecom from itself, first follow the updating rule, then stop updating $KEY$/$LOCK$ from further view change messages for the same view.} This preference prevents conflicting QCs created in the same view by Byzantine replicas from overwriting local variables.
\end{itemize}


\myparagraph{Voting rule.} Once a replica locks on view $e$ and value $v$, in subsequent views, it only votes when it observes a \qctwo on $(e,v)$  (same view and value as lock), or it observes a \qctwo from a higher view in a \nv message. In the latter case, it ``unlocks'' and vote for any value. % The only exception is when it observes a \qctwo on $(e,v)$ in a \nv message.

The safety and liveness of the VABA protocol when $f \leq t$ follows from the following:

\myparagraph{Uniqueness within a view.} Within a \pp instance, since replicas only vote once in each round, a \qcthree can be formed for only one value when $f \leq t$.

\myparagraph{Safety and liveness across views.} Safety across views is ensured by the use of locks and the voting rule for a \nv message. Whenever a replica commits a value, at least $2t+1$ other replicas are locked on the value in the view. A replica only votes for the value it is locked on. The only scenario in which it votes for a conflicting value $v'$ is if the leader includes a \qctwo for $v'$ from a higher view in \nv message. Similar to HotStuff, the constraint of voting for $v'$ is not necessary for safety, but only for liveness of the protocol.\kartik{a commit happens only after a leader is elected. Also, how do the 4th round of votes help here?} \gerui{For the first part I agree, and need we point it out here? For the second question, 4th round doesn't help safety. The output of 4th round is used in leader election.}



\subsection{Forensic Support for VABA}

Assume that there is a disagreement and the current view number is $e$. A client can query replicas for $Leader[e^\#]$ of each view $e^\#\le e$ (with a proof of leader), and then query the transcripts (such as \qctwo and \qcprecom) of the corresponding \pp instance. \gerui{Notice that \threscoin primitive ensures that one unique leader will be elected for each view, and Byzantine replicas cannot change the result of a leader election.} Therefore, retrospectively, there is only the leader's HotStuff-like instance in each view, and the transcripts are identical to those in HotStuff protocol. As a result, the HotStuff forensic protocol can be adapted for VABA straightforwardly.\kartik{a discussion about the existence of two leaders is missing. We need to talk about what can go wrong in that phase.} \gerui{I added a sentence in the middle of this paragraph.}

Algorithm~\ref{alg:fa-vaba} describes the protocol to obtain forensic support atop VABA.\ignore{A complete description of the VABA protocol is also provided in Algorithm~\ref{alg:vaba:01} and \ref{alg:vaba:02}. The messages in VABA protocol are similar to those in HotStuff except that the former messages contain an extra field $i$, the instance number.} In VABA, a leader is elected on the fly, therefore, the forensic protocol has a few changes for leader election verification. Each replica maintains a list of \pflock for all instances, containing all received \qctwo from \prepare messages, \nv messages, and \vc messages (line~\ref{alg:vaba-6},\ref{alg:vaba-6-2},\ref{alg:vaba-6-3}). When the leader of a view is elected, a replica keeps the \pflock from the leader's instance and discard others (line~\ref{alg:vaba-12}). A replica also keeps the random coins for leader election, for client's verification (line~\ref{alg:vaba-13}). A client should first query and verify the leader elections (line~\ref{alg:vaba-request-proof-leader-1}-\ref{alg:vaba-request-proof-leader-2}). Then, a client follows the steps similar to the HotStuff forensic protocol (line~\ref{alg:vaba-28}-\ref{alg:vaba-end}), where it should also verify the leader election of replicas' replies (line~\ref{alg:vaba-verify-leader-1},\ref{alg:vaba-verify-leader-2},\ref{alg:vaba-verify-leader-3}).
%if a client observes commits for two conflicting values in the same view, it can determine the culprits by two \commit messages (line~\ref{alg:hotstuff-28}).  Otherwise, the client sends a request to all replicas for possible proof between two committed views $e, e'$ for $e<e'$ (line~\ref{alg:hotstuff-23}). Each replica looks through its list for views $e<e^\#\le e'$. If there exists a \qctwo whose value is different from the value $v$ committed in $e$ and recorded $\eqc$ is less than $e$, it sends a reply with this \qctwo to the client (line~\ref{alg:hotstuff-12}). The client waits for a \qctwo (line~\ref{alg:hotstuff-24}) from $e^\#$ between two committed views. If it contains a different value from the first committed value and an older view number $\eqc < e$, the intersection of this \qctwo and the \qcthree from the commit message in the lower view proves at least $t+1$ culprits (line~\ref{alg:hotstuff-26}).

}


\ignore{
\begin{algorithm}[H]
\begin{algorithmic}[1]
    \State $KEY\gets \lr{0,v_i,\sigma_\perp,0}$ with selectors $e,v,\sigma,\eqc$
    \State $LOCK \gets \lr{0,v_\perp}$ with selectors $e,v$ \algorithmiccomment{$0, v_\perp,\sigma_\perp$: default view, value, and signature}
    \State $e\gets 1$ \algorithmiccomment{View number}
    \While{$true$}
        \LeftComment{\pp Stage}
        \State participate in $\pp(id,e,j)$ ($j\neq i$)
        \State start $\pp(id,e,i)$ as leader
        \State broadcast the output $\qcfour$ in message $\lr{\done,e,\qcfour}$
        \LeftComment{Leader-Election Stage}
        \State collect $\lr{\done,e,\cdot}$ from $2t+1$ distinct replicas, broadcast $\signed{\skipshare,e}$ \algorithmiccomment{Use \thressignature}
        \State collect $\signed{\skipshare,e}$ from $2t+1$ distinct replicas, denote the collection as $\Sigma$
        \State create threshold signature from $\Sigma$ denoted as $\sigma$, broadcast $\lr{\skipmsg,e,\sigma}$
        \Upon{$\lr{\skipmsg,e,\sigma}$}
        \State abandon all $\pp(id,e,j)$ ($j\in[n]$)
        \State broadcast $\lr{\skipmsg,e,\sigma}$ if has not done so
        \State broadcast $\signed{\coinshare,e}$ \algorithmiccomment{Use \threscoin}
        \State collect $\signed{\coinshare,e}$  from $2t+1$ distinct replicas, and generate a random leader by threshold coin-tossing, denoted as $Leader[e]$
        \State go to \vdashc stage
        \EndUpon
    \LeftComment{\vdashc Stage}
    \State extract \qctwo, \qcprecom, and \qcthree from $\pp(id,e,Leader[e])$; use $\perp$ if a QC is not recorded
    \State broadcast $\lr{\vc,e,\qctwo,\qcprecom,\qcthree}$%\algorithmiccomment{If any QC is not recorded, use $\perp$}
    \Upon{$\lr{\vc,e,\qctwo,\qcprecom,\qcthree}$} \algorithmiccomment{Assume its own message arrives first}
    \If{$\qctwo \neq \perp\land \qctwo.e>KEY.e$}
        \State $KEY\gets \qctwo$
    \EndIf
    \If{$\qcprecom \neq \perp\land \qcprecom.e>LOCK.e$}
        \State $LOCK\gets (\qcprecom.e,\qcprecom.v)$
    \EndIf
    \If{$\qcthree \neq \perp$}
        \State decide $\qcthree.v$
    \EndIf
    \EndUpon
    \State collect $\lr{\vc,e,\cdot,\cdot,\cdot}$ from $2t+1$ distinct replicas, enter  the next view, $e\gets e+1$
    \EndWhile
    % \ForInitialize{$e\ge 1$}
    % \State $Leader[e]\gets \perp$
    % \EndForInitialize
\end{algorithmic}
 \caption{VABA protocol, replica $i$'s initial value $v_i$}
 \label{alg:vaba:01}
\end{algorithm}

\begin{algorithm}[H]
\begin{algorithmic}[1]
    %\State parse $id$ as $(ID,e,i)$ \algorithmiccomment{Replica $i$ is the leader within instance}
    \LeftComment{Propose and \vone Phase}
    \As{a leader}
        \State broadcast $\lr{i,\nv,e,KEY}$
    \EndAs{}
    \As{a replica}
        \State wait for  $\lr{i,\nv,e,L}$ from leader
        \State $\eqc\gets L.e$ \algorithmiccomment{the view number of $L$}
        \If{$(LOCK.e < \eqc) \lor (LOCK.e=\eqc \land LOCK.v = v)$}
            \State send $\signed{i,\vone,e,v, \eqc}$ to leader 
        \EndIf
    \EndAs{}
    \LeftComment{\vtwo Phase}
    \As{a leader}
        \State collect $\signed{i,\vone,e,v,\eqc}$ from $2t+1$ distinct replicas, denote the collection as $\Sigma$
        \State $\sigma\gets \thressign(\Sigma)$ %\algorithmiccomment{$\sigma$ is $\qctwo$}
        \State broadcast $\lr{i,\prepare,e,v,\sigma,\eqc}$
    \EndAs{}
    \As{a replica}
        \State wait for $\lr{i,\prepare,e,v,\sigma,\eqc}$ from leader
        \State record $(e,v,\sigma, \eqc)$ as $\qctwo$ for this instance
        \State send $\signed{i,\vtwo,e,v}$ to leader
    \EndAs{}
    \LeftComment{\vthree Phase}
    \As{a leader}
        \State collect $\signed{i,\vtwo,e,v}$ from $2t+1$ distinct replicas, denote the collection as $\Sigma$
        \State $\sigma\gets \thressign(\Sigma)$
        \State broadcast $\lr{i,\precommit,e,v,\sigma}$
    \EndAs{}
\As{a replica}
        \State wait for $\lr{i,\precommit,e,v,\sigma}$ from leader
        \State record $(e,v,\sigma)$ as $\qcprecom$ for this instance
        \State send $\signed{i,\vthree,e,v}$ to leader
    \EndAs{}
    \LeftComment{\vfour and Output Phase}
    \As{a leader}
        \State collect $\signed{i,\vthree,e,v}$ from $2t+1$ distinct replicas, denote the collection as $\Sigma$
        \State $\sigma\gets \thressign(\Sigma)$ 
        \State broadcast $\lr{i,\commit,e,v,\sigma}$
        \State collect $\signed{i,\vfour,e,v}$ from $2t+1$ distinct replicas, denote the collection as $\Sigma'$
        \State $\sigma'\gets \thressign(\Sigma')$
        \State output $(e,v,\sigma')$ as $\qcfour$
    \EndAs{}
    \As{a replica}
        \State wait for $\lr{i,\commit,e,v,\sigma}$ from leader
        \State record $(e,v,\sigma)$ as $\qcthree$ for this instance
        \State send $\signed{i,\vfour,e,v}$ to leader
    \EndAs{}
\caption{VABA protocol, instance $\pp(id,e,i)$; replica $i$ is the leader within instance}
\label{alg:vaba:02}
\end{algorithmic}
\end{algorithm}
}
% \begin{algorithm}[H]
% \begin{algorithmic}[1]
%     \State parse $id$ as $(ID,e)$
%     \State extract recorded \qctwo, \qcprecom, and \qcthree from the leader's \pp instance identified by $(id,e,Leader[e])$; use $\perp$ if any type of QC is not recorded
%     \State broadcast $\lr{\vc,e,\qctwo,\qcprecom,\qcthree}$%\algorithmiccomment{If any QC is not recorded, use $\perp$}
%     \State collect $\lr{\vc,e,\cdot,\cdot,\cdot}$ from $2t+1$ distinct replicas, enter  the next view, $e\gets e+1$
%     \vspace{1em}
%     \Upon{$\lr{\vc,e,\qctwo,\qcprecom,\qcthree}$} \algorithmiccomment{Assume its own message arrives first}
%     \If{$\qctwo \neq \perp\land \qctwo.e>KEY.e$}
%         \State $KEY\gets \qctwo$
%     \EndIf
%     \If{$\qcprecom \neq \perp\land \qcprecom.e>LOCK.e$}
%         \State $LOCK\gets (\qcprecom.e,\qcprecom.v)$
%     \EndIf
%     \If{$\qcthree \neq \perp$}
%         \State decide $\qcthree.v$
%     \EndIf
%     \EndUpon
% \caption{VABA protocol, \vdashc stage: instance identifier $id=(ID,e)$}
% \label{alg:vaba:04}
% \end{algorithmic}
% \end{algorithm}

==> [CCS21] BFT Protocol Forensics/B_lb-sketch.tex <==
\section{Impossibility of Forensic Support for $n=2t+1$}\label{sec:lb}

A validated Byzantine agreement protocol allows replicas to obtain agreement, validity, and termination so far as the actual number of faults $f\leq t$ where $t$ is a Byzantine threshold set by the consensus protocol. A protocol that also provides forensic support with parameters $m$ and $d$ allows the detection of $d$ Byzantine replicas when $\leq m$ out of $n$ replicas are Byzantine faulty. In particular, in \S\ref{sec:pbft} and \S\ref{sec:basic-hotstuff}, we observed that when $t=\lfloor n/3\rfloor,\ m = 2t$, and $k=1$, we can obtain $(2t,1,d)$-forensic support for $d = t+1$. This section presents the limits on the number of Byzantine replicas detected ($d$), given the total number of Byzantine faulty replicas available in the system ($m$). In particular, we show that if the total number of Byzantine faults are too high, in case of a disagreement, the number of corrupt (Byzantine) replicas that can be deemed undeniably culpable will be too few.


\myparagraph{Intuition.} To gain intuition, let us consider a specific setting with $n = 2t+1$, $m = n-t = t+1$, and $d > 1$. Thus, such a protocol provides us with agreement, validity, and termination if the Byzantine replicas are in a minority. If they are in the majority, the protocol transcript provides undeniable guilt of more than one Byzantine fault. We show that such a protocol does not exist. Why? Suppose we split the replicas into three groups $P$, $Q$, and $R$ of sizes $t$, $t$, and $1$ respectively. First, observe that any protocol cannot expect Byzantine replicas to participate in satisfying agreement, validity, and termination. Hence, if the replicas in $Q$ are Byzantine, replicas in $P \cup R$ may not receive any messages from $Q$. However, if, in addition, the replica $R$ is also corrupt, then $R \cup Q$ can separately simulate another world where $P$ are Byzantine and not sending messages, and $Q \cup R$ output a different value. Even if an external client obtains a transcript of the entire protocol execution (i.e., transcripts of $k=n-f$ honest replicas and $f$ Byzantine replicas), the only replica that is undeniably culpable is $R$ since it participated in both worlds. For all other replicas, neither $ P $ nor $ Q $ have sufficient information to prove the other set's culpability. Thus, an external client will not be able to detect more than one Byzantine fault correctly.
Our lower bound generalizes this intuition to hold for $n > 2t$, $m = n-t$, $k = n-f$, and $d > n-2t$.

\begin{theorem} For any validated Byzantine agreement protocol with $t<n/2$, when $f > t$, if two honest replicas output conflicting values, $(n-t,\ n-f,\ d)$-forensic support is impossible with $d>n-2t$.
\end{theorem}

\begin{proof}
Suppose there exists a protocol that achieves agreement, validity, termination, and forensic support with parameters $n,\ t < n/2,\ m = n-t,\ k = n-f$ and $d > n-2t$. Through a sequence of worlds, and through an indistinguishability argument we will show the existence of a world where a client incorrectly holds at least one honest replica as culpable.
Consider the replicas to be split into three groups $P,\ Q$, and $R$ with $t$, $t$, and $n-2t$ replicas respectively. We consider the following sequence of worlds:

\myparagraph{World 1.} [$t$ Byzantine faults, satisfying agreement, validity, and termination]

\noindent\underline{Setup.} Replicas in $P$ and $R$ are honest while replicas in $Q$ have crashed. $P$ and $R$ start with a single externally valid input $v_1$. All messages between honest replicas arrive instantaneously.

\noindent\underline{Output.} Since there are $|Q| = t$ faults, due to agreement, validity and termination properties, replicas in $P$ and $R$ output $v_1$. Suppose replicas in $P$ and $R$ together produce a transcript $T_1$ of all the messages they have received. % Based on the transcript produced by $P$ and $R$, an external client commits $v_1$.

\myparagraph{World 2.} [$t$ Byzantine faults, satisfying agreement, validity, and termination]

\noindent\underline{Setup.} Replicas in $Q$ and $R$ are honest while replicas in $P$ have crashed. $Q$ and $R$ start with an externally valid input $v_2$. All messages between honest replicas arrive instantaneously.

\noindent\underline{Output.} Since $t$ replicas are Byzantine faulty, due to agreement, validity and termination properties, replicas in $Q$ and $R$ output $v_2$. Suppose replicas in $Q$ and $R$ together produce a transcript $T_2$ of all the messages they have received. % Based on the transcript produced by $Q$ and $R$, an external client commits $v_2$.

\myparagraph{World 3.} [$n-t$ Byzantine faults satisfying validity, termination, forensic support]

\noindent\underline{Setup.} Replicas in $P$ are honest while replicas in $Q$ and $R$ are Byzantine. Replicas in $P$ start with input $v_1$. Replicas in $Q$ and $R$ have access to both inputs $v_1$ and $v_2$. $Q$ behaves as if it starts with input $v_2$ whereas $R$ will use both inputs $v_1$ and $v_2$.  Replicas in $Q$ and $R$ behave with $P$ exactly like in World~1. In particular, replicas in $Q$ do not send any message to any replica in $P$. Replicas in $R$ perform a split-brain attack where one brain interacts with $P$ as if the input is $v_1$ and it is not receiving any message from $Q$. 
Also, separately, replicas in $Q$ and the other brain of $R$ start with input $v_2$ and communicate with each other exactly like in World~2. They ignore messages arriving from $P$. 

\noindent\underline{Output.} For replicas in $P$, this world is indistinguishable from that of World~1. Hence, they output $v_1$. Replicas in $P$ and the first brain of $R$ output transcript $T_1$ corresponding to the output. Replicas in $Q$ and the other brain of $R$ behave exactly like in World~2. Hence, they can output transcript $T_2$. Since the protocol provides $(n-t,n-f, d)$-forensic support for $d > n-2t$, the transcript  of messages should hold $d > n-2t$ Byzantine replicas undeniably corrupt. Suppose the client can find the culpability of $> n-2t$ replicas from $Q \cup R$, i.e., $\geq 1$ replica from $Q$.

\myparagraph{World 4.} [$n-t$ Byzantine faults satisfying validity, termination, forensic support]

\noindent\underline{Setup.} Replicas in $Q$ are honest while replicas in $P$ and $R$ are Byzantine. Replicas in $Q$ start with input $v_2$. Replicas in $P$ and $R$ have access to both inputs $v_1$ and $v_2$. $P$ behaves as if it starts with input $v_1$ whereas replicas in $R$ use both $v_1$ and $v_2$. Replicas in $P$ and $R$ behave with $Q$ exactly like in World~2. In particular, replicas in $P$ do not send any message to any replica in $Q$. Replicas in $R$ perform a split-brain attack where one brain interacts with $Q$ as if the input is $v_2$ and it is not receiving any message from $P$. 
Also, separately, replicas in $P$ and the other brain of $R$ start with input $v_1$ and communicate with each other exactly like in World~1. They ignore messages arriving from $Q$.

\noindent\underline{Output.} For replicas in $Q$, this world is indistinguishable from that of World~2. Hence, they output $v_2$. Replicas in $Q$ and the first brain of $R$ output transcript $T_2$ corresponding to the output. Replicas in $P$ and the other brain of $R$ behave exactly like in World~1. Hence, they can output transcript $T_1$. 

Observe that the transcript and outputs produced by replicas in $P$, $Q$, and $R$ are exactly the same as in World~3. Hence, the client will hold $> n-2t$ replicas from $Q \cup R$, i.e., $\geq 1$ replica from $Q$ as culpable. However, all replicas in $Q$ are honest in this world. This is a contradiction.
\end{proof}

==> [CCS21] BFT Protocol Forensics/C_proofs.tex <==
\section{Proof of Theorems}\label{sec:proof-diem}

\subsection{Proof of Theorem~\ref{thm:pbft}}
\label{sec:proofoftheorem4.1}

\begin{proof}

Suppose there are $f = 2t+1$ Byzantine replicas, and let there be three replica partitions $P, Q, R$, $|P|=|Q|=t$, $|R|=t+1$. To prove the result, suppose the protocol has forensic support for $d>0$, we construct two worlds where a different set of replicas are Byzantine in each world. 


\myparagraph{World~1.} Let $R,Q$ be Byzantine replicas in this world. During the protocol, replicas in $Q$ behave like honest parties. Suppose in view $e, e'$ ($e < e'$), two honest replicas $p_1,p_2\in P$ output two conflicting values $v, v'$ after receiving two \qcthree. The \qcthree for $v$ contains the \commit messages from $P$ and $R$, the \qcthree for $v'$ contains the \commit messages from $R$ and $Q$. All the other messages never reach $P$. During the forensic protocol, replicas in $P$ send their transcripts to the client. Since the protocol has forensic support for $d>0$, using these transcripts (two \qcthree), the forensic protocol determines some subset of $R$ are culpable (since $Q$ behave like honest).

\myparagraph{World~2.} Let $P,Q$ and some replica $r\in R$ are Byzantine replicas and replicas in $r$ behave honestly. Again, in view $e, e'$ ($e < e'$), two replicas $p_1,p_2\in P$ output two conflicting values $v, v'$ after receiving two \qcthree. The \qcthree for $v$ contains the \commit messages from $P$ and $R$, the \qcthree for $v'$ contains the \commit messages from $R$ and $Q$. Replicas in $R$ unlock themselves due to receiving a higher \qctwo formed in $e^*$ ($e<e^*<e'$). During the forensic protocol, replicas in $P$ send the same transcripts as of World~1 to the client (only two \qcthree). Thus, the forensic protocol outputs some subset of $R$ as culpable replicas. However, this is incorrect since replicas in $R$ are honest ($r$ is indistinguishable with replicas in $R/\{r\}$). This complete the proof.
\end{proof}


%\subsection{Proof of Theorem~\ref{thm:hotstuff_a}}
%\label{sec:proofoftheorem5.1}

%\subsection{Proof of Theorem~\ref{thm:hotstuff_b}}
%\label{sec:proofoftheorem5.2}

\subsection{Proof of Theorem~\ref{thm:hotstuff-null}}
\label{proof:hotstuff-null}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/null1.pdf}
    \caption{World~1 of Theorem~\ref{thm:hotstuff-null}. Replicas are represented as colored nodes. Replica partitions are $P$, $\{x\}$ (Byzantine), $R$ (Byzantine), and $Q$ from top to bottom.}
    \label{fig:hotstuff-null-1}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/null2.pdf}
    \caption{World~2 of Theorem~\ref{thm:hotstuff-null}. Replicas are represented as colored nodes. Replica partitions are $P$ (Byzantine), $\{x\}$ (Byzantine), $R$, and $Q$ from top to bottom.}
    \label{fig:hotstuff-null-2}
\end{figure}

\begin{proof}
Suppose the protocol provides forensic support to detect $d>1$ Byzantine replicas with irrefutable proof and the proof can be constructed from the transcripts of all honest replicas.  To prove this result, we construct two worlds where a different set of replicas are Byzantine in each world. We will fix the number of Byzantine replicas $f=t+1$, but the following argument works for any $f\ge t+1$.

Let there be four replica partitions $P,Q,R,\{x\}$. $|Q|=|P|=|R|=t$, and $x$ is an individual replica. In both worlds, the conflicting outputs are presented in view $e,e'$ ($e+1<e'$) respectively. Let $\qcthree_1$ be on value $v$ in view $e$, and signed by $P,R,x$. And let $\qcthree_2$ (and a \qcprecom) be on value $v'$ in view $e'$, and signed by $Q,R,x$. Suppose the leader of view $e,e^*,e'$ ($e<e^*<e'$) is replica $x$.

\myparagraph{World~1} is presented in Figure~\ref{fig:hotstuff-null-1}. % Let $R$ and $x$ be Byzantine replicas in this world, and they sign \qctwo on $v'$ in $e'$ with $Q$, which is in the first view $>e$. In view $e^*$, the leader proposes value $v'$ and $Q$ sends \prepare on it, but it doesn't form a \qctwo. % \kartik{Write this as: 
Let $R$ and $x$ be Byzantine replicas in this world. In view $e^*$, the leader proposes value $v'$ and $Q$ sends \prepare on it, but a \qctwo is not formed. In view $e'$, the Byzantine parties, together with $Q$, sign \qctwo on $v'$. $e'$ is the first view where a \qctwo for $v'$ is formed.

During the forensic protocol, all honest replicas in $P$ and $Q$ send their transcripts. Byzantine $R$ and $x$ do not provide any information. Since the protocol has forensic support, the forensic protocol can output $d > 1$ replicas in $R$ and $x$ as culprits. 


\myparagraph{World~2} is presented in Figure~\ref{fig:hotstuff-null-2}. % Let $P$ and $x$ be Byzantine replicas in this world, and they sign the first \qctwo on $v'$ in $e^*$ with $Q$, which is the first view $> e$. \kartik{
Let $P$ and $x$ be Byzantine replicas in this world. Here, in view $e^* > e$, $P$ and $x$, together with $Q$ sign \qctwo on $v'$. In this world, $e^*$ is the first view where a \qctwo for $v'$ is formed. View $e' > e^*$ is similar to that of World~1 except that honest $R$ receives a \nv message with $\qctwo^*$ (rather than $\qctwo_{old}$).

During the forensic protocol, $Q$ sends their transcripts, which are identical to those in World~1. Byzantine $P$ can provide the same transcripts as those in World~1. Observe that the transcripts from $P$ and $Q$ presented to the forensic protocol are identical to those in World~1. Thus, the forensic protocol can also outputs $d>1$ replicas in $R$ and $x$ as culpable. In World~2, this is incorrect since replicas in $R$ are honest. 

Based on $2t$ transcripts, World~1 and World~2 are indistinguishable. To obtain an irrefutable proof of $d>1$ culprits, the client needs to collect more than $2t$ transcripts, more than the number of honest parties available. This completes the proof. % However, Byzantine replicas can always choose to stay silent during the forensic protocol and honest replicas can provide at most $2t$ transcripts. This complete the proof.}
\end{proof}

\paragraph{Remark.} The above proof can be easily modified to work with parameters $d > 0$ when $m = t+2$.

\subsection{Proof of Theorem~\ref{thm:algorand}}\label{sec:algorand-proof}
\begin{proof}
We construct two worlds where a different set of replicas are Byzantine in each world. Let replicas be split into three partitions $P$, $Q$, and $R$, and $|P|=(n-2\epsilon)/3,|Q|=|R|=(n+\epsilon)/3$ 
%where $N$\gerui{Is $n,N$ same here?} is the number of replicas 
and $\epsilon>0$ is a small constant. Denote the numbers of replicas from $P,Q,R$ in a committee by $p,q,r$. Let $\kappa$ denote the expected committee size; $t_H=2\kappa/3$. With constant probability, we will have $p < \kappa/3$, $q > \kappa/3$ and $r > \kappa/3$ and $p+q < 2\kappa/3$ in steps 4 to 8. % \kartik{Pramod, do we need to be more formal here?}

\myparagraph{World~1.} Replicas in $R$ are Byzantine in this world. We have $p+q < t_H$ and $q+r > t_H$. The Byzantine parties follow the protocol in \gradedconsensus. Thus, all replicas in step 4 hold the same tuple of $b=0$ and $v$ ($v\neq v_\perp$). Then, the following steps are executed.
\begin{itemize}
    \item[Step 4] Honest committee members that belong to $P$ and $Q$ broadcast their votes on $(b=0,v)$ whereas Byzantine committee members that belong to $R$ send votes to replicas in $P$ and not $Q$. %(Without loss of generality, suppose the honest replicas in committees for the next steps belong to $Q$).
    \item[Step 5] Replicas in $P$ satisfy Ending Condition 0, and output $b=0$ and the value $v$. Replicas in $Q$ do not receive votes from committee members in $R$, so they update $b=0$ and broadcast their votes on $(b=0, v)$. %Honest committee members that belong to $Q$ doesn't receive votes from committee members in $R$, so they update $b=0$ and broadcast their votes on $(b=0,v)$. 
    Byzantine committee members that belong to $R$ pretend not to receive votes from committee members in $Q$, and also update $b=0$. And they send votes to replicas in $P$ and not $Q$.
    \item[Step 6] Replicas in $Q$ update $b=1$ since they receive $p+q<t_H$ votes.  Replicas in $R$ pretend not to receive votes from committee members in $Q$, and also update $b=1$. Committee members in $Q$ and $R$ broadcast their votes.
    \item[Steps 7-8] Committee members that belong to $Q$ and $R$ receive $q+r>t_H$ votes, so they update $b=1$ and broadcast their votes.
    %Since $q+r>2/3 n$, there are more than $2/3 n$ such votes.
    \item[Step9] Replicas in $Q$ and $R$ satisfy Ending Condition 1, and output $b=1$ and $v_\perp$, a disagreement with replicas in $P$.
\end{itemize}
During the forensic protocol, replicas in $P$ send their transcripts and state that they have output $b=0$. $Q$ and $R$ send their transcripts claiming in steps 4 and 5 they do not hear from the other partition, and they state that output $b=1$. %\gerui{$|P|<1/3$, I think ALgorand doesn't care about 1/3 replicas commit a value, right?}\kartik{did not understand this comment.}\gerui{the question is that do we need $b=0$ to be committed by $>1/3$ replicas? I guess no.}

If this protocol has any forensic support, then it should be able to detect some replica in $R$ as Byzantine.

\myparagraph{World~2.} This world is identical to World~1 except (i) Replicas in $Q$ are Byzantine and replicas in $R$ are honest, and (ii) the Byzantine set $Q$ behaves exactly like set $R$ in World~1, i.e., replicas in $Q$ do not send any votes to $R$ in steps 4 and 5 and ignore their votes. % symmetrically to  Let replicas in $Q$ be Byzantine in this world. Similar to world 1, assume \gradedconsensus gives all committee members in step 4 $(b=0,v)$. Next, in steps 4-9, let $Q$ act symmetrically as if they are in world 1: $Q$ don't send to $R$ and ignore votes from $R$ in step 4 and 5. 
During the forensic protocol, $P$ send their transcripts and state that they have output $b=0$. $Q$ and $R$ send their transcripts claiming in steps 4 and 5 they do not hear from the other partition, and they state that output $b=1$. 

From an external client's perspective, World~2 is indistinguishable from World~1. In World~2, the client should detect some replica in $R$ as Byzantine as in World~1, but all replicas in $R$ are honest. % which is a contradiction.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:diem}}


\begin{proof}Suppose two conflicting blocks $b,\ b'$ are output in views $e$, $e'$ respectively.

\myparagraph{Case $e=e'$.}

\noindent\underline{Culpability.} The \qcthree of $b$ (the QC in $e+3$) and \qcthree of $b'$ intersect in $t+1$ replicas. These $t+1$ replicas should be Byzantine since the protocol requires a replica to vote for at most one value in a view. 

\noindent\underline{Witnesses.} Client can get the proof based on the two blocks in $e+3$, so additional witnesses are not necessary in this case.

\myparagraph{Case $e\neq e'$.}

\noindent\underline{Culpability.}
If $e \neq e'$, then WLOG, suppose $e < e'$. Since $b$ is output in view $e$, it must be the case that $2t+1$ replicas are locked on $(b, e)$ at the end of view $e$. Now consider the first view $e < e^* \leq e'$ in which a higher lock $(b'', e^*)$ is formed where $b'', b$ are not on the same chain (possibly $b''$ is on the chain of $b'$). Such a view must exist since $b'$ is output in view $e' > e$ and a lock will be formed in at least view $e'$. For a lock to be formed, a higher \qctwo must be formed too. 


Consider the first view $e<e^\# \leq e'$ in which a \qctwo in chain of $b''$ is formed. The leader in $e^\#$ broadcasts the block containing a \hqc on $(b'', e'')$. Since this is the first time a higher \qctwo is formed and there is no \qctwo for chain of $b''$ formed between view $e$ and $e^\#$, we have $e''\le e$. The formation of the higher \qctwo indicates that $2t+1$ replicas received the block extending $b''$ with \hqc on $(b'', e'')$ and consider it a valid proposal, i.e., the view number $e''$ is larger than their locks because the block is on another chain. 

 Recall that the output block $b$ indicates $2t+1$ replicas are locked on $(b, e)$ at the end of view $e$. In this case, the $2t+1$ votes in \qctwo in view $e^\#$ intersect with the $2t+1$ votes in \qcthree in view $e$ at $t+1$ Byzantine replicas. These replicas should be Byzantine because they were locked on the block $b$ in view $e$ and vote for a conflicting block in a higher view $e^\#$ whose \hqc is from a view $e'' \leq e$. Thus, they have violated the voting rule.

\noindent\underline{Witnesses.} Client can get the proof by storing a \qctwo formed in $e^\#$ between $e$ and $e'$ in a different chain from $b$. The \qctwo is for the previous block in $e^\#$ whose \hqc is formed in a view $e'' < e$. For the replicas who have access to the \qctwo, they must have access to all blocks in the same blockchain. Thus only one witness is needed ($k=1)$ to provide the \qctwo and its previous block containing the \hqc on $(b'', e'')$, the \qctwo, \hqc and the first \qcthree act as the irrefutable proof.
\end{proof}



==> [CCS21] BFT Protocol Forensics/D_protocols.tex <==
\section{Description of BFT Protocols}\label{sec:bft-protocols}

In the protocols in this paper, we assume that replicas and clients ignore messages with invalid signatures and messages containing external invalid values. When searching for an entity (e.g. lock or \qctwo) with the highest view, break ties by alphabetic order of the value. Notice that ties only occur when $f>t$ and Byzantine replicas deliberately construct conflicting quorum certificates in a view.

With $n=3t+1$, the descriptions of the PBFT protocol and HotStuff protocol are presented in Algorithm~\ref{alg:single-pbft} and \ref{alg:single-hotstuff-modified}.

\subsection{A Forensic Attack on HotStuff-view}
\label{sec:change}
Compared to HotStuff~\cite[Algorithm 2]{yin2019hotstuff}, Algorithm~\ref{alg:single-hotstuff-modified} highlights a slightly different voting rule in line~\ref{alg:change}. In addition to check whether $(LOCK.e < \hqc.e) \lor (LOCK.v = v)$ holds as in HotStuff~\cite[Algorithm 2]{yin2019hotstuff}, when the value in \nv is the same as the value in lock, our voting rule requires $LOCK.e = \hqc.e$.

We argue that the lack of this additional check on the view number will not affect the safety and liveness for HotStuff, but pose a threat for forensics. In the following, we exhibit a forensic attack on \hsa protocol with the original voting rule.
\begin{itemize}
    \item $e=i > 0:$ An honest replica $R$ receives a $\lr{\commit,i,v,\sigma}$ from the leader and updates its lock to be $(i, v, \sigma)$. $R$ sends $\lr{\commit,i,v}$ to leader, which is contained in a $\qcthree$ denoted as $qc_1$. $v$ is output in this view.
    \item $e=i+1:$ $R$ receives $\lr{\commit,i+1,v',\sigma'}$ and updates its lock to be $(i+1, v', \sigma')$. 
    \item $e = i+2:$ A leader broadcasts $\lr{\nv,i+2,v',\hqc}$, where \hqc is a QC from $i-1$. Replica $R$ receives the message and sends $\signed{\vone,i+2, v', i-1}$, because $LOCK.v = v'$ by checking the original voting rule. This message is contained into a $\qctwo$ denoted as $qc_2$. Further, $v'$ is output in this view.
\end{itemize}

In this execution, replica $R$ follows the protocol, however, it will be mistakenly blamed by Algorithm~\ref{alg:fa-hotstuff-a} if the client receives the $qc_1$ for $v$ and the $qc_2$ for $v'$. Since $qc_2.v \ne qc_1.v$ and $qc_2.e_{qc} = i-1 \le qc_1.e = i$ according to line~\ref{alg:hotstuffb-13}.

While the actual \qctwo whose intersection with $qc_1$ should be blamed is generated in $e=i+1$, it is possible that some honest replicas who have the same transcripts as $R$ will be improperly held culpable in this case. By adding the condition to check $LOCK.e = \hqc.e$, honest replicas will not vote for a \nv with stale \hqc, which prevents them from the attack described above.

%\peiyao{Do we need to explain why line14 Algorithm6 is different from original HotStuff? (With the example Jovan Komatovic pointed out)} \kartik{let's do it}

\begin{algorithm*}[t]
\begin{algorithmic}[1]
    \State $LOCK\gets (0,v_\perp,\sigma_\perp)$ with selectors $e,v,\sigma$  \algorithmiccomment{$0, v_\perp,\sigma_\perp$: default view, value, and signature}
    \State $e\gets 1$
    \While{true}
    \LeftComment{\ppr and \vone Phase}
    \As{a leader}
        \State collect $\signed{\vc,e-1,\cdot}$ from $2t+1$ distinct replicas as status certificate $M$ \algorithmiccomment{Assume special \vc messages from view 0}
        \State $ v\gets$ the locked value with the highest view number in $M$
        \If{$v=v_\perp$}
        \State $v\gets v_i$
        \EndIf
        \State broadcast $\lr{\nv,e,v,M}$
    \EndAs{}
    \As{a replica} 
        \State wait for valid $\lr{\nv,e,v,M}$ from leader \algorithmiccomment{Use function \textsc{Valid($\lr{\nv,e,v,M}$)}}
        \State send $\signed{\vone,e,v}$ to leader
        
    \EndAs{}
    \LeftComment{\commit Phase}
    \As{a leader}
        \State collect $\signed{\vone,e,v}$ from $2t+1$ distinct replicas, denote the collection as $\Sigma$
        \State $\sigma\gets \thressign(\Sigma)$ %\algorithmiccomment{$\sigma$ is $\qctwo$}
        \State broadcast $\lr{\commit,e,v,\sigma}$
    \EndAs{}
    \As{a replica}
        \State wait for $\lr{\commit,e,v,\sigma}$ from leader \algorithmiccomment{$\qctwo$}
        \State $LOCK\gets (e,v,\sigma)$
        \State send $\signed{\commit,e,v}$ to leader
    \EndAs{}
    \LeftComment{\reply Phase}
    \As{a leader}
        \State collect $\signed{\commit,e,v}$ from $2t+1$ distinct replicas, denote the collection as $\Sigma$
        \State $\sigma\gets \thressign(\Sigma)$ %\algorithmiccomment{$\sigma$ is $\qcthree$}
        \State broadcast $\lr{\reply,e,v,\sigma}$
    \EndAs{}
\As{a replica}
        \State wait for $\lr{\reply,e,v,\sigma}$ from leader  \algorithmiccomment{$\qcthree$}
        \State output $v$ and send $\lr{\reply,e,v,\sigma}$ to the client
    \EndAs{}
    \State call procedure $\vc()$%Gerui: is this necessary?
    \EndWhile
    \State if a replica encounters timeout in any ``wait for'', call procedure $\vc()$
    \vspace{1em}
\Procedure{$\vc()$}{}
    \State broadcast $\signed{\blame,e}$
    \State collect $\signed{\blame,e}$ from $t+1$ distinct replicas, broadcast them
    \State quit this view
    \State send $\signed{\vc,e,LOCK}$ to the next leader
    \State enter the next view, $e\gets e+1$
\EndProcedure
\Function{\textsc{Valid}}{$\lr{\nv,e,v,M}$}
    \State $v^*\gets$ the locked value with the highest view number in $M$
    \If{$( v^*=v\lor v^*=v_\perp )\land$($M$ contains locks from $2t+1$ distinct replicas)}
    \State return $true$
    \Else
    \State return $false$
    \EndIf
\EndFunction
\caption{PBFT-PK protocol: replica's initial value $v_i$\ignore{\kartik{should move to appendix}\kartik{remove broadcast commit and add changes discussed in algorithm 1}\kartik{use e for view}}}
\label{alg:single-pbft}
\end{algorithmic}
\end{algorithm*}
%Define a valid \nv message as: $\nv.v$ is the highest locked value in $\nv.M$ or the highest locked value is $v_\perp$. And $\nv.v$ pass $\exval$.




\begin{algorithm*}[t]

\begin{algorithmic}[1]
\caption{General HotStuff protocol: replica's initial value $v_i$, protocol variant indicator $var\in$$ \{$`\hsa', `\hsb', `\hsc'$\}$}
\label{alg:single-hotstuff-modified}
    \State $\qctwo\gets (0,v_\perp,\sigma_\perp, \info_\perp)$ with selectors $e,v,\sigma,\info$ 
    \State $LOCK\gets (0,v_\perp)$ with selectors $e,v$  \algorithmiccomment{$0, v_\perp,\sigma_\perp, \info_\perp$: default view, value, signature, and info}
    \State $e\gets 1$
    \While{true}
    \LeftComment{\ppr and \prepare Phase}
    \As{a leader}
        \State collect $\lr{\vc,e-1,\cdot}$ from $2t+1$ distinct replicas as  $M$
        \algorithmiccomment{Assume special \vc messages from view 0}
        \State $\hqc\gets$ the highest QC in $M$
        \State $v\gets$ $\hqc.v$
        \If{$v=v_\perp$}
        \State $v\gets v_i$
        \EndIf
        \State broadcast $\lr{\nv,e,v,\hqc}$
    \EndAs{}
    \As{a replica}
        \State wait for  $\lr{\nv,e,v,\hqc}$ from leader s.t. $\hqc.v=v\lor \hqc.v=v_{\bot}$ \algorithmiccomment{Validate $v$}
            \If{$(LOCK.e < \hqc.e) \lor ( LOCK.v = v \land LOCK.e=\hqc.e)$}\label{alg:change}\Comment{Voting rule, see Appendix~\ref{sec:change}} %$(LOCK.e < \hqc.e) \lor (LOCK.v = v)$}
                \State send $\signed{\vone,e,v, \textsc{Info}(var, \hqc)}$ to leader \Comment{Use function $\textsc{Info}(var, \hqc)$ }
            \EndIf
    \EndAs{}
    \LeftComment{\precommit Phase}
    \As{a leader}
        \State collect $\signed{\vone,e,v,\info}$ from $2t+1$ distinct replicas, denote the collection as $\Sigma$
        \State $\sigma\gets \thressign(\Sigma)$ 
        \State broadcast $\lr{\precommit,e,v,\sigma,\info}$
    \EndAs{}
    \As{a replica}
        \State wait for $\lr{\precommit,e,v,\sigma,\info}$ from leader \algorithmiccomment{$\qctwo$}
        \State $\qctwo\gets (e,v,\sigma, \info)$
        \State send $\signed{\precommit,e,v}$ to leader
    \EndAs{}
    \LeftComment{\commit Phase}
    \As{a leader}
        \State collect $\signed{\precommit,e,v}$ from $2t+1$ distinct replicas, denote the collection as $\Sigma$
        \State $\sigma\gets \thressign(\Sigma)$ 
        \State broadcast $\lr{\commit,e,v,\sigma}$
    \EndAs{}
\As{a replica}
        \State wait for $\lr{\commit,e,v,\sigma}$ from leader  \algorithmiccomment{$\qcprecom$}
        \State $LOCK\gets (e,v)$
        \State send $\signed{\commit,e,v}$ to leader
    \EndAs{}
    \LeftComment{\reply Phase}
    \As{a leader}
        \State collect $\signed{\commit,e,v}$ from $2t+1$ distinct replicas, denote the collection as $\Sigma$
        \State $\sigma\gets \thressign(\Sigma)$ %\algorithmiccomment{$\sigma$ is $\qcthree$}
        \State broadcast $\lr{\reply,e,v,\sigma}$
    \EndAs{}
    \As{a replica}
        \State wait for $\lr{\reply,e,v,\sigma}$ from leader \algorithmiccomment{$\qcthree$}
        \State output $v$ and send $\lr{\reply,e,v,\sigma}$ to the client
    \EndAs{}
    
    \State call procedure $\vc()$
    \EndWhile
    \State if a replica encounters timeout in any ``wait for'', call procedure $\vc()$
    \algstore{hotstuff} 
\end{algorithmic}
\end{algorithm*}

\begin{algorithm*}[t]
\begin{algorithmic}[1]
\algrestore{hotstuff} 
\Procedure{$\vc()$}{}
    \State broadcast $\signed{\blame,e}$
    \State collect $\signed{\blame,e}$ from $t+1$ distinct replicas, broadcast them
    \State quit this view
    \State send $\lr{\vc,e,\qctwo}$ to the next leader
    \State enter the next view, $e\gets e+1$
\EndProcedure
\Function{\textsc{Info}}{$var, \hqc$}\Comment{$var \in \{$`\hsa', `\hsb', `\hsc'$\}$}
    \If{$var = $`\hsa'}
        \State return $\hqc.e$
    \EndIf
    \If{$var = $`\hsb'}
        \State return $\text{Hash}(\hqc)$
    \EndIf
    \If{$var = $`\hsc'}
        \State return $\emptyset$
    \EndIf
\EndFunction

\end{algorithmic}
\end{algorithm*}

==> [CCS21] BFT Protocol Forensics/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> [CCS21] BFT Protocol Forensics/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> [CCS21] BFT Protocol Forensics/old/old_2_model.tex <==
\section{Problem Statement and Model}
\begin{table}[t]
    \centering
    \caption{Summary of notations.}
    \label{tab:notations}
    \begin{tabularx}{\columnwidth}{c|X} \toprule
        Symbol & \makecell{Interpretation}\\
        \toprule
        $n$ & total number of replicas\\
        \midrule
        $t$ & maximum number of faults for obtaining agreement and termination \\
        \midrule
        $f$ & actual number of faults\\
        \midrule
        $m$ & maximum number of Byzantine replicas under which forensic support can be provided\\
        \midrule
        $d$ & the number of Byzantine replicas that can be held culpable in case of an agreement violation\\
        \midrule
        $w$ & the number of witnesses who hold evidence for culpability\\\bottomrule
    \end{tabularx}
\end{table}

The goal of state machine replication (SMR) is to build a replicated service that takes requests from clients and provides the clients with the interface of a single non-faulty server, i.e., each client receives the same totally ordered sequence of values. To achieve this, the replicated service use multiple servers, also called replicas, some of which may be faulty. We are concerned with Byzantine faults where a faulty replica can behave arbitrarily. A state machine replication protocol needs to satisfy two guarantees:

\begin{itemize}[leftmargin=*, topsep=0pt]
    \item[-] \textbf{(Safety)} Any two honest replicas can only commit the same sequence of values.
    \item[-] \textbf{(Liveness)} Honest replicas keep committing values.
\end{itemize}

SMR setting also has external validity, i.e., replicas only commit values sent by clients. The replicas commit values and these commits are learned by the clients. Depending on the context, a replica may be interested in learning about commits too. Hence, whenever we refer to a client for learning purposes, it can be external entity or a server replica. We use $n$ to denote the total number of replicas and consider protocols that achieve safety and liveness when the actual number of Byzantine faults $f$ is less than or equal to an upper bound $t$. A table of notations is presented in Table~\ref{tab:notations}. %, Appendix~\ref{sec:tab:notations}.

Our protocols and our lower bound, for simplicity, consider the setting of committing a single value instead of a sequence of values. The safety and liveness properties from SMR can then be expressed using the following definition:
\begin{definition}[Validated Byzantine Agreement]
\label{defn:vba}
A protocol solves validated Byzantine agreement among $n$ replicas tolerating a maximum of $t$ faults, if it satisfies the following properties:
\begin{enumerate}[leftmargin=*, topsep=0pt]
    \item[] (Agreement) If the actual number of faults $f \leq t$ and any two honest replicas commit values $v$ and $v'$, then $v = v'$.
    \item[] (Validity) If an honest replica commits $v$, then $v$ is an externally valid value, i.e., $v$ is signed by a client.
    \item[] (Termination) If the actual number of faults $f \leq t$, all honest replicas start with externally valid values, and all messages sent among them have been delivered, then honest replicas will commit a value.
\end{enumerate}
\end{definition}


\myparagraph{Forensic support.} 
Traditionally, consensus protocols provide guarantees only when $f \leq t$. When $f > t$, there can be a safety or liveness violation. The goal of our work is to provide \emph{forensic support} whenever there is a safety violation and the number of Byzantine replicas in the system are not too high. In particular, if the actual number of Byzantine faults are bounded by $m$ (for some $m > t$) and there is a safety violation, we can detect $d$ Byzantine replicas with an irrefutable proof. Moreover, we use $w$ to denote the total number of honest replicas (witnesses) who have access to this proof.

To provide forensic support, we consider a setting where a client observes the existence of commits for two conflicting values. The client sends (possibly a subset of) these conflicting commits to all replicas. For a strong forensic support, even if it receives a response from one of the $w$ witnesses, it can obtain an irrefutable proof for the culpability of $d$ Byzantine replicas. 

\begin{definition}
\label{defn:forensic-support}
($(m,k,d)$-Forensic Support) If $t < f \leq m$ and two honest replicas commit conflicting values, then with the transcript of messages received by $k$ replicas during the protocol stored, a client can prove the culpability of $\geq d$ Byzantine replicas.
\end{definition}

Note that forensic support is an additional property provided to SMR/validated Byzantine agreement protocols, and hence, the notations $f$ and $t$ refer to the notations in those definitions. All of our upper bounds provide such a strong forensic support. In addition to an external client, a replica can also request for forensic support.

We provide a weaker definition of forensic support where a client can request the transcript of all replicas (including the Byzantine replicas). After receiving such a transcript, the client can determine $\geq d$ Byzantine replicas as irrefutably corrupt so far as the total number of Byzantine replicas is $\leq m$.

\begin{definition}
($(m,d)$-Weak Forensic Support) If $t < f \leq m$ and two honest replicas commit conflicting values, % $v$ and $v'$ such that $v \neq v'$, 
then the transcript of messages received by all replicas during the protocol can hold $\geq d$ Byzantine replicas undeniably culpable to a client.
\end{definition}

Observe that the definition is particularly strong; it expects the transcripts from all replicas, including the Byzantine faulty ones. In practice, the Byzantine replicas may have ``deleted'' some of these messages. However, we only use the weak definition to prove our lower bound (Section~\ref{sec:lb}). This makes our lower bound stronger -- it holds even if Byzantine replicas truthfully send all of their message transcripts.


\myparagraph{Comparing with Polygraph's definition.} The accountability definition in Polygraph~\cite{civit2019polygraph} requires the two honest replicas $i$ and $j$ who commit conflicting values to provide sufficient proof to detect $d = t+1$ culpable Byzantine replicas. In comparison, Definition~\ref{defn:forensic-support} allows a client to ask the replicas for a proof of culpability. Even one response from among the $w$ witnesses suffices. Looking ahead, we will see that protocols such as PBFT and HotStuff will have sufficiently many witnesses and hence, they provide robust forensic support.

\kartikold{example for }
\myparagraph{Other assumptions.}
We assume a partially synchronous network where there is an unknown time bound GST until which messages sent between replicas are only eventually delivered. After GST, all messages will arrive within a bounded delay $\Delta$ after they are sent. %\kartik{revisit if we have VABA}

We assume all messages are digitally signed. %\gerui{We don't need all messages are signed. In protocol I write signed messages and unsigned differently.} 
For forensic purposes, we assume the use of multi-signatures~\cite{bls}. Whenever the number of signatures exceeds a threshold, the resulting aggregate signature is denoted by a pair $\sigma = (\sigma_{agg}, \epsilon)$, where $\epsilon=[b_0,\cdots,b_{n-1}]$ is a bitmap indicating whose signatures are included in $\sigma_{agg}$. %\gerui{When the context is clear, we abuse the notation $\sigma$ by referring to the set of replicas who sign the messages.} \gerui{In this abusing notation, in forensic protocol we don't need $\sigma.\epsilon$.} 
We define the intersection of two aggregated messages to be the set of replicas who sign both messages, i.e., $\sigma \cap \sigma' := \{i|\sigma.\epsilon[i]\land \sigma'.\epsilon[i] = 1\}$. An aggregate signature serves as a quorum certificate (QC) in our protocols, and we will use the two terms interchangeably. We should note that for forensic purposes, we cannot use threshold signatures.

\ignore{
 Byzantine Agreement (BA), first introduced by [] solves the problem where $n$ replicas, at most $t$ of which are corrupted, want to agree on a single value based on everyone's input value. The problem is extended to fault tolerant state machine replication (SMR) when the purpose of deciding a value becomes to process a sequence of requests for clients. We consider a network consisting of $n$ replicas (each replica is a replica under the SMR setting), among them a subset of replicas $T\subset [n]$ are corrupted (called Byzantine replicas, coordinated by an adversary), any replica if not corrupted is called honest.

\subsubsection{External Clients} In SMR setting, clients send requests to all replicas and wait for the responses for the execution results. In BA setting, we also hope that values to agree on are practically meaningful, i.e. not a default value or values sent by rogue replicas. We introduce external clients also for BA, so that only values that are valid to clients can be decided. The formal definition of the extended Byzantine Agreement is as follows:



\subsubsection{Communication} We consider communication is authenticated and reliable, an honest replica $i$ will receive a message from an honest replica $j$ if and only if $j$ send a message to $i$. According to the message delay bound $\Delta$, there are three types of network. Synchronous model ensures each message arrives within a known bound $\Delta$, partially synchronous model has the same property only after an unknown global stabilization time $t_{GST}$. Before $t_{GST}$, the message delay is unknown for partially synchronous model, which is always the case when network is asynchronous. 

\subsubsection{Cryptographic Primitives} We use BLS signature for the sake of authentication. The messages would be signed by the secret key of the sender, and validated by its public key. In protocol, we use $\signed{\cdot}$ to denote a signed message. We use BLS multi-signature\cite{bls} to represent quorum certificate ($QC$), which is a collection of $(2t+1)$ votes for the same message. When a leader receives signatures over this threshold, it generates the aggregated message, denoted as a pair $\sigma = (\sigma_{agg}, \epsilon)$, where $\epsilon=[b_0,\cdots,b_{n-1}]$ is an ordered list of bits indicating whose signatures are included in $\sigma_{agg}$. We define the intersection of two aggregated messages to be the set of replicas who sign both messages, i.e. $\sigma \cap \sigma' := \{i|\sigma.\epsilon[i]\land \sigma'.\epsilon[i] = 1\}$. 
%Notation $\thresvalid()$, $\sharesign()$, $\thressign$.
%This provides similar message authentication except for negligible probability  compared to the assumption in \cite{vaba}. 
\subsubsection{Forensic Support} Traditional Byzantine fault tolerant protocols don't talk about what will happen when there are more than $t$ Byzantine replicas. Although safety is violated, we can still seek for some remedies, e.g., collect irrefutable evidence of bad behaviors. Sometimes evidence lies in one replica is not complete and all honest replicas need to work together to get it (termed ``weak forensic support"). In other cases, evidence can be provided by one replica, and multiple replicas may have the evidence at the same time (termed ``forensic support"). We formally define the forensic support a protocol can have as follows:

\begin{definition}
($(m,d)$-Weak Forensic Support) If $t < f \leq m$ and two honest replicas commit values $v$ and $v'$ such that $v \neq v'$, then the transcript of messages received by all replicas can hold $\geq d$ Byzantine replicas undeniably culpable to an external client.
\end{definition}
}

%\begin{definition}[Validated Byzantine Agreement with Weak Forensic Support]
%A validated Byzantine agreement satisfying Definition~\ref{defn:vba} is said to provide $(m,d)$-weak forensic support if when $t < f \leq m$, and two honest replicas commit values $v$ and $v'$ such that $v \neq v'$, then the transcript of messages received by all replicas can hold $\geq d$ Byzantine replicas undeniably culpable to an external client.
%\end{definition}





\ignore{
\begin{definition}[State Machine Replication with $(t,d)$-Forensic Support]
A protocol solves State Machine Replication (SMR) with forensic support among $n$ replicas and parameters $f, t,$ and $d$, if it satisfies the following properties:
\begin{enumerate}
    \item (Safety) If $\leq f$ out of $n$ replicas are Byzantine, honest replicas do not commit conflicting logs,
    \item (Liveness) If $\leq f$ out of $n$ replicas are Byzantine, each client request is eventually committed by all honest replicas,
    \item ($(t,d)$-Forensic Support) If $\leq t$ out of $n$ replicas are Byzantine and two honest replicas commit conflicting logs, then the information stored on the transcript from the two honest replicas can hold $\geq d$ Byzantine replicas undeniably culpable to the client.
\end{enumerate}
\end{definition}
}

==> [CCS21] BFT Protocol Forensics/old/old_3_pbft.tex <==
\section{PBFT has Strong Forensic Support}\label{sec:pbft}

\ignore{In this section, we show that PBFT has forensic support by cross-checking the transcripts of honest replicas internally or launching a simple message exchange phase by an external client.
\subsection{PBFT Overview}
PBFT Byzantine agreement protocol proceeds in consecutive views. In a view, there is a leader who broadcasts proposed value and other replicas vote for the value. If the leader is suspected to be failed, a view change will be triggered to make the protocol move on. There are three phases in the protocol when state is steady. In the first phase, leader proposes a value by broadcasting a \nv message, replicas send \vone if agree on the value. If the leader receives $n-t=2t+1$ \vone, it aggregates these messages to form a quorum certificate (QC) and broadcasts it inside a \prepare message in the second phase. The QC in this phase is called \qctwo. Replicas send \vtwo and lock on the value in phase two. In the third phase, $n-t$ \vtwo messages are aggregated to \qcthree and a \commit message is broadcast to replicas. Replicas who receive \commit message will decide on its value.
    
When suspecting a leader is failed, replicas send \vc messages, with current lock inside, to the next leader. Leader in the next view then collects $n-t$ \vc messages from distinct replicas (we assume there is a special \vc message for the first view) and select the highest locked value to propose.
}

PBFT is a classical partially synchronous consensus protocol that provides an optimal resilience of $t$ Byzantine faults out of $n = 3t+1$ replicas. However, when the actual number of faults $f$ exceeds $t$, it does not provide any safety or liveness. In this section, we argue that while PBFT does not provide these guarantees, in case of a safety violation, we can provide strong  \emph{forensic support} to detect the culpability of Byzantine replicas.

\subsection{Overview} We start with an overview of the protocol. For simplicity, we discuss a single-shot version of PBFT, i.e., a protocol for consensus on a single value. The protocol proceeds in a sequence of consecutive views where each view has a unique leader. Each view of PBFT progresses as follows:

\begin{itemize}[leftmargin=*, topsep=0pt]
    \item[-] \textbf{Propose.} The leader proposes a \nv message containing a proposal $v$ and a status certificate $M$ (explained later) to all replicas.
    \item[-] \textbf{\vone.} On receiving the first \nv message containing a valid value $v$ in a view $e$, a replica sends \vone for $v$ if it is \emph{safe} to vote based on a locking mechanism (explained later). It sends this vote to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qctwo. The leader sends \qctwo to all replicas.
    \item[-] \textbf{\vtwo.} On receiving a \qctwo in view $e$ containing message $v$, a replica locks on $(v, e)$ and sends \vtwo to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qcthree. The leader sends \qcthree to all replicas.
    \item[-] \textbf{\commit.} On receiving \qcthree from the leader, replicas commit $v$.
\end{itemize}

Once a replica locks on a given value $v$, it only votes for the value $v$ in subsequent views. The only scenario in which it votes for a value $v' \neq v$ is when the status certificate $M$ provides sufficient information stating that $2t+1$ replicas are not locked on $v$. At the end of a view, every replica sends its lock to the leader of the next view. The next view leader collects $2t+1$ such values as a status certificate $M$.

The safety of PBFT follows from two key quorum intersection arguments:

\myparagraph{Uniqueness within a view.} Within a view, safety is ensured by votes in either round. Since a replica only votes once for the first valid value it receives, by a quorum intersection argument, two conflicting values cannot both obtain \qcthree when $f \leq t$. %for two conflicting values $v$ and $v'$ to obtain \qctwo, each of them have been voted by $2t+1$ replicas. Any two quorums of size $2t+1$ intersect in $t+1$ replicas. Thus, if at most $t$ replicas are Byzantine, both $v$ and $v'$ cannot obtain \qctwo.

\myparagraph{Safety across views.} Safety across views is ensured by the use of locks and the status certificate. First, observe that if a replica $r$ commits a value $v$ in view $e$, then a quorum of replicas lock on $(v, e)$. When $f \le t$, this quorum includes a set $H$ of at least $t+1$ honest replicas. For any replica in $H$ to update to a higher lock, they need a \qctwo in a higher view $e' > e$, which in turn requires a vote from at least one of these honest replicas in view $e'$. %A pre-requisite for forming such a $\qctwo$ is to obtain $n-t$ votes in the view, which requires a vote from at least one honest replica in $H$. 
However, replicas in $H$ will vote for a conflicting value $v'$ in a higher view only if it is accompanied by a status certificate $M$ containing $2t+1$ locks that are not on value $v$. When $f \le t$, honest replicas in $M$ intersect with honest replicas in $H$  at least one replica -- this honest replica will not vote for a conflicting value $v'$.


\subsection{Forensic Support for PBFT}

The agreement property for PBFT holds only when $f \leq t$. When the number of faults are higher, this agreement property (and even termination) can be violated. In this section, we show how to provide forensic support for PBFT when the agreement property is violated. We show that, if two honest replicas commit on conflicting values $v$ and $v'$ due to the presence of $f > t$ Byzantine replicas, our forensic protocol can detect $t+1$ Byzantine replicas with an irrefutable proof. For each of the possible scenarios in which safety can be violated, the proof shows exactly what property of PBFT was not respected by the Byzantine replicas. We also show that the proof of safey violation is abundantly available: $2t+1-f$ replicas can act as witnesses with access to this proof. This shows the robustness of the protocol in terms of its forensic capability: if $f = t+1$, then there are about one-third witnesses, and even in the catastrophic scenario of $f = 2t$, there is still at least one witness.



\begin{figure}[htbp]
    \centering
    \vspace{-20pt}
    \includegraphics[width=0.75\columnwidth]{figures/pbft.pdf}
    \caption{\textbf{An example sequence of events in the PBFT protocol that leads to replicas $i$ and $j$ committing to a different sequence of values.}}
    \label{fig:pbft-disagree}
    \vspace{-20pt}
\end{figure}


\myparagraph{Intuition.} In order to build intuition, let us assume $n = 3t+1$ and $f = t+1$. Let us start with a simple scenario: two honest replicas commit values $v$ and $v'$ in the same view. It must then be the case that a \qcthree is formed for both $v$ and $v'$. Due to a quorum intersection argument, it must be the case that all replicas in the intersection have voted for two conflicting values to break the uniqueness property. Thus, all the replicas in the intersection are culpable. The \qcthree (as well as \qctwo) for the two conflicting values act as the irrefutable proof for detecting $t+1$ Byzantine replicas. %Moreover, there are sufficient witnesses -- since both values were committed in the same view, at least $2t+1$ replicas must have access to the \qctwo for each value. Out of these, at least $t$ replicas are honest.

When two honest replicas commit conflicting values in different views, there are many different sequence of events that could lead to such a disagreement. One such sequence is described in Figure~\ref{fig:pbft-disagree}. The replicas are split into three sets: the blue set and the green set are honest replicas each of size $t$  and the red replicas are Byzantine replicas of size $t+1$. 

\begin{itemize}[leftmargin=*, topsep=0pt]
    \item In view $e$, replica $i$ commits to $v$ due to $\vtwo$ from the honest blue set and the Byzantine red set. At the end of the view, replicas in the blue and red set hold locks $(v, e)$ whereas the green set holds a lower lock for a different value. 
    \item In the next few views, no higher locks are formed. Thus, the blue and the red set still hold locks $(v, e)$.
    \item Suppose $e^*$ is the first view where a higher lock is formed. At the start of this view, the leader received locks from the honest green set who hold lower-ranked locks and the Byzantine red set who maliciously send lower-ranked locks. The set of locks received by the leader is denoted by $M$ and suppose the highest lock was received  for $v'$. The leader proposes $v'$ along with $M$. This can make any honest replica ``unlock'' and vote for $v'$ and form quorum certificates in this view.
    \item In some later view $e'$, replica $j$ commits to $v'$.
\end{itemize}

With this sequence of events, let us try to answer the following questions: (1) Is this an admissible sequence of events? (2) How do we find the culpable Byzantine replicas? What does the irrefutable proof consist of? (3) Which honest replicas can act as witnesses for such a proof?

To answer the first question, the only non-trivial part in our example is the existence of a view $e^*$ where a higher lock is formed. However, such a view $e < e^* \leq e'$ must exist because replica $j$ commits in view $e'$ and a higher lock must be formed at the latest in view $e'$. % \kartik{comment about $e^*$}

For the second question, observe that both the red replicas as well as the green replicas sent locks lower than $(v, e)$ to the leader in $e^*$. However, only the red replicas also sent commit messages for value $v$ in view $e$. Thus, by intersecting the set of commit messages for value $v$ in view $e$ and the messages forming the status certificate sent to the leader of $e^*$, we can obtain a culpable set of $t+1$ Byzantine replicas. The proof indicates that the replicas sent a lower lock in view $e^*$ despite having access to a higher lock in a lower view $e$.

For the third question, in order to form a lock for value $v'$ in view $e^*$, at least $t$ honest replicas ($2t+1$ replicas overall) must have received the \nv message containing the status certificate $M$ in view $e^*$. These $t$ honest replicas can act as witnesses. 

\begin{algorithm}[htbp]
\begin{algorithmic}[1]
\As{a replica running PBFT}
\LeftComment{patch for PBFT}
    \ForInitialize{$e\ge 1$}
        \State $ledger[e]\gets \{\}$
        %\State \gerui{\pflock is no longer used  so should delete it}$\pflock[e]\gets \{\}$
        \EndForInitialize
    \Upon{$\lr{id,\nv,e,v,M}$ from the leader of view $e$}
        \State $\ledger[e]\gets (v,M)$
        %\algorithmiccomment{\textgreen{Save every \nv message in \ledger}}
     %   \State $e^*\gets$ the highest locked view in $M$
     %   \State $V\gets$ all locked values in $e^*$ from $M$ 
     %   \If{$|V|>1$} \label{alg1-9-twoM}
     %   \algorithmiccomment{\textgreen{Conflicting lock detected}}
     %       \State $qc, qc'\gets$ \qctwo for two values in $V$\label{alg1-10-twoM}
     %       \State send $\signed{\proofwithin, e, qc, qc'}$ to clients\label{alg1-11-twoM}
      %  \EndIf
    \EndUpon
 %   \Upon{$\lr{id,\prepare,e,v,\sigma}$ from any replica}
    %    \If{$(\pflock[e]\ne \{\}) \land (\pflock[e].v \ne v)$}\algorithmiccomment{\textgreen{Conflicting lock detected}}
     %       \State send $\lr{id,\proofwithin, e, \pflock[e].\sigma, \sigma}$ to clients
    %    \Else \algorithmiccomment{\textgreen{Save every \qctwo message in \pflock}}
           % \State $\pflock[e]\gets (v, \sigma)$\gerui{should delete it}
   % \EndUpon
    \Upon{$\lr{id,\conflictacross, e, v, \sigma}$ from a client}
        \For{all $e^* > e$, $\ledger[e^*]\ne \{\}$}\label{alg:pbft-10}
            \State $(e'',v'')\gets$ the highest lock in $\ledger[e^*].M$ \label{alg:line:conflict:1}
            \If{$ (v \ne v'')\land(e \ge e'')$} \label{alg:line:conflict:2}
            \algorithmiccomment{\textgreen{Conflicting ledger detected}}
                \State send $\lr{id,\proofacross, e^*, \ledger[e^*]}$ to clients \label{alg:pbft-13}
            \EndIf
        \EndFor
    \EndUpon
%    \gerui{Remove proof-within-view, also need to remove prepareQC, need to change ledger to use $\cup\{(v,M)\}$}
    % \Upon{$\lr{id,\conflictwithin, e, v, v'}$ from a client}
    %     \If{$\pflock[e]\ne \{\}$}
    %         \State send $\lr{id,\textsc{QC}, e, \pflock[e]}$ to the client
    %     \EndIf
    % \EndUpon
\EndAs{}

\As{a client}
    \Upon{two conflicting \commit messages}\label{alg:pbft-18}
        \If{the two \commit messages are from different views}
            \State $\lr{id,\commit,e,v,\sigma}\gets$ the message from lower view
            \State broadcast $\lr{id,\conflictacross, e, v, \sigma}$ \label{alg:pbft-21}
            \State wait for: $\lr{id,\proofacross, e^*, \ledger}$ s.t. $e^*>e$ and $\ledger$ is a conflicting ledger in view $e^*$. \algorithmiccomment{Check conflict as per line~\ref{alg:line:conflict:1}-\ref{alg:line:conflict:2}}
%            \gerui{Add the following if}
            \If{in $\ledger.M$ there are two lock $(e',v_1,\sigma_1)$ and $(e',v_2,\sigma_2)$ s.t. $v_1\neq v_2$} \label{alg:pbft-20-withinM}
            \State \textbf{output} $\sigma_1\cap \sigma_2$ \algorithmiccomment{\textgreen{Conflicting lock detected}}
            \Else
            \State \textbf{output} the intersection of senders in $\ledger.M$ and signers of $\sigma$.\label{alg:pbft-23} 
            \EndIf
        \Else\label{alg:pbft-25}\algorithmiccomment{\textgreen{Conflicting \qcthree detected}}
            \ignore{\State $v, v',e\gets$ two committed values and the view number
            \State broadcast $\lr{id,\conflictwithin, e, v, v'}$
            \State wait for: $qc, qc'\gets$ two \qctwo of committed values from possibly different replicas in view $e$.
            \State \textbf{output} $qc.\sigma \cap qc'.\sigma$}
            \State $\lr{id,\commit,e,v,\sigma}\gets$ first \commit message
            \State $\lr{id,\commit,e,v',\sigma'}\gets$ second \commit message
            \State \textbf{output} $\sigma \cap \sigma'$\label{alg:pbft-28}
        \EndIf
    \EndUpon
  %  \Upon{$\lr{id,\proofwithin, e, qc, qc'}$} 
   % \algorithmiccomment{\textgreen{sent by anyone}} % \kartik{doesn't matter who sends it, }
    %    \State \textbf{output} $qc \cap qc'$
  %  \EndUpon
    
\EndAs{}
\end{algorithmic}
\caption{Forensic protocol for PBFT Byzantine agreement: instance identifier~$id$}
\label{alg:fa-pbft1}
\end{algorithm}

\myparagraph{Forensic protocol.}
% The example in Figure~\ref{fig:pbft-disagree} is just one example of a sequence of events. 
Algorithm~\ref{alg:fa-pbft1} describes the entire protocol to obtain forensic support atop PBFT. For completeness, we also provide a complete description of the PBFT protocol in Algorithm~\ref{alg:single-pbft}. Each replica maintains a \emph{ledger} containing the value proposed and the status certificate $M$ obtained in the \nv message of view $e$. %If a replica observes locks for two conflicting values from the same view $e^*$ in status certificate $M$ (lines~\ref{alg1-9-twoM}), then the replicas can immediately flag this as a culpability proof to an external client. The culpability proof consists of the two conflicting locks from the same view. Since each lock consists of $2t+1$ signatures, at least $t+1$ replicas must have signed for conflicting values in the same view.
If a client observes commits for two conflicting values, then it first checks if the two values are committed in the same view (line~\ref{alg:pbft-18}). If yes, then any two \qcthree for the two different committed values can provide culpability proof for at least $t+1$ replicas (lines~\ref{alg:pbft-25}-\ref{alg:pbft-28}). Otherwise, the client picks the value that was committed in a lower view and sends $\signed{\conflictacross, e, v, \sigma}$ to all replicas to request a proof of culpability from witnesses (lines~\ref{alg:pbft-21}). Each replica looks through its ledgers for views $> e$. If there exists a ledger of the smallest view $e^* > e$ such that the status certificate $M$ contains the highest lock for a conflicting value $v''$, it sends $\ledger[e^*]$ to the client (lines~\ref{alg:pbft-10}-\ref{alg:pbft-13}). If inside $M$ there are conflicting locks in the same view, the intersection of them proves at least $t+1$ culprits (line~\ref{alg:pbft-20-withinM}), otherwise the intersection of $M$ and the \qcthree proves at least $t+1$ culprits (line~\ref{alg:pbft-23}).

\ignore{
Suppose replicas $i$ and $j$ commit to conflicting values $v$ and $v'$. Suppose replica $i$ commits first in view $e$ and replica $j$ commits in a later view $e'$. In PBFT, replica $i's$ commit must be guarded by $2t+1$ replicas who hold locks on $v$. When the number of faults are few $(f \leq t)$, the honest replicas among them ensure that no other value is proposed in a subsequent view. In our case, $f = t+1$ and this does not hold anymore. Suppose $2t+1$ replicas include the Byzantine red set and the honest blue set; thus at the end of view $e$, the highest lock that these replicas hold is for $(v, e)$. Honest replicas in the green set may have a lower lock (say $(v', e'')$) at the end of view $e$. 

What about replica $j$? We know that $j$ commits a conflicting value $v'$ in some higher view $e'$. Such a commit implies that there are $2t+1$ replicas (at least $t$ honest replicas) are locked on a different value $v'$ in view $e'$, and more importantly a higher lock for a conflicting value $v'$ is formed. Between views $e$ and $e'$, there may exist many such views where a lock for a value other than $v$ is formed. This may not necessarily be view $e+1$. In order to find culpable replicas, let us consider the first such view $e^*$ and the \nv message (proposal) sent in this view. Recall that the honest blue replicas and the Byzantine red replicas were responsible for guarding the safety of $i$'s commit. However, in our example, the leader of view $e^*$ receives locks from the Byzantine red replicas and the honest green replicas. In this case, the Byzantine replicas incorrectly send a lower lock and the honest green replicas may only have access to a lower lock. With this a (possibly honest) leader in view $e^*$


\myparagraph{How to disagree.} The safety of PBFT is guaranteed by $f<t$, when $f>t$, the adversary can violate the uniqueness within the view. It splits the honest replicas into two part, send \qctwo for one value to the first replica and send \qctwo for another value to the second replica. Each replica will vote for their values and then commit on corresponding values. Such attack is easy to detect by comparing the information within the view. Another potential attack is to construct a higher lock after some honest replica's committing. For example in Fig. \ref{fig:pbft-disagree}, an honest replica $i$ commits in view $e$ on value $v$. At the end of view $e$, $f$ honest replicas (blue replicas) are locked on $(v,e)$ while another $f$ honest replicas (red replicas) are locked on an older lock $(v',e''), e''<e$. In some view $e^*$ after $e$, a Byzantine replica can collect locks from $f$ red replicas, generate a \nv message proposing $v'$ and broadcast it to red replicas. Since the highest lock in \nv is for value $v'$, red replicas are happy to vote for it, a higher lock of $v'$ will be formed. This lock can either be used to make some red replica commit in this view, or change the lock of blue replicas later. A second commit can happen anytime afterwards.
}


\subsection{Proof for Forensic Support}

The following theorem shows that so far as up to $f \leq 2t$ replicas are Byzantine and safety violation occurs, Algorithm~\ref{alg:fa-pbft1} can be used to irrefutably detect $t+1$ Byzantine replicas. The proof indicates the Byzantine action performed by a detected Byzantine replica. Moreover, $2t+1-f$ honest witnesses have access to such a proof.

\ignore{
A disagreement in PBFT may happen when one replica $i$ is first committed on a value $v$ locally, then another replica $j$ commits a distinct value $v'$ afterwards. It is possible since no matter the second replica is locked on $v$ or not when $i$ commits, Byzantine replicas can generate a higher lock by equivocating to control the lock of $j$. We first prove that if disagreement happens, PBFT has forensic support to detect equivocating behaviors.}

\kartikold{note for myself: possibly change all notations}
%\kartik{mention need for aggregate signatures and not threshold}
\begin{theorem}
\label{thm:pbft}
For $n=3t+1$, if two honest replicas commit to conflicting values, PBFT provides $(2t,\ 2t+1-f,\ t+1)$-forensic support as per Definition~\ref{defn:forensic-support}.
\end{theorem}
\begin{proof}
Suppose values $v$ and $v'$ are committed in views $e$ and $e'$ respectively. 

\myparagraph{Case $e=e'$.} 

\noindent\underline{Culpability.} The quorums \qcthree  for $v$ and \qcthree  for $v'$ intersect in $t+1$ replicas. These $t+1$ replicas should be Byzantine since the protocol requires a replica to vote for at most one value in a view. 

% \kartik{who knows it? check} \peiyao{Do these replicas receive \qctwo for another value from clients?}

\noindent\underline{Witnesses.} Client can get the proof based on the two \commit messages, so additional witnesses are not necessary in this case.%For each of $v$ and $v'$, since $2t+1$ replicas have sent a commit message, both values' $\qctwo$ are available to some $2t+1-f$ honest replicas.

\ignore{
If $e\ne e'$, w.l.o.g, we assume $e < e'$. That $v$ is committed in $e$ indicates $2t+1$ replicas have lock $(v, e)$ at the end of view $v$. Now consider the first view $e < e^* \le e'$ in which a higher lock $(v', e^*)$ forms. Such view must exist since $v'$ is committed in $e'$. Since this is the first view $e^*>e$ where a lock for $v'$ forms, the highest lock in \nv message sent by the leader in this view must have view $e'' \le e$, which means the highest lock is $(v', e''), e''\le e$. Thus, the intersection of $2t+1$ locks in the \nv of $e^*$ and $2t+1$ commit messages in view $e$ contains at least $t+1$ equivocating replicas.

Since a higher lock $(v', e^*)$ forms, at least $2t+1$ replicas receive the \nv message and vote in this view, among them at least $2t+1-f$ are honest, thus all these replicas can get the above evidence for equivocating replicas.

---------
}
\myparagraph{Case $e\neq e'$.}

\noindent\underline{Culpability.}
If $e \neq e'$, then WLOG, suppose $e < e'$. Since $v$ is committed in view $e$, it must be the case that $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$. Now consider the first view $e < e^* \leq e'$ in which a higher lock $(v'', e^*)$ is formed (not necessarily known to any honest party) where $v'' \neq v$ (possibly $v'' = v'$). Such a view must exist since $v'$ is committed in view $e' > e$ and a lock will be formed in at least view $e'$. Consider the status certificate $M$ sent by the leader of view $e^*$ in its \nv message. $M$ must contain $2t+1$ locks; each of these locks must be from view $e'' \le e$, and a highest lock among them is $(v'', e'')$. % Otherwise, \kartik{explain not first} 

We consider two cases based on whether the status message contains a lock $(v''', e)$ for a value $v''' \neq v''$. The two cases are (i) there does not exist a such a lock $(v''', e)$, and (ii) there exists such a lock $(v''', e)$. %\peiyao{Shall these $e$ in this paragraph be $e''$?}

\ignore{if $e'' = e$ then $v'$ is the only highest lock, if $e'' < e$, there could be more such high locks.}
For the first case, the status certificate $M$ with $2t+1$ locks intersect with the $2t+1$ signers of \qcthree  in view $e$ at $t+1$ Byzantine replicas. These replicas are Byzantine because they had a lock in view $e$ that was different from, and at least as high as the one sent to the leader of view $e^* > e$.

For the second case, since $v''$ is proposed in view $e^*$, it exists in the status certificate $M$ and is a highest lock in $M$. Moreover, in this case, $(v''', e)$ exists in $M$ too. Both of these locks were formed in view $e$. The two quorums forming the two locks in view $e$ intersect in $t+1$ replicas. These replicas are Byzantine since they voted for more than one value in view $e$.%\gerui{I think the protocol (Alg 1) doesn't capture this case. I think we need to add some actions after line 22.}

\noindent\underline{Witnesses.} Since a higher lock $(v'', e^*)$ is formed in view $e^*$, at least $2t+1$ replicas have voted for $v''$ in view $e^*$. These replicas must have received the \nv message and at most $f$ among them are Byzantine. Thus, all of these $2t+1-f$ replicas are witnesses who have access to the status certificate $M$.
\end{proof}

%\kartik{start from here -- do not read these paragraphs.}
%The proof of Theorem \ref{thm:pbft} indicates that if two values are committed in two different views, there must exist honest replicas who will receive equivocating messages between two views. The first scheme is to broadcast messages internally. We make these changes to the PBFT protocol,
%\begin{enumerate}
%    \item Upon receiving a \commit message, save and echo the message.
%    \item Upon receiving a \nv message, save the status collection.
%    \item For each status collection received from view $e$, pick the highest lock $(v^*, e^*)$, check all \commit messages committing on $(v', e')$ before $e$, if $e^* < e'$ and $v^* \ne v'$, broadcast the \vc message and status collection.
%\end{enumerate}
%The second scheme is executed by external clients. With PBFT protocol unchanged, if an client receives two conflicting \commit messages, it broadcasts them and wait for responses. Then honest replicas will check all status collections and at least one honest replica will get the evidence and send it back to the client.


% \kartik{need to change locks to explicitly have signatures?}







==> [CCS21] BFT Protocol Forensics/old/old_4_hotstuff.tex <==
\section{HotStuff has Strong Forensic Support}
\label{sec:basic-hotstuff}
HotStuff~\cite{yin2019hotstuff} is a partially synchronous consensus protocol that provides optimal resiliency of $t<n/3$. The HotStuff protocol is similar to PBFT but there are subtle differences which allow it to obtain a linear communication complexity for both its steady state and view change protocols (assuming the presence of threshold signatures). Looking ahead, these differences significantly change the way forensics is conducted if a safety violation happens.

\subsection{Overview}  We start with an overview of the protocol. For simplicity, we discuss a single-shot version of HotStuff. The protocol proceeds in a sequence of consecutive views where each view has a unique leader. Each view of HotStuff progresses as follows:
% \kartik{witness definition}
\begin{itemize}[leftmargin=*, topsep=0pt]
    \item[-] \textbf{Propose.} The leader proposes a \nv message containing a proposal $v$ along with the highest \qctwo known to it and sends it to all replicas.
    \item[-] \textbf{\vone.} On receiving a \nv message containing a valid value $v$ in a view $e$ and a \qctwo message, a replica sends \vone for $v$ if it is \emph{safe} to vote based on a locking mechanism (explained later). It sends this vote to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qctwo in view $e$. The leader sends the view $e$ \qctwo to all replicas.
    \item[-] \textbf{\vtwo.} On receiving a \qctwo in view $e$ containing message $v$, a replica updates its highest \qctwo to $(v, e)$ and sends \vtwo to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qcprecom.
    \item[-] \textbf{\vthree.} On receiving \qcprecom in view $e$ containing message $v$ from the leader, a replica locks on $(v, e)$ and sends \vthree to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qcthree.
    \item[-] \textbf{\commit.} On receiving \qcthree from the leader, replicas commit to the value $v$.
\end{itemize}

Once a replica locks on a given value $v$, it only votes for the value $v$ in subsequent views. The only scenario in which it votes for a value $v' \neq v$ is when it observes a \qctwo from a higher view in a \nv message. At the end of a view, every replica sends its highest \qctwo to the leader of the next view. The next view leader collects $2t+1$ such values and picks the highest \qctwo.

The safety and liveness of HotStuff when $f \leq t$ follows from the following:

\myparagraph{Uniqueness within a view.} Since replicas only vote once in each round, a \qcthree can be formed for only one value when $f \leq t$.

\myparagraph{Safety and liveness across views.} Safety across views is ensured by the use of locks and the voting rule for a \nv message. Whenever a replica commits a value, at least $2t+1$ other replicas are locked on the value in the view. Observe that compared to PBFT, there is no status certificate $M$ in the \nv message to ``unlock'' a replica. Thus, a replica only votes for the value it is locked on. The only scenario in which it votes for a conflicting value $v'$ is if the leader includes a \qctwo for $v'$ from a higher view in \nv message. This indicates that at least $2t+1$ replicas are not locked on $v$ in a higher view, and hence it should be safe to vote for it. The latter constraint of voting for $v'$ is not necessary for safety, but only for liveness of the protocol.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/hotstuff-diff.pdf}
    \caption{\textbf{Depiction of events in the HotStuff protocol for the first two views where a higher \qctwo for $v'$ is formed.}} %\kartik{In this example, why should $e^*$ be the view of interest. It can be that $e^\#$ was the view where first prepareQC containing culpable act was formed, and in a higher view $e^{\#\#}< e^*$, a new view message with prepareQC from $e^\#$ was sent. Shouldn't receivers of the NewView message of $e^{\#\#}$ contain the witnesses and not $e^*$?}} %  Replicas in the red ellipse contain culpable Byzantine replicas. Replicas in the blue ellipse and (honest) replicas in the red ellipse have access to $\qctwo$ and the \nv message respectively.}
    \label{fig:hotstuff-diff}
\end{figure}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/hotstuff-equal.pdf}
    \caption{\textbf{Depiction of events in the HotStuff protocol for the first view where a higher \qctwo and lock are formed in the same view.}} %  Replicas in the red ellipse contain culpable Byzantine replicas. Replicas in the blue ellipse and (honest) replicas in the red ellipse have access to $\qctwo$ and the \nv message respectively.}
    \label{fig:hotstuff-equal}
\end{figure}

\subsection{Forensic Support for HotStuff}

Similar to PBFT, our forensic protocol on HotStuff can detect $t+1$ Byzantine replicas when the number of Byzantine faults is $f \leq 2t$. We make a simple modification to the message structure in HotStuff~\cite[Algorithm~2]{yin2019hotstuff} which ensures that there are at least $2t+1-f$ witnesses can individually prove the culpability.

\myparagraph{Intuition.} If two conflicting values are committed in the same view, Byzantine replicas can be detected using \qcthree  and using ideas similar to that in PBFT. However, when the conflicting commits of replicas $i$ and $j$ are across views $e$ and $e'$ for $e < e'$, the same ideas do not hold anymore. To understand this, observe that the two key ingredients for proving the culpability of Byzantine replicas in PBFT were (i) a \qcthree  for the value committed in a lower view (denoted by $\sigma$ for replica $i$'s commit in Figure~\ref{fig:pbft-disagree}) and (ii) a status certificate from the first view higher than $e$ containing the locks from $2t+1$ replicas (denoted by $M$ for view $e^* > e$ in Figure~\ref{fig:pbft-disagree}). In HotStuff, a \qcthree still exists. However, for communication efficiency reasons, HotStuff does not include a status certificate $M$ in its \nv message. The status certificate in PBFT provides us with the following:

\begin{itemize}[leftmargin=*, topsep=0pt]
    \item \textbf{Identifying a potential set of culpable replicas.} Depending on the contents of $M$ and knowing $\sigma$, we could identify a set of Byzantine replicas.
    \item \textbf{Determining whether the view is the first view where a higher lock for a conflicting value is formed.} By inspecting all the locks in $M$, we can easily determine this. Ensuring first view with a higher lock is important; once a higher lock is formed, even honest replicas may update their locks and the proof of Byzantine behavior may not exist in the messages in subsequent views.
\end{itemize}

Unfortunately, with HotStuff, the leader does not broadcast $M$. Our goal is to find witnesses who have access to the information contained in $M$ (as described in the bullets above). %this information. 


Let us try to understand this based on the first view $e^\#$ where a higher \qctwo is formed for $v'\ne v$. If the first higher lock for $v'$ is also formed in $e^* = e^\#$ (see Figure~\ref{fig:hotstuff-equal}), then $2t+1$ replicas (denoted by the blue ellipse) have access to \qctwo for a conflicting value in view $e^\#$. Otherwise, consider the second \qctwo which is formed in $e^{\#\#}$ where $e^\#<e^{\#\#}\le e^*$ (see Figure~\ref{fig:hotstuff-diff}), $2t+1$ replicas in blue ellipse who receive the \nv message have access to \qctwo formed in $e^\#$. The set of replicas who sent \vone (the red ellipse) in $e^\#$ and formed this \qctwo are our potential set of Byzantine replicas. Why? If $e^\#$ is indeed the first view in which a higher \qctwo is formed, then all of these replicas voted for a \nv message containing a \qctwo from a lower or equal view $e''$ on a different value. If any of these replicas also held a lock $(v, e)$ (by voting for replica $i$'s commit) then these replicas have committed the culpable act of not respecting the voting rule. Thus, the blue set of replicas are witnesses who help determine a red set of potentially culpable replicas.

\ignore{
Let us try to understand this based on the first view $e^*$ where a higher lock is formed and the first view $e^\#$ where the corresponding \qctwo is formed. For intuition, a graphical representation is depicted in Figure~\ref{fig:hotstuff-case} for the case where $e^\# < e^*$. The special case when $e^\# = e^*$ is depicted in Figure~\ref{fig:hotstuff-case2}.\kartik{figure numbers are in reverse? perhaps we should keep just the generic figure?} Formation of a higher lock implies that $2t+1$ replicas (denoted by the blue ellipse) have access to \qctwo for a conflicting value in view $e^*$, which is either contained in \nv message when $e^\# < e^*$ or contained in \prepare message when $e^\# = e^*$.\kartik{check my comment in figure 2. is $e^*$ where a lock is formed the view of interest here?} The set of replicas who sent \vone (the red ellipse) in $e^\#$ and formed this \qctwo are our potential set of Byzantine replicas. Why? If $e^\#$ is indeed the first view in which a higher \qctwo is formed, then all of these replicas voted for a \nv message containing a \qctwo from a lower or equal view $e''$. If any of these replicas also held a lock $(v, e)$ (by voting for replica $i$'s commit) then these replicas have committed the culpable act of not respecting the voting rule. Thus, the blue set of replicas are witnesses who help determine a red set of potentially culpable replicas.
}
\ignore{
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{false-alarm.pdf}
    \caption{\textbf{Byzantine leader can create fake \nv message to accuse honest replicas.}} %  Replicas in the red ellipse contain culpable Byzantine replicas. Replicas in the blue ellipse and (honest) replicas in the red ellipse have access to $\qctwo$ and the \nv message respectively.}
    \label{fig:hotstuff-false}
\end{figure}
}

The only remaining part is to ensure that this is indeed the first view where a higher conflicting \qctwo is formed. To detect this, we include the view number where \qctwo was formed in \vone messages (in the $\eqc$ field). %\peiyao{To detect this, we include $\eqc$, the view number of \qctwo in \nv message, whenever replicas send \vone.} 
When the leader collects enough \vone messages, the new \qctwo contains $\eqc$ too. This explicitly states the message they vote for and provides the necessary link to show culpable behavior.

\ignore{
\noindent {\bf Importance of this minor modification to Hotstuff}. \peiyao{If the extra information $\eqc$ is not included, the client can not determine whether received \qctwo is indeed formed in the first view, except it receives the \nv message in the same view. If the client asks replicas for the \nv message, Byzantine replicas can send a fake \nv message to the client to implicate honest replicas. An example is depicted in Figure~\ref{fig:hotstuff-false}: consider the first view $e^\#$ where a higher \qctwo for $v'$ is formed and the first view $e^*$ where a higher lock for $v'$ is formed. The Byzantine leader in view $e^*>e^\#$ sends a \nv message containing the \qctwo formed in $e^\#>e$ to replicas, since there is no lock higher than $e$ formed yet, $2t+1$ honest replicas will send \vone then a new \qctwo for $v'$ is formed. Since $v'\ne v$, this \qctwo should be sent to the client -- at this time, the Byzantine leader creates a fake \nv message containing the \qctwo formed in $e''\le e$ to the client to pretend that $e^*$ is the first view where a higher \qctwo is formed. If the client is convinced that $2t+1$ honest replicas vote for the fake \nv message, honest replicas who also vote for the first \commit message will be implicated as culprits.}
}


Thus, to summarize, the red set of replicas in view $e^\#$ are a potential set of culpable nodes of size $2t+1$. The blue set acts as witnesses and a client needs a proof of culpability from the blue set. Since there are $f$ actual faults, the number of honest replicas with such a proof is $2t+1-f$. 

\myparagraph{Comparison to the two HotStuff protocols.} We note that adding $\eqc$ in the vote is a modification to the basic HotStuff protocol described in \cite[Algorithm~2]{yin2019hotstuff}. The modification is only relevant to the forensic capability. Interestingly, the chained version of their protocol~\cite[Algorithm~3]{yin2019hotstuff} does include similar information, enabling forensics directly.

\begin{algorithm}[htbp]
\begin{algorithmic}[1]
\As{a replica running HotStuff}
\LeftComment{patch for HotStuff}
    \ForInitialize{$e\ge 1$}
        % \State $ledger[e]\gets \{\}$
        \State $\pflock[e]\gets \{\}$
        \EndForInitialize
    \Upon{$\lr{id,\nv,e,v,L}$ from the leader of view $e$}
        \State $(e', v', \sigma, \eqc)\gets L $\Comment{Note that $L$ has selectors $e,v,\sigma,\eqc$\ignore{ $= (e, v, \sigma, \eqc)$}} 
        \State $\pflock[e'] \gets  \pflock[e']\cup \{(v', \sigma, \eqc)\}$\label{alg:hotstuff-6}
    \EndUpon
    \Upon{$\lr{id,\prepare,e,v,\sigma,\eqc}$ from the leader of view $e$}
        \State $\pflock[e]\gets \pflock[e]\cup \{(v, \sigma,\eqc)\}$\label{alg:hotstuff-6-2}
    \EndUpon
    \Upon{$\lr{id,\conflictacross, e, v, \sigma, e'}$ from a client}
        \For{all $e<e^\#\le e'$}
            % \If{$(\ledger[e^*]\ne \{\})\land(\ledger[e^*].L.e\le e)\land(\ledger[e^*].v\neq v)$}
            %     \State send $\lr{id,NV, e^*, \ledger[e^*]}$ to the client\label{alg:hotstuff-12}
            % \EndIf
            \For{$qc\in \pflock[e^\#]$} % \kartik{what is this iterating over? $pflock$ is a list of votes?}\gerui{a malicious leader could send multiple prepareQC in a view, hence it is a list of prepareQC}
            \If{$(qc.v\neq v)\land (qc.\eqc\le e)$} % \kartik{check $\eqc = e$ case, is the proof the same?}
                \State send $\lr{id,\proofacross, e^\#, qc}$ to the client\label{alg:hotstuff-12} %\kartik{$\textsc{QC}$ is undefined.}\gerui{changed to \proofacross}
            \EndIf
            \EndFor
        \EndFor
    \EndUpon
    % \Upon{$\lr{id,\conflictwithin, e, v, v'}$ from a client}
    %     \If{$\pflock[e]\ne \{\}$}
    %         \State send $\lr{id,\proofacross, e, \pflock[e]}$ to the client\label{alg:hotstuff-17}
    %     \EndIf
    % \EndUpon
\EndAs{}

\As{a client}
    \Upon{two conflicting \commit messages}
        \If{the two \commit messages are from different views}\label{alg1:28}
            \State $\lr{id,\commit,e,v,\sigma}\gets$ the message from lower view
            \State $e'\gets$ the view number of message from higher view
            \State broadcast $\lr{id,\conflictacross, e, v, \sigma, e'}$ \label{alg:hotstuff-23}
            \State wait for  $\lr{id,\proofacross, e^\#, qc}$ s.t.
            \begin{enumerate}[leftmargin=1in]
                \item[(1)] $e<e^\#\le e'$, and\label{alg:hotstuff-24}
                \item[(2)] $(qc.v\neq v)\land (qc.\eqc\le e)$
                %\item[(3)] check signature, (do we need to mention it?) %
            \end{enumerate}%\gerui{wait for a matching pair of $\lr{id,NV, e^*, m},\lr{id,\proofacross, e^*, qc}$ s.t. 1) $e<e^*\le e'$ 2) $m.H.e \le e\wedge\ m.v\neq v$ and 3) the hash of $m.H$ matches that in $qc$}
            \State \textbf{output} $qc.\sigma \cap \sigma$\label{alg:hotstuff-26}
\label{alg:hotstuff-25}
        \Else \label{alg:hotstuff-28}
            \State $\lr{id,\commit,e,v,\sigma}\gets$ first \commit message
            \State $\lr{id,\commit,e,v',\sigma'}\gets$ second \commit message
            \State \textbf{output} $\sigma \cap \sigma'$
            % \State $v, v',e\gets$ two committed values and the view number
            % \State broadcast $\lr{id,\conflictwithin, e, v, v'}$\label{alg:hotstuff-28}
            % \State wait for: $qc, qc'\gets$ two \qctwo of committed values from possibly different replicas in view $e$.\label{alg:hotstuff-29}
            % \State \textbf{output} $qc.\sigma \cap qc'.\sigma$
        \EndIf
    \EndUpon
\EndAs{}
\end{algorithmic}
\caption{Forensic protocol for Basic HotStuff}
\label{alg:fa-hotstuff-modified}
\end{algorithm}


\myparagraph{Forensic protocol.}
% The example in Figure~\ref{fig:pbft-disagree} is just one example of a sequence of events. 
Algorithm~\ref{alg:fa-hotstuff-modified} describes the entire protocol to obtain forensic support atop HotStuff. A complete description of the HotStuff protocol is also provided in Algorithm~\ref{alg:single-hotstuff-modified}. Each replica maintains a list of \pflock containing all received \qctwo from \prepare messages and \nv messages (line~\ref{alg:hotstuff-6},\ref{alg:hotstuff-6-2}). %\kartik{this line is confusing}\gerui{use PlaceHolder, is it good now? we can change latex command to change its name}
If a client observes commits for two conflicting values in the same view, it can determine the culprits by two \commit messages (line~\ref{alg:hotstuff-28}).  Otherwise, the client sends a request to all replicas for possible proof between two committed views $e, e'$ for $e<e'$ (line~\ref{alg:hotstuff-23}). Each replica looks through its list for views $e<e^\#\le e'$. If there exists a \qctwo whose value is different from the value $v$ committed in $e$ and recorded $\eqc$ is less than or equal to $e$, it sends a reply with this \qctwo to the client (line~\ref{alg:hotstuff-12}). The client waits for a \qctwo (line~\ref{alg:hotstuff-24}) from $e^\#$ between two committed views. If it contains a different value from the first committed value and an older view number $\eqc < e$, the intersection of this \qctwo and the \qcthree from the commit message in the lower view proves at least $t+1$ culprits (line~\ref{alg:hotstuff-26}).

\subsection{Proof for Forensic Support}

The following theorem provides the necessary culpability proof for HotStuff.

\begin{theorem}
\label{thm:hotstuff}
For $n=3t+1$, if two honest replicas commit to conflicting values, HotStuff provides $(2t,\ 2t+1-f,\ t+1)$-forensic support as per Definition~\ref{defn:forensic-support}.
\end{theorem}
\begin{proof}
Suppose two conflicting values $v,\ v'$ are committed in views $e$, $e'$ respectively. 

\myparagraph{Case $e=e'$.}

\noindent\underline{Culpability.} The \qcthree of $v$ and \qcthree of $v'$ intersect in $t+1$ replicas. These $t+1$ replicas should be Byzantine since the protocol requires a replica to vote for at most one value in a view. 

\noindent\underline{Witnesses.} Client can get the proof by itself when receiving two \commit messages, so witnesses are not necessary in this case. %For each of $v$ and $v'$, since $2t+1$ replicas have sent a \vtwo message, both values' $\qctwo$ are available to some $2t+1-f$ honest replicas.

\myparagraph{Case $e\neq e'$.}

\noindent\underline{Culpability.}
If $e \neq e'$, then WLOG, suppose $e < e'$. Since $v$ is committed in view $e$, it must be the case that $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$. Now consider the first view $e < e^* \leq e'$ in which a higher lock $(v'', e^*)$ is formed where $v''\ne v$ (possibly $v''=v'$). Such a view must exist since $v'$ is committed in view $e' > e$ and a lock will be formed in at least % \gerui{at latest? I think at least means $\ge$ but we actually mean $\le$. Section 3 also has this word.} 
view $e'$. For a lock to be formed, a higher \qctwo must be formed too. Consider the first view $e<e^\# \leq e'$ in which the corresponding \qctwo for $v''$ is formed. The leader in $e^\#$ broadcasts the \nv message containing a \qctwo on $(v'', e'')$ (the highest QC collected from other replicas). Since this is the first time a higher \qctwo is formed and there is no higher \qctwo for $v''$ formed between view $e$ and $e^\#$, we have $e''\le e$. The formation of the higher \qctwo indicates that $2t+1$ replicas received the \nv message proposing $v''$ with \qctwo on $(v'', e'')$ and consider it a valid proposal, i.e., the view number $e''$ is larger than their locks because the value is different. 

\ignore{A lock for $v''$ is formed in $e^*$ only under two cases: 1) If $e^\# = e^*$, the leader collects $2t+1$ \vtwo messages which form a \qcprecom, so that $2t+1$ replicas receive \qctwo; 2) If $e^\# < e^*$, consider the second view  $e^{\#\#}$ where a \qctwo for $v''$ \kartik{a value $\neq v$ is formed?} is formed, $2t+1$ replicas receive \qctwo contained in the \nv message in $e^{\#\#}$ (and send \vone). In both cases $2t+1$ replicas receive the \qctwo, which contains $2t+1$ \vone messages including $\eqc = e''$, indicating that $2t+1$ replicas received the \nv message proposing $v''$ with \qctwo on $(v'', e'')$ and consider it a valid proposal, i.e., the view number $e''$ is larger than their locks because the value is different. \gerui{I think this para belongs to witnesses.}}

 Recall that the committed value $v$ indicates $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$. In this case, the $2t+1$ votes in \qctwo in view $e^\#$ intersect with the $2t+1$ votes in \qcthree in view $e$ at $t+1$ Byzantine replicas. These replicas should be Byzantine because they were locked on value $v$ in view $e$ and vote for a value $v'' \neq v$ in a higher view $e^\#$ when the \nv message contained a \qctwo from a  view $e'' \leq e$. Thus, they have violated the voting rule.
\ignore{If $e \neq e'$, then WLOG, suppose $e < e'$. Since $v$ is committed in view $e$, it must be the case that $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$. Now consider the first view $e < e^* \leq e'$ in which a higher lock $(v'', e^*)$ is formed where $v''\ne v$ (possibly $v''=v'$) and the first view $e < e^\# \leq e'$ in which the corresponding \qctwo for $v''$ is formed. Such views must exist since $v'$ is committed in view $e' > e$ and a lock will be formed in at least view $e'$. Consider the \qctwo on $(v'', e'')$ sent by the leader of view $e^\#$ in its \nv message. Since there is no lock formed between view $e$ and $e^*$ (other than lock on $v$), we have $e''\le e$.

A lock for $v''$ is formed in $e^*$ only under two cases: 1) If $e^\# = e^*$, the leader collects $2t+1$ \vtwo messages which form a \qcprecom, so that $2t+1$ replicas receive \qctwo; 2) If $e^\# < e^*$, $2t+1$ replicas receive \qctwo contained in \nv message in $e^*$ and after two-round voting a lock is formed. In both cases $2t+1$ replicas receive the \qctwo, which contains $2t+1$ \vone messages including the view number $\eqc = e''$ in \nv message, indicating that $2t+1$ replicas received the \nv message proposing $v''$ with \qctwo on $(v'', e'')$ and considered it a valid proposal, i.e., the view number $e''$ is larger than their locks because the value is different. \kartik{However, this is not true since $e'' < e$ and $2t+1$ replicas are locked on $v$ at the end of view $e$.}

Recall that the committed value $v$ indicates $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$. In this case, the $2t+1$ votes in \qctwo in view $e^\#$ intersect with the $2t+1$ votes in \qcthree in view $e$ at $t+1$ Byzantine replicas. These replicas should be Byzantine because they were locked on value $v$ in view $e$ and vote for a value $v'' \neq v$ in a higher view $e^\#$ when the \nv message contained a \qctwo from a  view $e'' \leq e$. Thus, they have violated the voting rule.}


\noindent\underline{Witnesses.} Since a higher lock $(v'', e^*)$ is formed in view $e^*$, there are two possible cases: 1) If $e^\# = e^*$, the leader collects $2t+1$ \vtwo messages which form a \qcprecom, so that $2t+1$ replicas receive \qctwo; 2) If $e^\# < e^*$, consider the second view $e^{\#\#}$ (possibly $= e^*$) where a \qctwo for $v''$ is formed, $2t+1$ replicas receive the \nv message (containing the \qctwo formed in $e^\#$). In both cases $2t+1$ replicas receive the \qctwo, at most $f$ among which are Byzantine. Thus, all of these $2t+1-f$ replicas are witnesses who have access to the required proof.
\end{proof} 




==> [CCS21] BFT Protocol Forensics/old/old_7_Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
In this paper, we have embarked on a systematic study of the forensic properties of BFT protocols and demonstrated strong forensics properties for a few popular protocols. In this section, we discuss the implications, extensions and possible future research following up on our results. 

\myparagraph{Chained consensus.} In this paper, we have focused on Validated Byzantine Agreement, a core consensus formalism for {\em single-shot} consensus in a state machine replication (SMR) system. SMR protocols (blockchains) extend this to serve consensus for a sequence of values. For instance, in protocols such as chained HotStuff (\cite[Algorithm~3]{yin2019hotstuff}) adopted by Libra, SBFT~\cite{gueta2019sbft} adopted by Concord, and Streamlet~\cite{chan2020streamlet}, the consensus protocol decides on a sequence of decision values. The sequence of values can either be treated independently (like in SBFT) or chained by hash pointers (like in chained HotStuff). When treated independently, it may be essential for replicas to exchange and maintain additional metadata information (e.g., $e_{qc}$ in HotStuff). Chained protocols, on the other hand, may maintain this metadata in the chain itself. In fact, the availability of this information on the chain may be a requirement for a replica to make progress. This strong availability requirement may enable a stronger forensic support, where we just require a replica to provide (part of) the chain and metadata rather than a specific witness to provide a specific evidence. For instance, in chained HotStuff, we would have the crucial \qctwo of view $e^{\#}$ on the chain itself. Thus a client can query (even Byzantine) replicas for the chain between $e$ and $e'$ and find the desired \qctwo somewhere on the chain. This may make it easier to identify culprits on the chain. Generally speaking, if a protocol has forensic support and all supporting evidence (e.g., quorum certificates) are put on chain, then a client can query the chain from replicas and identify culprits exclusively on the chain.

\myparagraph{Implementation details matter.} A second observation is that minor details matter when it comes to BFT protocol forensics. Consider three different versions of the HotStuff protocol: (i) The one described in Algorithm~\ref{alg:single-hotstuff-modified}, (ii) The one described in \cite[Algorithm~2]{yin2019hotstuff}, and (iii) the one in Algorithm~\ref{alg:single-hotstuff-modified} without sending $e_{qc}$ along with votes. While all three variants embody the key contribution of HotStuff to make the protocol achieve linear communication (assuming threshold signatures), all three of them have different forensic capabilities. We have shown that the variant described in Algorithm~\ref{alg:single-hotstuff-modified} has strong forensic capability. The variant from \cite[Algorithm~2]{yin2019hotstuff} has forensic capability but requires communicating to two types of witnesses, and there exist $2t+1-f$ witnesses of each type. Essentially, in addition to the witness in Algorithm~\ref{alg:single-hotstuff-modified}, we need  another witness holding information about $e_{qc}$ to determine the first time a \qctwo is formed in a higher view. Using the two witnesses, and the fact that the blocks are linked through hashes, culpable nodes can be determined. Finally, the variant from Algorithm~\ref{alg:single-hotstuff-modified} with $e_{qc}$ not being sent as a part of the votes has no forensic support. The lack of information about $e_{qc}$ with witnesses, and the absence of hash-links between blocks does not allow a client to determine \emph{whether a view was the first view} where a higher conflicting \qctwo was formed. 

%\kartik{Sreeram, do you want to take a stab at the $t > 2n/3$ setting?}

%\myparagraph{Future work.} A final consideration is on the generality of our results. Our work has focused on three protocols, two of which are in the partially synchronous setting and one in the asynchronous setting. In all cases, we observed that, ignoring simple modifications, all these protocols have strong forensic support. Based on these results, a natural question is: what are the requirements to make any protocol have strong forensic support? As an example, all of the protocols we considered used digital signatures. Whether we can achieve any guarantees for protocols relying only on authenticated channels is an open question. Moreover, all of our techniques were for protocols tolerating $< 1/3$ faults. Whether we can achieve forensic support for protocols tolerating a larger fraction (e.g., synchronous protocols) is still an open question. %\kartik{I am not sure if we should include this paragraph. Both of these are juicy open questions that we should work on straightaway!}

\ignore{
{\bf Para 1}. In this paper we have focused on Validated Byzantine Agreement, a core consensus formalism. In blockchain applications, this core protocol is adapted to serve consensus for a sequential setting. {\em Discuss chained VBA protocols via an example. Give the example of Hotstuff being used in Libra. Now ask how forensics changes in this context (even definition might change?) and point out some basic results (ideally blackbox -- if VBA has a certain forensic support then the chained version in a blockchain also has the following forensic support properties (this should be stated as a proposition). If this para becomes too long it should be a whole section in itself. Note that proofs can be moved to appendix. }
\gerui{In protocols such as Chained HotStuff (Algorithm~3~\cite{yin2019hotstuff}) and Streamlet~\cite{chan2020streamlet}, the consensus protocol decides on a sequence of decision values that are chained by hash pointers. Sometimes, metadata such as  quorum certificates are also put on chain, as in Chained HotStuff. Libra project adopts LibraBFT~\cite{}, a consensus protocol based on Chained HotStuff, as its core consensus protocol. Comparing simplistic single-shot Byzantine agreement to practical chained SMR protocols, a distinctive difference is that in chained SMR protocols, the entire chain and metadata, from genesis to up-to-date chain tip, have to be made available to a replica in order for it to make progress. This strong availability requirement enables a stronger forensics support, where we just require a replica to provide (part of) the chain and metadata rather than a specific witness to provide a specific evidence. Take the HotStuff case in Figure~\ref{fig:hotstuff-case} as an example: in Chained HotStuff we would have the crucial \qctwo of view $e^*$ on chain for $e<e^*\le e'$, thus a client can query (even Byzantine) replicas for the chain between $e$ and $e'$ and find that \qctwo somewhere on the chain. Generally speaking, if a protocol has forensic support and all quorum certificates are put on chain, then a client can query the chain from replicas and identify culprits exclusively on chain.}

{\bf Para 2}. Emphasize that we needed a minor change to Hotstuff. Its a trivial change, no difference in complexity but makes a crucial difference for forensic capability. (note: how come David's paper is claiming some forensics support for Hotstuff directly? Is their result wrong? Not worth pointing it out in paper, but good for us to know internally.) Ask if there is a way to bring this modification systematically to any BFT protocol to improve forensic support without changing complexity or security properties. {Kartik: any ideas here? I feel you might have something very smart to say here. } 

{\bf Para 3}. What happens when $t> 2f/3$? Note that in synchronous setting, one can securely design consensus against 99\% adversarial resistance. Compare with polygraph here. 


{\bf Para 4}. Forensic support of other VBA protocols. Point out that we covered different network conditions (partially synchronous, asynchronous) and classical/efficient protocols in both settings and find that (with minor implementation level modifications) they already have strong forensic support. Two questions are natural: (1)  whether all VBA protocols also have strong forensic support  (with potentially minor implementatino level modifications)? (2) how about VBA protocols that dont use digital signatures -- but instead rely on authenticated channels? (3) how about VBA protocols in synchronous setting where t is strictly smaller than 50\% (eg: 40\%)? (are there even examples of such protocols???). 
}


==> old/old_2_model.tex <==
\section{Problem Statement and Model}
\begin{table}[t]
    \centering
    \caption{Summary of notations.}
    \label{tab:notations}
    \begin{tabularx}{\columnwidth}{c|X} \toprule
        Symbol & \makecell{Interpretation}\\
        \toprule
        $n$ & total number of replicas\\
        \midrule
        $t$ & maximum number of faults for obtaining agreement and termination \\
        \midrule
        $f$ & actual number of faults\\
        \midrule
        $m$ & maximum number of Byzantine replicas under which forensic support can be provided\\
        \midrule
        $d$ & the number of Byzantine replicas that can be held culpable in case of an agreement violation\\
        \midrule
        $w$ & the number of witnesses who hold evidence for culpability\\\bottomrule
    \end{tabularx}
\end{table}

The goal of state machine replication (SMR) is to build a replicated service that takes requests from clients and provides the clients with the interface of a single non-faulty server, i.e., each client receives the same totally ordered sequence of values. To achieve this, the replicated service use multiple servers, also called replicas, some of which may be faulty. We are concerned with Byzantine faults where a faulty replica can behave arbitrarily. A state machine replication protocol needs to satisfy two guarantees:

\begin{itemize}[leftmargin=*, topsep=0pt]
    \item[-] \textbf{(Safety)} Any two honest replicas can only commit the same sequence of values.
    \item[-] \textbf{(Liveness)} Honest replicas keep committing values.
\end{itemize}

SMR setting also has external validity, i.e., replicas only commit values sent by clients. The replicas commit values and these commits are learned by the clients. Depending on the context, a replica may be interested in learning about commits too. Hence, whenever we refer to a client for learning purposes, it can be external entity or a server replica. We use $n$ to denote the total number of replicas and consider protocols that achieve safety and liveness when the actual number of Byzantine faults $f$ is less than or equal to an upper bound $t$. A table of notations is presented in Table~\ref{tab:notations}. %, Appendix~\ref{sec:tab:notations}.

Our protocols and our lower bound, for simplicity, consider the setting of committing a single value instead of a sequence of values. The safety and liveness properties from SMR can then be expressed using the following definition:
\begin{definition}[Validated Byzantine Agreement]
\label{defn:vba}
A protocol solves validated Byzantine agreement among $n$ replicas tolerating a maximum of $t$ faults, if it satisfies the following properties:
\begin{enumerate}[leftmargin=*, topsep=0pt]
    \item[] (Agreement) If the actual number of faults $f \leq t$ and any two honest replicas commit values $v$ and $v'$, then $v = v'$.
    \item[] (Validity) If an honest replica commits $v$, then $v$ is an externally valid value, i.e., $v$ is signed by a client.
    \item[] (Termination) If the actual number of faults $f \leq t$, all honest replicas start with externally valid values, and all messages sent among them have been delivered, then honest replicas will commit a value.
\end{enumerate}
\end{definition}


\myparagraph{Forensic support.} 
Traditionally, consensus protocols provide guarantees only when $f \leq t$. When $f > t$, there can be a safety or liveness violation. The goal of our work is to provide \emph{forensic support} whenever there is a safety violation and the number of Byzantine replicas in the system are not too high. In particular, if the actual number of Byzantine faults are bounded by $m$ (for some $m > t$) and there is a safety violation, we can detect $d$ Byzantine replicas with an irrefutable proof. Moreover, we use $w$ to denote the total number of honest replicas (witnesses) who have access to this proof.

To provide forensic support, we consider a setting where a client observes the existence of commits for two conflicting values. The client sends (possibly a subset of) these conflicting commits to all replicas. For a strong forensic support, even if it receives a response from one of the $w$ witnesses, it can obtain an irrefutable proof for the culpability of $d$ Byzantine replicas. 

\begin{definition}
\label{defn:forensic-support}
($(m,k,d)$-Forensic Support) If $t < f \leq m$ and two honest replicas commit conflicting values, then with the transcript of messages received by $k$ replicas during the protocol stored, a client can prove the culpability of $\geq d$ Byzantine replicas.
\end{definition}

Note that forensic support is an additional property provided to SMR/validated Byzantine agreement protocols, and hence, the notations $f$ and $t$ refer to the notations in those definitions. All of our upper bounds provide such a strong forensic support. In addition to an external client, a replica can also request for forensic support.

We provide a weaker definition of forensic support where a client can request the transcript of all replicas (including the Byzantine replicas). After receiving such a transcript, the client can determine $\geq d$ Byzantine replicas as irrefutably corrupt so far as the total number of Byzantine replicas is $\leq m$.

\begin{definition}
($(m,d)$-Weak Forensic Support) If $t < f \leq m$ and two honest replicas commit conflicting values, % $v$ and $v'$ such that $v \neq v'$, 
then the transcript of messages received by all replicas during the protocol can hold $\geq d$ Byzantine replicas undeniably culpable to a client.
\end{definition}

Observe that the definition is particularly strong; it expects the transcripts from all replicas, including the Byzantine faulty ones. In practice, the Byzantine replicas may have ``deleted'' some of these messages. However, we only use the weak definition to prove our lower bound (Section~\ref{sec:lb}). This makes our lower bound stronger -- it holds even if Byzantine replicas truthfully send all of their message transcripts.


\myparagraph{Comparing with Polygraph's definition.} The accountability definition in Polygraph~\cite{civit2019polygraph} requires the two honest replicas $i$ and $j$ who commit conflicting values to provide sufficient proof to detect $d = t+1$ culpable Byzantine replicas. In comparison, Definition~\ref{defn:forensic-support} allows a client to ask the replicas for a proof of culpability. Even one response from among the $w$ witnesses suffices. Looking ahead, we will see that protocols such as PBFT and HotStuff will have sufficiently many witnesses and hence, they provide robust forensic support.

\kartikold{example for }
\myparagraph{Other assumptions.}
We assume a partially synchronous network where there is an unknown time bound GST until which messages sent between replicas are only eventually delivered. After GST, all messages will arrive within a bounded delay $\Delta$ after they are sent. %\kartik{revisit if we have VABA}

We assume all messages are digitally signed. %\gerui{We don't need all messages are signed. In protocol I write signed messages and unsigned differently.} 
For forensic purposes, we assume the use of multi-signatures~\cite{bls}. Whenever the number of signatures exceeds a threshold, the resulting aggregate signature is denoted by a pair $\sigma = (\sigma_{agg}, \epsilon)$, where $\epsilon=[b_0,\cdots,b_{n-1}]$ is a bitmap indicating whose signatures are included in $\sigma_{agg}$. %\gerui{When the context is clear, we abuse the notation $\sigma$ by referring to the set of replicas who sign the messages.} \gerui{In this abusing notation, in forensic protocol we don't need $\sigma.\epsilon$.} 
We define the intersection of two aggregated messages to be the set of replicas who sign both messages, i.e., $\sigma \cap \sigma' := \{i|\sigma.\epsilon[i]\land \sigma'.\epsilon[i] = 1\}$. An aggregate signature serves as a quorum certificate (QC) in our protocols, and we will use the two terms interchangeably. We should note that for forensic purposes, we cannot use threshold signatures.

\ignore{
 Byzantine Agreement (BA), first introduced by [] solves the problem where $n$ replicas, at most $t$ of which are corrupted, want to agree on a single value based on everyone's input value. The problem is extended to fault tolerant state machine replication (SMR) when the purpose of deciding a value becomes to process a sequence of requests for clients. We consider a network consisting of $n$ replicas (each replica is a replica under the SMR setting), among them a subset of replicas $T\subset [n]$ are corrupted (called Byzantine replicas, coordinated by an adversary), any replica if not corrupted is called honest.

\subsubsection{External Clients} In SMR setting, clients send requests to all replicas and wait for the responses for the execution results. In BA setting, we also hope that values to agree on are practically meaningful, i.e. not a default value or values sent by rogue replicas. We introduce external clients also for BA, so that only values that are valid to clients can be decided. The formal definition of the extended Byzantine Agreement is as follows:



\subsubsection{Communication} We consider communication is authenticated and reliable, an honest replica $i$ will receive a message from an honest replica $j$ if and only if $j$ send a message to $i$. According to the message delay bound $\Delta$, there are three types of network. Synchronous model ensures each message arrives within a known bound $\Delta$, partially synchronous model has the same property only after an unknown global stabilization time $t_{GST}$. Before $t_{GST}$, the message delay is unknown for partially synchronous model, which is always the case when network is asynchronous. 

\subsubsection{Cryptographic Primitives} We use BLS signature for the sake of authentication. The messages would be signed by the secret key of the sender, and validated by its public key. In protocol, we use $\signed{\cdot}$ to denote a signed message. We use BLS multi-signature\cite{bls} to represent quorum certificate ($QC$), which is a collection of $(2t+1)$ votes for the same message. When a leader receives signatures over this threshold, it generates the aggregated message, denoted as a pair $\sigma = (\sigma_{agg}, \epsilon)$, where $\epsilon=[b_0,\cdots,b_{n-1}]$ is an ordered list of bits indicating whose signatures are included in $\sigma_{agg}$. We define the intersection of two aggregated messages to be the set of replicas who sign both messages, i.e. $\sigma \cap \sigma' := \{i|\sigma.\epsilon[i]\land \sigma'.\epsilon[i] = 1\}$. 
%Notation $\thresvalid()$, $\sharesign()$, $\thressign$.
%This provides similar message authentication except for negligible probability  compared to the assumption in \cite{vaba}. 
\subsubsection{Forensic Support} Traditional Byzantine fault tolerant protocols don't talk about what will happen when there are more than $t$ Byzantine replicas. Although safety is violated, we can still seek for some remedies, e.g., collect irrefutable evidence of bad behaviors. Sometimes evidence lies in one replica is not complete and all honest replicas need to work together to get it (termed ``weak forensic support"). In other cases, evidence can be provided by one replica, and multiple replicas may have the evidence at the same time (termed ``forensic support"). We formally define the forensic support a protocol can have as follows:

\begin{definition}
($(m,d)$-Weak Forensic Support) If $t < f \leq m$ and two honest replicas commit values $v$ and $v'$ such that $v \neq v'$, then the transcript of messages received by all replicas can hold $\geq d$ Byzantine replicas undeniably culpable to an external client.
\end{definition}
}

%\begin{definition}[Validated Byzantine Agreement with Weak Forensic Support]
%A validated Byzantine agreement satisfying Definition~\ref{defn:vba} is said to provide $(m,d)$-weak forensic support if when $t < f \leq m$, and two honest replicas commit values $v$ and $v'$ such that $v \neq v'$, then the transcript of messages received by all replicas can hold $\geq d$ Byzantine replicas undeniably culpable to an external client.
%\end{definition}





\ignore{
\begin{definition}[State Machine Replication with $(t,d)$-Forensic Support]
A protocol solves State Machine Replication (SMR) with forensic support among $n$ replicas and parameters $f, t,$ and $d$, if it satisfies the following properties:
\begin{enumerate}
    \item (Safety) If $\leq f$ out of $n$ replicas are Byzantine, honest replicas do not commit conflicting logs,
    \item (Liveness) If $\leq f$ out of $n$ replicas are Byzantine, each client request is eventually committed by all honest replicas,
    \item ($(t,d)$-Forensic Support) If $\leq t$ out of $n$ replicas are Byzantine and two honest replicas commit conflicting logs, then the information stored on the transcript from the two honest replicas can hold $\geq d$ Byzantine replicas undeniably culpable to the client.
\end{enumerate}
\end{definition}
}

==> old/old_3_pbft.tex <==
\section{PBFT has Strong Forensic Support}\label{sec:pbft}

\ignore{In this section, we show that PBFT has forensic support by cross-checking the transcripts of honest replicas internally or launching a simple message exchange phase by an external client.
\subsection{PBFT Overview}
PBFT Byzantine agreement protocol proceeds in consecutive views. In a view, there is a leader who broadcasts proposed value and other replicas vote for the value. If the leader is suspected to be failed, a view change will be triggered to make the protocol move on. There are three phases in the protocol when state is steady. In the first phase, leader proposes a value by broadcasting a \nv message, replicas send \vone if agree on the value. If the leader receives $n-t=2t+1$ \vone, it aggregates these messages to form a quorum certificate (QC) and broadcasts it inside a \prepare message in the second phase. The QC in this phase is called \qctwo. Replicas send \vtwo and lock on the value in phase two. In the third phase, $n-t$ \vtwo messages are aggregated to \qcthree and a \commit message is broadcast to replicas. Replicas who receive \commit message will decide on its value.
    
When suspecting a leader is failed, replicas send \vc messages, with current lock inside, to the next leader. Leader in the next view then collects $n-t$ \vc messages from distinct replicas (we assume there is a special \vc message for the first view) and select the highest locked value to propose.
}

PBFT is a classical partially synchronous consensus protocol that provides an optimal resilience of $t$ Byzantine faults out of $n = 3t+1$ replicas. However, when the actual number of faults $f$ exceeds $t$, it does not provide any safety or liveness. In this section, we argue that while PBFT does not provide these guarantees, in case of a safety violation, we can provide strong  \emph{forensic support} to detect the culpability of Byzantine replicas.

\subsection{Overview} We start with an overview of the protocol. For simplicity, we discuss a single-shot version of PBFT, i.e., a protocol for consensus on a single value. The protocol proceeds in a sequence of consecutive views where each view has a unique leader. Each view of PBFT progresses as follows:

\begin{itemize}[leftmargin=*, topsep=0pt]
    \item[-] \textbf{Propose.} The leader proposes a \nv message containing a proposal $v$ and a status certificate $M$ (explained later) to all replicas.
    \item[-] \textbf{\vone.} On receiving the first \nv message containing a valid value $v$ in a view $e$, a replica sends \vone for $v$ if it is \emph{safe} to vote based on a locking mechanism (explained later). It sends this vote to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qctwo. The leader sends \qctwo to all replicas.
    \item[-] \textbf{\vtwo.} On receiving a \qctwo in view $e$ containing message $v$, a replica locks on $(v, e)$ and sends \vtwo to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qcthree. The leader sends \qcthree to all replicas.
    \item[-] \textbf{\commit.} On receiving \qcthree from the leader, replicas commit $v$.
\end{itemize}

Once a replica locks on a given value $v$, it only votes for the value $v$ in subsequent views. The only scenario in which it votes for a value $v' \neq v$ is when the status certificate $M$ provides sufficient information stating that $2t+1$ replicas are not locked on $v$. At the end of a view, every replica sends its lock to the leader of the next view. The next view leader collects $2t+1$ such values as a status certificate $M$.

The safety of PBFT follows from two key quorum intersection arguments:

\myparagraph{Uniqueness within a view.} Within a view, safety is ensured by votes in either round. Since a replica only votes once for the first valid value it receives, by a quorum intersection argument, two conflicting values cannot both obtain \qcthree when $f \leq t$. %for two conflicting values $v$ and $v'$ to obtain \qctwo, each of them have been voted by $2t+1$ replicas. Any two quorums of size $2t+1$ intersect in $t+1$ replicas. Thus, if at most $t$ replicas are Byzantine, both $v$ and $v'$ cannot obtain \qctwo.

\myparagraph{Safety across views.} Safety across views is ensured by the use of locks and the status certificate. First, observe that if a replica $r$ commits a value $v$ in view $e$, then a quorum of replicas lock on $(v, e)$. When $f \le t$, this quorum includes a set $H$ of at least $t+1$ honest replicas. For any replica in $H$ to update to a higher lock, they need a \qctwo in a higher view $e' > e$, which in turn requires a vote from at least one of these honest replicas in view $e'$. %A pre-requisite for forming such a $\qctwo$ is to obtain $n-t$ votes in the view, which requires a vote from at least one honest replica in $H$. 
However, replicas in $H$ will vote for a conflicting value $v'$ in a higher view only if it is accompanied by a status certificate $M$ containing $2t+1$ locks that are not on value $v$. When $f \le t$, honest replicas in $M$ intersect with honest replicas in $H$  at least one replica -- this honest replica will not vote for a conflicting value $v'$.


\subsection{Forensic Support for PBFT}

The agreement property for PBFT holds only when $f \leq t$. When the number of faults are higher, this agreement property (and even termination) can be violated. In this section, we show how to provide forensic support for PBFT when the agreement property is violated. We show that, if two honest replicas commit on conflicting values $v$ and $v'$ due to the presence of $f > t$ Byzantine replicas, our forensic protocol can detect $t+1$ Byzantine replicas with an irrefutable proof. For each of the possible scenarios in which safety can be violated, the proof shows exactly what property of PBFT was not respected by the Byzantine replicas. We also show that the proof of safey violation is abundantly available: $2t+1-f$ replicas can act as witnesses with access to this proof. This shows the robustness of the protocol in terms of its forensic capability: if $f = t+1$, then there are about one-third witnesses, and even in the catastrophic scenario of $f = 2t$, there is still at least one witness.



\begin{figure}[htbp]
    \centering
    \vspace{-20pt}
    \includegraphics[width=0.75\columnwidth]{figures/pbft.pdf}
    \caption{\textbf{An example sequence of events in the PBFT protocol that leads to replicas $i$ and $j$ committing to a different sequence of values.}}
    \label{fig:pbft-disagree}
    \vspace{-20pt}
\end{figure}


\myparagraph{Intuition.} In order to build intuition, let us assume $n = 3t+1$ and $f = t+1$. Let us start with a simple scenario: two honest replicas commit values $v$ and $v'$ in the same view. It must then be the case that a \qcthree is formed for both $v$ and $v'$. Due to a quorum intersection argument, it must be the case that all replicas in the intersection have voted for two conflicting values to break the uniqueness property. Thus, all the replicas in the intersection are culpable. The \qcthree (as well as \qctwo) for the two conflicting values act as the irrefutable proof for detecting $t+1$ Byzantine replicas. %Moreover, there are sufficient witnesses -- since both values were committed in the same view, at least $2t+1$ replicas must have access to the \qctwo for each value. Out of these, at least $t$ replicas are honest.

When two honest replicas commit conflicting values in different views, there are many different sequence of events that could lead to such a disagreement. One such sequence is described in Figure~\ref{fig:pbft-disagree}. The replicas are split into three sets: the blue set and the green set are honest replicas each of size $t$  and the red replicas are Byzantine replicas of size $t+1$. 

\begin{itemize}[leftmargin=*, topsep=0pt]
    \item In view $e$, replica $i$ commits to $v$ due to $\vtwo$ from the honest blue set and the Byzantine red set. At the end of the view, replicas in the blue and red set hold locks $(v, e)$ whereas the green set holds a lower lock for a different value. 
    \item In the next few views, no higher locks are formed. Thus, the blue and the red set still hold locks $(v, e)$.
    \item Suppose $e^*$ is the first view where a higher lock is formed. At the start of this view, the leader received locks from the honest green set who hold lower-ranked locks and the Byzantine red set who maliciously send lower-ranked locks. The set of locks received by the leader is denoted by $M$ and suppose the highest lock was received  for $v'$. The leader proposes $v'$ along with $M$. This can make any honest replica ``unlock'' and vote for $v'$ and form quorum certificates in this view.
    \item In some later view $e'$, replica $j$ commits to $v'$.
\end{itemize}

With this sequence of events, let us try to answer the following questions: (1) Is this an admissible sequence of events? (2) How do we find the culpable Byzantine replicas? What does the irrefutable proof consist of? (3) Which honest replicas can act as witnesses for such a proof?

To answer the first question, the only non-trivial part in our example is the existence of a view $e^*$ where a higher lock is formed. However, such a view $e < e^* \leq e'$ must exist because replica $j$ commits in view $e'$ and a higher lock must be formed at the latest in view $e'$. % \kartik{comment about $e^*$}

For the second question, observe that both the red replicas as well as the green replicas sent locks lower than $(v, e)$ to the leader in $e^*$. However, only the red replicas also sent commit messages for value $v$ in view $e$. Thus, by intersecting the set of commit messages for value $v$ in view $e$ and the messages forming the status certificate sent to the leader of $e^*$, we can obtain a culpable set of $t+1$ Byzantine replicas. The proof indicates that the replicas sent a lower lock in view $e^*$ despite having access to a higher lock in a lower view $e$.

For the third question, in order to form a lock for value $v'$ in view $e^*$, at least $t$ honest replicas ($2t+1$ replicas overall) must have received the \nv message containing the status certificate $M$ in view $e^*$. These $t$ honest replicas can act as witnesses. 

\begin{algorithm}[htbp]
\begin{algorithmic}[1]
\As{a replica running PBFT}
\LeftComment{patch for PBFT}
    \ForInitialize{$e\ge 1$}
        \State $ledger[e]\gets \{\}$
        %\State \gerui{\pflock is no longer used  so should delete it}$\pflock[e]\gets \{\}$
        \EndForInitialize
    \Upon{$\lr{id,\nv,e,v,M}$ from the leader of view $e$}
        \State $\ledger[e]\gets (v,M)$
        %\algorithmiccomment{\textgreen{Save every \nv message in \ledger}}
     %   \State $e^*\gets$ the highest locked view in $M$
     %   \State $V\gets$ all locked values in $e^*$ from $M$ 
     %   \If{$|V|>1$} \label{alg1-9-twoM}
     %   \algorithmiccomment{\textgreen{Conflicting lock detected}}
     %       \State $qc, qc'\gets$ \qctwo for two values in $V$\label{alg1-10-twoM}
     %       \State send $\signed{\proofwithin, e, qc, qc'}$ to clients\label{alg1-11-twoM}
      %  \EndIf
    \EndUpon
 %   \Upon{$\lr{id,\prepare,e,v,\sigma}$ from any replica}
    %    \If{$(\pflock[e]\ne \{\}) \land (\pflock[e].v \ne v)$}\algorithmiccomment{\textgreen{Conflicting lock detected}}
     %       \State send $\lr{id,\proofwithin, e, \pflock[e].\sigma, \sigma}$ to clients
    %    \Else \algorithmiccomment{\textgreen{Save every \qctwo message in \pflock}}
           % \State $\pflock[e]\gets (v, \sigma)$\gerui{should delete it}
   % \EndUpon
    \Upon{$\lr{id,\conflictacross, e, v, \sigma}$ from a client}
        \For{all $e^* > e$, $\ledger[e^*]\ne \{\}$}\label{alg:pbft-10}
            \State $(e'',v'')\gets$ the highest lock in $\ledger[e^*].M$ \label{alg:line:conflict:1}
            \If{$ (v \ne v'')\land(e \ge e'')$} \label{alg:line:conflict:2}
            \algorithmiccomment{\textgreen{Conflicting ledger detected}}
                \State send $\lr{id,\proofacross, e^*, \ledger[e^*]}$ to clients \label{alg:pbft-13}
            \EndIf
        \EndFor
    \EndUpon
%    \gerui{Remove proof-within-view, also need to remove prepareQC, need to change ledger to use $\cup\{(v,M)\}$}
    % \Upon{$\lr{id,\conflictwithin, e, v, v'}$ from a client}
    %     \If{$\pflock[e]\ne \{\}$}
    %         \State send $\lr{id,\textsc{QC}, e, \pflock[e]}$ to the client
    %     \EndIf
    % \EndUpon
\EndAs{}

\As{a client}
    \Upon{two conflicting \commit messages}\label{alg:pbft-18}
        \If{the two \commit messages are from different views}
            \State $\lr{id,\commit,e,v,\sigma}\gets$ the message from lower view
            \State broadcast $\lr{id,\conflictacross, e, v, \sigma}$ \label{alg:pbft-21}
            \State wait for: $\lr{id,\proofacross, e^*, \ledger}$ s.t. $e^*>e$ and $\ledger$ is a conflicting ledger in view $e^*$. \algorithmiccomment{Check conflict as per line~\ref{alg:line:conflict:1}-\ref{alg:line:conflict:2}}
%            \gerui{Add the following if}
            \If{in $\ledger.M$ there are two lock $(e',v_1,\sigma_1)$ and $(e',v_2,\sigma_2)$ s.t. $v_1\neq v_2$} \label{alg:pbft-20-withinM}
            \State \textbf{output} $\sigma_1\cap \sigma_2$ \algorithmiccomment{\textgreen{Conflicting lock detected}}
            \Else
            \State \textbf{output} the intersection of senders in $\ledger.M$ and signers of $\sigma$.\label{alg:pbft-23} 
            \EndIf
        \Else\label{alg:pbft-25}\algorithmiccomment{\textgreen{Conflicting \qcthree detected}}
            \ignore{\State $v, v',e\gets$ two committed values and the view number
            \State broadcast $\lr{id,\conflictwithin, e, v, v'}$
            \State wait for: $qc, qc'\gets$ two \qctwo of committed values from possibly different replicas in view $e$.
            \State \textbf{output} $qc.\sigma \cap qc'.\sigma$}
            \State $\lr{id,\commit,e,v,\sigma}\gets$ first \commit message
            \State $\lr{id,\commit,e,v',\sigma'}\gets$ second \commit message
            \State \textbf{output} $\sigma \cap \sigma'$\label{alg:pbft-28}
        \EndIf
    \EndUpon
  %  \Upon{$\lr{id,\proofwithin, e, qc, qc'}$} 
   % \algorithmiccomment{\textgreen{sent by anyone}} % \kartik{doesn't matter who sends it, }
    %    \State \textbf{output} $qc \cap qc'$
  %  \EndUpon
    
\EndAs{}
\end{algorithmic}
\caption{Forensic protocol for PBFT Byzantine agreement: instance identifier~$id$}
\label{alg:fa-pbft1}
\end{algorithm}

\myparagraph{Forensic protocol.}
% The example in Figure~\ref{fig:pbft-disagree} is just one example of a sequence of events. 
Algorithm~\ref{alg:fa-pbft1} describes the entire protocol to obtain forensic support atop PBFT. For completeness, we also provide a complete description of the PBFT protocol in Algorithm~\ref{alg:single-pbft}. Each replica maintains a \emph{ledger} containing the value proposed and the status certificate $M$ obtained in the \nv message of view $e$. %If a replica observes locks for two conflicting values from the same view $e^*$ in status certificate $M$ (lines~\ref{alg1-9-twoM}), then the replicas can immediately flag this as a culpability proof to an external client. The culpability proof consists of the two conflicting locks from the same view. Since each lock consists of $2t+1$ signatures, at least $t+1$ replicas must have signed for conflicting values in the same view.
If a client observes commits for two conflicting values, then it first checks if the two values are committed in the same view (line~\ref{alg:pbft-18}). If yes, then any two \qcthree for the two different committed values can provide culpability proof for at least $t+1$ replicas (lines~\ref{alg:pbft-25}-\ref{alg:pbft-28}). Otherwise, the client picks the value that was committed in a lower view and sends $\signed{\conflictacross, e, v, \sigma}$ to all replicas to request a proof of culpability from witnesses (lines~\ref{alg:pbft-21}). Each replica looks through its ledgers for views $> e$. If there exists a ledger of the smallest view $e^* > e$ such that the status certificate $M$ contains the highest lock for a conflicting value $v''$, it sends $\ledger[e^*]$ to the client (lines~\ref{alg:pbft-10}-\ref{alg:pbft-13}). If inside $M$ there are conflicting locks in the same view, the intersection of them proves at least $t+1$ culprits (line~\ref{alg:pbft-20-withinM}), otherwise the intersection of $M$ and the \qcthree proves at least $t+1$ culprits (line~\ref{alg:pbft-23}).

\ignore{
Suppose replicas $i$ and $j$ commit to conflicting values $v$ and $v'$. Suppose replica $i$ commits first in view $e$ and replica $j$ commits in a later view $e'$. In PBFT, replica $i's$ commit must be guarded by $2t+1$ replicas who hold locks on $v$. When the number of faults are few $(f \leq t)$, the honest replicas among them ensure that no other value is proposed in a subsequent view. In our case, $f = t+1$ and this does not hold anymore. Suppose $2t+1$ replicas include the Byzantine red set and the honest blue set; thus at the end of view $e$, the highest lock that these replicas hold is for $(v, e)$. Honest replicas in the green set may have a lower lock (say $(v', e'')$) at the end of view $e$. 

What about replica $j$? We know that $j$ commits a conflicting value $v'$ in some higher view $e'$. Such a commit implies that there are $2t+1$ replicas (at least $t$ honest replicas) are locked on a different value $v'$ in view $e'$, and more importantly a higher lock for a conflicting value $v'$ is formed. Between views $e$ and $e'$, there may exist many such views where a lock for a value other than $v$ is formed. This may not necessarily be view $e+1$. In order to find culpable replicas, let us consider the first such view $e^*$ and the \nv message (proposal) sent in this view. Recall that the honest blue replicas and the Byzantine red replicas were responsible for guarding the safety of $i$'s commit. However, in our example, the leader of view $e^*$ receives locks from the Byzantine red replicas and the honest green replicas. In this case, the Byzantine replicas incorrectly send a lower lock and the honest green replicas may only have access to a lower lock. With this a (possibly honest) leader in view $e^*$


\myparagraph{How to disagree.} The safety of PBFT is guaranteed by $f<t$, when $f>t$, the adversary can violate the uniqueness within the view. It splits the honest replicas into two part, send \qctwo for one value to the first replica and send \qctwo for another value to the second replica. Each replica will vote for their values and then commit on corresponding values. Such attack is easy to detect by comparing the information within the view. Another potential attack is to construct a higher lock after some honest replica's committing. For example in Fig. \ref{fig:pbft-disagree}, an honest replica $i$ commits in view $e$ on value $v$. At the end of view $e$, $f$ honest replicas (blue replicas) are locked on $(v,e)$ while another $f$ honest replicas (red replicas) are locked on an older lock $(v',e''), e''<e$. In some view $e^*$ after $e$, a Byzantine replica can collect locks from $f$ red replicas, generate a \nv message proposing $v'$ and broadcast it to red replicas. Since the highest lock in \nv is for value $v'$, red replicas are happy to vote for it, a higher lock of $v'$ will be formed. This lock can either be used to make some red replica commit in this view, or change the lock of blue replicas later. A second commit can happen anytime afterwards.
}


\subsection{Proof for Forensic Support}

The following theorem shows that so far as up to $f \leq 2t$ replicas are Byzantine and safety violation occurs, Algorithm~\ref{alg:fa-pbft1} can be used to irrefutably detect $t+1$ Byzantine replicas. The proof indicates the Byzantine action performed by a detected Byzantine replica. Moreover, $2t+1-f$ honest witnesses have access to such a proof.

\ignore{
A disagreement in PBFT may happen when one replica $i$ is first committed on a value $v$ locally, then another replica $j$ commits a distinct value $v'$ afterwards. It is possible since no matter the second replica is locked on $v$ or not when $i$ commits, Byzantine replicas can generate a higher lock by equivocating to control the lock of $j$. We first prove that if disagreement happens, PBFT has forensic support to detect equivocating behaviors.}

\kartikold{note for myself: possibly change all notations}
%\kartik{mention need for aggregate signatures and not threshold}
\begin{theorem}
\label{thm:pbft}
For $n=3t+1$, if two honest replicas commit to conflicting values, PBFT provides $(2t,\ 2t+1-f,\ t+1)$-forensic support as per Definition~\ref{defn:forensic-support}.
\end{theorem}
\begin{proof}
Suppose values $v$ and $v'$ are committed in views $e$ and $e'$ respectively. 

\myparagraph{Case $e=e'$.} 

\noindent\underline{Culpability.} The quorums \qcthree  for $v$ and \qcthree  for $v'$ intersect in $t+1$ replicas. These $t+1$ replicas should be Byzantine since the protocol requires a replica to vote for at most one value in a view. 

% \kartik{who knows it? check} \peiyao{Do these replicas receive \qctwo for another value from clients?}

\noindent\underline{Witnesses.} Client can get the proof based on the two \commit messages, so additional witnesses are not necessary in this case.%For each of $v$ and $v'$, since $2t+1$ replicas have sent a commit message, both values' $\qctwo$ are available to some $2t+1-f$ honest replicas.

\ignore{
If $e\ne e'$, w.l.o.g, we assume $e < e'$. That $v$ is committed in $e$ indicates $2t+1$ replicas have lock $(v, e)$ at the end of view $v$. Now consider the first view $e < e^* \le e'$ in which a higher lock $(v', e^*)$ forms. Such view must exist since $v'$ is committed in $e'$. Since this is the first view $e^*>e$ where a lock for $v'$ forms, the highest lock in \nv message sent by the leader in this view must have view $e'' \le e$, which means the highest lock is $(v', e''), e''\le e$. Thus, the intersection of $2t+1$ locks in the \nv of $e^*$ and $2t+1$ commit messages in view $e$ contains at least $t+1$ equivocating replicas.

Since a higher lock $(v', e^*)$ forms, at least $2t+1$ replicas receive the \nv message and vote in this view, among them at least $2t+1-f$ are honest, thus all these replicas can get the above evidence for equivocating replicas.

---------
}
\myparagraph{Case $e\neq e'$.}

\noindent\underline{Culpability.}
If $e \neq e'$, then WLOG, suppose $e < e'$. Since $v$ is committed in view $e$, it must be the case that $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$. Now consider the first view $e < e^* \leq e'$ in which a higher lock $(v'', e^*)$ is formed (not necessarily known to any honest party) where $v'' \neq v$ (possibly $v'' = v'$). Such a view must exist since $v'$ is committed in view $e' > e$ and a lock will be formed in at least view $e'$. Consider the status certificate $M$ sent by the leader of view $e^*$ in its \nv message. $M$ must contain $2t+1$ locks; each of these locks must be from view $e'' \le e$, and a highest lock among them is $(v'', e'')$. % Otherwise, \kartik{explain not first} 

We consider two cases based on whether the status message contains a lock $(v''', e)$ for a value $v''' \neq v''$. The two cases are (i) there does not exist a such a lock $(v''', e)$, and (ii) there exists such a lock $(v''', e)$. %\peiyao{Shall these $e$ in this paragraph be $e''$?}

\ignore{if $e'' = e$ then $v'$ is the only highest lock, if $e'' < e$, there could be more such high locks.}
For the first case, the status certificate $M$ with $2t+1$ locks intersect with the $2t+1$ signers of \qcthree  in view $e$ at $t+1$ Byzantine replicas. These replicas are Byzantine because they had a lock in view $e$ that was different from, and at least as high as the one sent to the leader of view $e^* > e$.

For the second case, since $v''$ is proposed in view $e^*$, it exists in the status certificate $M$ and is a highest lock in $M$. Moreover, in this case, $(v''', e)$ exists in $M$ too. Both of these locks were formed in view $e$. The two quorums forming the two locks in view $e$ intersect in $t+1$ replicas. These replicas are Byzantine since they voted for more than one value in view $e$.%\gerui{I think the protocol (Alg 1) doesn't capture this case. I think we need to add some actions after line 22.}

\noindent\underline{Witnesses.} Since a higher lock $(v'', e^*)$ is formed in view $e^*$, at least $2t+1$ replicas have voted for $v''$ in view $e^*$. These replicas must have received the \nv message and at most $f$ among them are Byzantine. Thus, all of these $2t+1-f$ replicas are witnesses who have access to the status certificate $M$.
\end{proof}

%\kartik{start from here -- do not read these paragraphs.}
%The proof of Theorem \ref{thm:pbft} indicates that if two values are committed in two different views, there must exist honest replicas who will receive equivocating messages between two views. The first scheme is to broadcast messages internally. We make these changes to the PBFT protocol,
%\begin{enumerate}
%    \item Upon receiving a \commit message, save and echo the message.
%    \item Upon receiving a \nv message, save the status collection.
%    \item For each status collection received from view $e$, pick the highest lock $(v^*, e^*)$, check all \commit messages committing on $(v', e')$ before $e$, if $e^* < e'$ and $v^* \ne v'$, broadcast the \vc message and status collection.
%\end{enumerate}
%The second scheme is executed by external clients. With PBFT protocol unchanged, if an client receives two conflicting \commit messages, it broadcasts them and wait for responses. Then honest replicas will check all status collections and at least one honest replica will get the evidence and send it back to the client.


% \kartik{need to change locks to explicitly have signatures?}







==> old/old_4_hotstuff.tex <==
\section{HotStuff has Strong Forensic Support}
\label{sec:basic-hotstuff}
HotStuff~\cite{yin2019hotstuff} is a partially synchronous consensus protocol that provides optimal resiliency of $t<n/3$. The HotStuff protocol is similar to PBFT but there are subtle differences which allow it to obtain a linear communication complexity for both its steady state and view change protocols (assuming the presence of threshold signatures). Looking ahead, these differences significantly change the way forensics is conducted if a safety violation happens.

\subsection{Overview}  We start with an overview of the protocol. For simplicity, we discuss a single-shot version of HotStuff. The protocol proceeds in a sequence of consecutive views where each view has a unique leader. Each view of HotStuff progresses as follows:
% \kartik{witness definition}
\begin{itemize}[leftmargin=*, topsep=0pt]
    \item[-] \textbf{Propose.} The leader proposes a \nv message containing a proposal $v$ along with the highest \qctwo known to it and sends it to all replicas.
    \item[-] \textbf{\vone.} On receiving a \nv message containing a valid value $v$ in a view $e$ and a \qctwo message, a replica sends \vone for $v$ if it is \emph{safe} to vote based on a locking mechanism (explained later). It sends this vote to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qctwo in view $e$. The leader sends the view $e$ \qctwo to all replicas.
    \item[-] \textbf{\vtwo.} On receiving a \qctwo in view $e$ containing message $v$, a replica updates its highest \qctwo to $(v, e)$ and sends \vtwo to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qcprecom.
    \item[-] \textbf{\vthree.} On receiving \qcprecom in view $e$ containing message $v$ from the leader, a replica locks on $(v, e)$ and sends \vthree to the leader. The leader collects $2t+1$ such votes to form an aggregate signature \qcthree.
    \item[-] \textbf{\commit.} On receiving \qcthree from the leader, replicas commit to the value $v$.
\end{itemize}

Once a replica locks on a given value $v$, it only votes for the value $v$ in subsequent views. The only scenario in which it votes for a value $v' \neq v$ is when it observes a \qctwo from a higher view in a \nv message. At the end of a view, every replica sends its highest \qctwo to the leader of the next view. The next view leader collects $2t+1$ such values and picks the highest \qctwo.

The safety and liveness of HotStuff when $f \leq t$ follows from the following:

\myparagraph{Uniqueness within a view.} Since replicas only vote once in each round, a \qcthree can be formed for only one value when $f \leq t$.

\myparagraph{Safety and liveness across views.} Safety across views is ensured by the use of locks and the voting rule for a \nv message. Whenever a replica commits a value, at least $2t+1$ other replicas are locked on the value in the view. Observe that compared to PBFT, there is no status certificate $M$ in the \nv message to ``unlock'' a replica. Thus, a replica only votes for the value it is locked on. The only scenario in which it votes for a conflicting value $v'$ is if the leader includes a \qctwo for $v'$ from a higher view in \nv message. This indicates that at least $2t+1$ replicas are not locked on $v$ in a higher view, and hence it should be safe to vote for it. The latter constraint of voting for $v'$ is not necessary for safety, but only for liveness of the protocol.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\columnwidth]{figures/hotstuff-diff.pdf}
    \caption{\textbf{Depiction of events in the HotStuff protocol for the first two views where a higher \qctwo for $v'$ is formed.}} %\kartik{In this example, why should $e^*$ be the view of interest. It can be that $e^\#$ was the view where first prepareQC containing culpable act was formed, and in a higher view $e^{\#\#}< e^*$, a new view message with prepareQC from $e^\#$ was sent. Shouldn't receivers of the NewView message of $e^{\#\#}$ contain the witnesses and not $e^*$?}} %  Replicas in the red ellipse contain culpable Byzantine replicas. Replicas in the blue ellipse and (honest) replicas in the red ellipse have access to $\qctwo$ and the \nv message respectively.}
    \label{fig:hotstuff-diff}
\end{figure}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/hotstuff-equal.pdf}
    \caption{\textbf{Depiction of events in the HotStuff protocol for the first view where a higher \qctwo and lock are formed in the same view.}} %  Replicas in the red ellipse contain culpable Byzantine replicas. Replicas in the blue ellipse and (honest) replicas in the red ellipse have access to $\qctwo$ and the \nv message respectively.}
    \label{fig:hotstuff-equal}
\end{figure}

\subsection{Forensic Support for HotStuff}

Similar to PBFT, our forensic protocol on HotStuff can detect $t+1$ Byzantine replicas when the number of Byzantine faults is $f \leq 2t$. We make a simple modification to the message structure in HotStuff~\cite[Algorithm~2]{yin2019hotstuff} which ensures that there are at least $2t+1-f$ witnesses can individually prove the culpability.

\myparagraph{Intuition.} If two conflicting values are committed in the same view, Byzantine replicas can be detected using \qcthree  and using ideas similar to that in PBFT. However, when the conflicting commits of replicas $i$ and $j$ are across views $e$ and $e'$ for $e < e'$, the same ideas do not hold anymore. To understand this, observe that the two key ingredients for proving the culpability of Byzantine replicas in PBFT were (i) a \qcthree  for the value committed in a lower view (denoted by $\sigma$ for replica $i$'s commit in Figure~\ref{fig:pbft-disagree}) and (ii) a status certificate from the first view higher than $e$ containing the locks from $2t+1$ replicas (denoted by $M$ for view $e^* > e$ in Figure~\ref{fig:pbft-disagree}). In HotStuff, a \qcthree still exists. However, for communication efficiency reasons, HotStuff does not include a status certificate $M$ in its \nv message. The status certificate in PBFT provides us with the following:

\begin{itemize}[leftmargin=*, topsep=0pt]
    \item \textbf{Identifying a potential set of culpable replicas.} Depending on the contents of $M$ and knowing $\sigma$, we could identify a set of Byzantine replicas.
    \item \textbf{Determining whether the view is the first view where a higher lock for a conflicting value is formed.} By inspecting all the locks in $M$, we can easily determine this. Ensuring first view with a higher lock is important; once a higher lock is formed, even honest replicas may update their locks and the proof of Byzantine behavior may not exist in the messages in subsequent views.
\end{itemize}

Unfortunately, with HotStuff, the leader does not broadcast $M$. Our goal is to find witnesses who have access to the information contained in $M$ (as described in the bullets above). %this information. 


Let us try to understand this based on the first view $e^\#$ where a higher \qctwo is formed for $v'\ne v$. If the first higher lock for $v'$ is also formed in $e^* = e^\#$ (see Figure~\ref{fig:hotstuff-equal}), then $2t+1$ replicas (denoted by the blue ellipse) have access to \qctwo for a conflicting value in view $e^\#$. Otherwise, consider the second \qctwo which is formed in $e^{\#\#}$ where $e^\#<e^{\#\#}\le e^*$ (see Figure~\ref{fig:hotstuff-diff}), $2t+1$ replicas in blue ellipse who receive the \nv message have access to \qctwo formed in $e^\#$. The set of replicas who sent \vone (the red ellipse) in $e^\#$ and formed this \qctwo are our potential set of Byzantine replicas. Why? If $e^\#$ is indeed the first view in which a higher \qctwo is formed, then all of these replicas voted for a \nv message containing a \qctwo from a lower or equal view $e''$ on a different value. If any of these replicas also held a lock $(v, e)$ (by voting for replica $i$'s commit) then these replicas have committed the culpable act of not respecting the voting rule. Thus, the blue set of replicas are witnesses who help determine a red set of potentially culpable replicas.

\ignore{
Let us try to understand this based on the first view $e^*$ where a higher lock is formed and the first view $e^\#$ where the corresponding \qctwo is formed. For intuition, a graphical representation is depicted in Figure~\ref{fig:hotstuff-case} for the case where $e^\# < e^*$. The special case when $e^\# = e^*$ is depicted in Figure~\ref{fig:hotstuff-case2}.\kartik{figure numbers are in reverse? perhaps we should keep just the generic figure?} Formation of a higher lock implies that $2t+1$ replicas (denoted by the blue ellipse) have access to \qctwo for a conflicting value in view $e^*$, which is either contained in \nv message when $e^\# < e^*$ or contained in \prepare message when $e^\# = e^*$.\kartik{check my comment in figure 2. is $e^*$ where a lock is formed the view of interest here?} The set of replicas who sent \vone (the red ellipse) in $e^\#$ and formed this \qctwo are our potential set of Byzantine replicas. Why? If $e^\#$ is indeed the first view in which a higher \qctwo is formed, then all of these replicas voted for a \nv message containing a \qctwo from a lower or equal view $e''$. If any of these replicas also held a lock $(v, e)$ (by voting for replica $i$'s commit) then these replicas have committed the culpable act of not respecting the voting rule. Thus, the blue set of replicas are witnesses who help determine a red set of potentially culpable replicas.
}
\ignore{
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{false-alarm.pdf}
    \caption{\textbf{Byzantine leader can create fake \nv message to accuse honest replicas.}} %  Replicas in the red ellipse contain culpable Byzantine replicas. Replicas in the blue ellipse and (honest) replicas in the red ellipse have access to $\qctwo$ and the \nv message respectively.}
    \label{fig:hotstuff-false}
\end{figure}
}

The only remaining part is to ensure that this is indeed the first view where a higher conflicting \qctwo is formed. To detect this, we include the view number where \qctwo was formed in \vone messages (in the $\eqc$ field). %\peiyao{To detect this, we include $\eqc$, the view number of \qctwo in \nv message, whenever replicas send \vone.} 
When the leader collects enough \vone messages, the new \qctwo contains $\eqc$ too. This explicitly states the message they vote for and provides the necessary link to show culpable behavior.

\ignore{
\noindent {\bf Importance of this minor modification to Hotstuff}. \peiyao{If the extra information $\eqc$ is not included, the client can not determine whether received \qctwo is indeed formed in the first view, except it receives the \nv message in the same view. If the client asks replicas for the \nv message, Byzantine replicas can send a fake \nv message to the client to implicate honest replicas. An example is depicted in Figure~\ref{fig:hotstuff-false}: consider the first view $e^\#$ where a higher \qctwo for $v'$ is formed and the first view $e^*$ where a higher lock for $v'$ is formed. The Byzantine leader in view $e^*>e^\#$ sends a \nv message containing the \qctwo formed in $e^\#>e$ to replicas, since there is no lock higher than $e$ formed yet, $2t+1$ honest replicas will send \vone then a new \qctwo for $v'$ is formed. Since $v'\ne v$, this \qctwo should be sent to the client -- at this time, the Byzantine leader creates a fake \nv message containing the \qctwo formed in $e''\le e$ to the client to pretend that $e^*$ is the first view where a higher \qctwo is formed. If the client is convinced that $2t+1$ honest replicas vote for the fake \nv message, honest replicas who also vote for the first \commit message will be implicated as culprits.}
}


Thus, to summarize, the red set of replicas in view $e^\#$ are a potential set of culpable nodes of size $2t+1$. The blue set acts as witnesses and a client needs a proof of culpability from the blue set. Since there are $f$ actual faults, the number of honest replicas with such a proof is $2t+1-f$. 

\myparagraph{Comparison to the two HotStuff protocols.} We note that adding $\eqc$ in the vote is a modification to the basic HotStuff protocol described in \cite[Algorithm~2]{yin2019hotstuff}. The modification is only relevant to the forensic capability. Interestingly, the chained version of their protocol~\cite[Algorithm~3]{yin2019hotstuff} does include similar information, enabling forensics directly.

\begin{algorithm}[htbp]
\begin{algorithmic}[1]
\As{a replica running HotStuff}
\LeftComment{patch for HotStuff}
    \ForInitialize{$e\ge 1$}
        % \State $ledger[e]\gets \{\}$
        \State $\pflock[e]\gets \{\}$
        \EndForInitialize
    \Upon{$\lr{id,\nv,e,v,L}$ from the leader of view $e$}
        \State $(e', v', \sigma, \eqc)\gets L $\Comment{Note that $L$ has selectors $e,v,\sigma,\eqc$\ignore{ $= (e, v, \sigma, \eqc)$}} 
        \State $\pflock[e'] \gets  \pflock[e']\cup \{(v', \sigma, \eqc)\}$\label{alg:hotstuff-6}
    \EndUpon
    \Upon{$\lr{id,\prepare,e,v,\sigma,\eqc}$ from the leader of view $e$}
        \State $\pflock[e]\gets \pflock[e]\cup \{(v, \sigma,\eqc)\}$\label{alg:hotstuff-6-2}
    \EndUpon
    \Upon{$\lr{id,\conflictacross, e, v, \sigma, e'}$ from a client}
        \For{all $e<e^\#\le e'$}
            % \If{$(\ledger[e^*]\ne \{\})\land(\ledger[e^*].L.e\le e)\land(\ledger[e^*].v\neq v)$}
            %     \State send $\lr{id,NV, e^*, \ledger[e^*]}$ to the client\label{alg:hotstuff-12}
            % \EndIf
            \For{$qc\in \pflock[e^\#]$} % \kartik{what is this iterating over? $pflock$ is a list of votes?}\gerui{a malicious leader could send multiple prepareQC in a view, hence it is a list of prepareQC}
            \If{$(qc.v\neq v)\land (qc.\eqc\le e)$} % \kartik{check $\eqc = e$ case, is the proof the same?}
                \State send $\lr{id,\proofacross, e^\#, qc}$ to the client\label{alg:hotstuff-12} %\kartik{$\textsc{QC}$ is undefined.}\gerui{changed to \proofacross}
            \EndIf
            \EndFor
        \EndFor
    \EndUpon
    % \Upon{$\lr{id,\conflictwithin, e, v, v'}$ from a client}
    %     \If{$\pflock[e]\ne \{\}$}
    %         \State send $\lr{id,\proofacross, e, \pflock[e]}$ to the client\label{alg:hotstuff-17}
    %     \EndIf
    % \EndUpon
\EndAs{}

\As{a client}
    \Upon{two conflicting \commit messages}
        \If{the two \commit messages are from different views}\label{alg1:28}
            \State $\lr{id,\commit,e,v,\sigma}\gets$ the message from lower view
            \State $e'\gets$ the view number of message from higher view
            \State broadcast $\lr{id,\conflictacross, e, v, \sigma, e'}$ \label{alg:hotstuff-23}
            \State wait for  $\lr{id,\proofacross, e^\#, qc}$ s.t.
            \begin{enumerate}[leftmargin=1in]
                \item[(1)] $e<e^\#\le e'$, and\label{alg:hotstuff-24}
                \item[(2)] $(qc.v\neq v)\land (qc.\eqc\le e)$
                %\item[(3)] check signature, (do we need to mention it?) %
            \end{enumerate}%\gerui{wait for a matching pair of $\lr{id,NV, e^*, m},\lr{id,\proofacross, e^*, qc}$ s.t. 1) $e<e^*\le e'$ 2) $m.H.e \le e\wedge\ m.v\neq v$ and 3) the hash of $m.H$ matches that in $qc$}
            \State \textbf{output} $qc.\sigma \cap \sigma$\label{alg:hotstuff-26}
\label{alg:hotstuff-25}
        \Else \label{alg:hotstuff-28}
            \State $\lr{id,\commit,e,v,\sigma}\gets$ first \commit message
            \State $\lr{id,\commit,e,v',\sigma'}\gets$ second \commit message
            \State \textbf{output} $\sigma \cap \sigma'$
            % \State $v, v',e\gets$ two committed values and the view number
            % \State broadcast $\lr{id,\conflictwithin, e, v, v'}$\label{alg:hotstuff-28}
            % \State wait for: $qc, qc'\gets$ two \qctwo of committed values from possibly different replicas in view $e$.\label{alg:hotstuff-29}
            % \State \textbf{output} $qc.\sigma \cap qc'.\sigma$
        \EndIf
    \EndUpon
\EndAs{}
\end{algorithmic}
\caption{Forensic protocol for Basic HotStuff}
\label{alg:fa-hotstuff-modified}
\end{algorithm}


\myparagraph{Forensic protocol.}
% The example in Figure~\ref{fig:pbft-disagree} is just one example of a sequence of events. 
Algorithm~\ref{alg:fa-hotstuff-modified} describes the entire protocol to obtain forensic support atop HotStuff. A complete description of the HotStuff protocol is also provided in Algorithm~\ref{alg:single-hotstuff-modified}. Each replica maintains a list of \pflock containing all received \qctwo from \prepare messages and \nv messages (line~\ref{alg:hotstuff-6},\ref{alg:hotstuff-6-2}). %\kartik{this line is confusing}\gerui{use PlaceHolder, is it good now? we can change latex command to change its name}
If a client observes commits for two conflicting values in the same view, it can determine the culprits by two \commit messages (line~\ref{alg:hotstuff-28}).  Otherwise, the client sends a request to all replicas for possible proof between two committed views $e, e'$ for $e<e'$ (line~\ref{alg:hotstuff-23}). Each replica looks through its list for views $e<e^\#\le e'$. If there exists a \qctwo whose value is different from the value $v$ committed in $e$ and recorded $\eqc$ is less than or equal to $e$, it sends a reply with this \qctwo to the client (line~\ref{alg:hotstuff-12}). The client waits for a \qctwo (line~\ref{alg:hotstuff-24}) from $e^\#$ between two committed views. If it contains a different value from the first committed value and an older view number $\eqc < e$, the intersection of this \qctwo and the \qcthree from the commit message in the lower view proves at least $t+1$ culprits (line~\ref{alg:hotstuff-26}).

\subsection{Proof for Forensic Support}

The following theorem provides the necessary culpability proof for HotStuff.

\begin{theorem}
\label{thm:hotstuff}
For $n=3t+1$, if two honest replicas commit to conflicting values, HotStuff provides $(2t,\ 2t+1-f,\ t+1)$-forensic support as per Definition~\ref{defn:forensic-support}.
\end{theorem}
\begin{proof}
Suppose two conflicting values $v,\ v'$ are committed in views $e$, $e'$ respectively. 

\myparagraph{Case $e=e'$.}

\noindent\underline{Culpability.} The \qcthree of $v$ and \qcthree of $v'$ intersect in $t+1$ replicas. These $t+1$ replicas should be Byzantine since the protocol requires a replica to vote for at most one value in a view. 

\noindent\underline{Witnesses.} Client can get the proof by itself when receiving two \commit messages, so witnesses are not necessary in this case. %For each of $v$ and $v'$, since $2t+1$ replicas have sent a \vtwo message, both values' $\qctwo$ are available to some $2t+1-f$ honest replicas.

\myparagraph{Case $e\neq e'$.}

\noindent\underline{Culpability.}
If $e \neq e'$, then WLOG, suppose $e < e'$. Since $v$ is committed in view $e$, it must be the case that $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$. Now consider the first view $e < e^* \leq e'$ in which a higher lock $(v'', e^*)$ is formed where $v''\ne v$ (possibly $v''=v'$). Such a view must exist since $v'$ is committed in view $e' > e$ and a lock will be formed in at least % \gerui{at latest? I think at least means $\ge$ but we actually mean $\le$. Section 3 also has this word.} 
view $e'$. For a lock to be formed, a higher \qctwo must be formed too. Consider the first view $e<e^\# \leq e'$ in which the corresponding \qctwo for $v''$ is formed. The leader in $e^\#$ broadcasts the \nv message containing a \qctwo on $(v'', e'')$ (the highest QC collected from other replicas). Since this is the first time a higher \qctwo is formed and there is no higher \qctwo for $v''$ formed between view $e$ and $e^\#$, we have $e''\le e$. The formation of the higher \qctwo indicates that $2t+1$ replicas received the \nv message proposing $v''$ with \qctwo on $(v'', e'')$ and consider it a valid proposal, i.e., the view number $e''$ is larger than their locks because the value is different. 

\ignore{A lock for $v''$ is formed in $e^*$ only under two cases: 1) If $e^\# = e^*$, the leader collects $2t+1$ \vtwo messages which form a \qcprecom, so that $2t+1$ replicas receive \qctwo; 2) If $e^\# < e^*$, consider the second view  $e^{\#\#}$ where a \qctwo for $v''$ \kartik{a value $\neq v$ is formed?} is formed, $2t+1$ replicas receive \qctwo contained in the \nv message in $e^{\#\#}$ (and send \vone). In both cases $2t+1$ replicas receive the \qctwo, which contains $2t+1$ \vone messages including $\eqc = e''$, indicating that $2t+1$ replicas received the \nv message proposing $v''$ with \qctwo on $(v'', e'')$ and consider it a valid proposal, i.e., the view number $e''$ is larger than their locks because the value is different. \gerui{I think this para belongs to witnesses.}}

 Recall that the committed value $v$ indicates $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$. In this case, the $2t+1$ votes in \qctwo in view $e^\#$ intersect with the $2t+1$ votes in \qcthree in view $e$ at $t+1$ Byzantine replicas. These replicas should be Byzantine because they were locked on value $v$ in view $e$ and vote for a value $v'' \neq v$ in a higher view $e^\#$ when the \nv message contained a \qctwo from a  view $e'' \leq e$. Thus, they have violated the voting rule.
\ignore{If $e \neq e'$, then WLOG, suppose $e < e'$. Since $v$ is committed in view $e$, it must be the case that $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$. Now consider the first view $e < e^* \leq e'$ in which a higher lock $(v'', e^*)$ is formed where $v''\ne v$ (possibly $v''=v'$) and the first view $e < e^\# \leq e'$ in which the corresponding \qctwo for $v''$ is formed. Such views must exist since $v'$ is committed in view $e' > e$ and a lock will be formed in at least view $e'$. Consider the \qctwo on $(v'', e'')$ sent by the leader of view $e^\#$ in its \nv message. Since there is no lock formed between view $e$ and $e^*$ (other than lock on $v$), we have $e''\le e$.

A lock for $v''$ is formed in $e^*$ only under two cases: 1) If $e^\# = e^*$, the leader collects $2t+1$ \vtwo messages which form a \qcprecom, so that $2t+1$ replicas receive \qctwo; 2) If $e^\# < e^*$, $2t+1$ replicas receive \qctwo contained in \nv message in $e^*$ and after two-round voting a lock is formed. In both cases $2t+1$ replicas receive the \qctwo, which contains $2t+1$ \vone messages including the view number $\eqc = e''$ in \nv message, indicating that $2t+1$ replicas received the \nv message proposing $v''$ with \qctwo on $(v'', e'')$ and considered it a valid proposal, i.e., the view number $e''$ is larger than their locks because the value is different. \kartik{However, this is not true since $e'' < e$ and $2t+1$ replicas are locked on $v$ at the end of view $e$.}

Recall that the committed value $v$ indicates $2t+1$ replicas are locked on $(v, e)$ at the end of view $e$. In this case, the $2t+1$ votes in \qctwo in view $e^\#$ intersect with the $2t+1$ votes in \qcthree in view $e$ at $t+1$ Byzantine replicas. These replicas should be Byzantine because they were locked on value $v$ in view $e$ and vote for a value $v'' \neq v$ in a higher view $e^\#$ when the \nv message contained a \qctwo from a  view $e'' \leq e$. Thus, they have violated the voting rule.}


\noindent\underline{Witnesses.} Since a higher lock $(v'', e^*)$ is formed in view $e^*$, there are two possible cases: 1) If $e^\# = e^*$, the leader collects $2t+1$ \vtwo messages which form a \qcprecom, so that $2t+1$ replicas receive \qctwo; 2) If $e^\# < e^*$, consider the second view $e^{\#\#}$ (possibly $= e^*$) where a \qctwo for $v''$ is formed, $2t+1$ replicas receive the \nv message (containing the \qctwo formed in $e^\#$). In both cases $2t+1$ replicas receive the \qctwo, at most $f$ among which are Byzantine. Thus, all of these $2t+1-f$ replicas are witnesses who have access to the required proof.
\end{proof} 




==> old/old_7_Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
In this paper, we have embarked on a systematic study of the forensic properties of BFT protocols and demonstrated strong forensics properties for a few popular protocols. In this section, we discuss the implications, extensions and possible future research following up on our results. 

\myparagraph{Chained consensus.} In this paper, we have focused on Validated Byzantine Agreement, a core consensus formalism for {\em single-shot} consensus in a state machine replication (SMR) system. SMR protocols (blockchains) extend this to serve consensus for a sequence of values. For instance, in protocols such as chained HotStuff (\cite[Algorithm~3]{yin2019hotstuff}) adopted by Libra, SBFT~\cite{gueta2019sbft} adopted by Concord, and Streamlet~\cite{chan2020streamlet}, the consensus protocol decides on a sequence of decision values. The sequence of values can either be treated independently (like in SBFT) or chained by hash pointers (like in chained HotStuff). When treated independently, it may be essential for replicas to exchange and maintain additional metadata information (e.g., $e_{qc}$ in HotStuff). Chained protocols, on the other hand, may maintain this metadata in the chain itself. In fact, the availability of this information on the chain may be a requirement for a replica to make progress. This strong availability requirement may enable a stronger forensic support, where we just require a replica to provide (part of) the chain and metadata rather than a specific witness to provide a specific evidence. For instance, in chained HotStuff, we would have the crucial \qctwo of view $e^{\#}$ on the chain itself. Thus a client can query (even Byzantine) replicas for the chain between $e$ and $e'$ and find the desired \qctwo somewhere on the chain. This may make it easier to identify culprits on the chain. Generally speaking, if a protocol has forensic support and all supporting evidence (e.g., quorum certificates) are put on chain, then a client can query the chain from replicas and identify culprits exclusively on the chain.

\myparagraph{Implementation details matter.} A second observation is that minor details matter when it comes to BFT protocol forensics. Consider three different versions of the HotStuff protocol: (i) The one described in Algorithm~\ref{alg:single-hotstuff-modified}, (ii) The one described in \cite[Algorithm~2]{yin2019hotstuff}, and (iii) the one in Algorithm~\ref{alg:single-hotstuff-modified} without sending $e_{qc}$ along with votes. While all three variants embody the key contribution of HotStuff to make the protocol achieve linear communication (assuming threshold signatures), all three of them have different forensic capabilities. We have shown that the variant described in Algorithm~\ref{alg:single-hotstuff-modified} has strong forensic capability. The variant from \cite[Algorithm~2]{yin2019hotstuff} has forensic capability but requires communicating to two types of witnesses, and there exist $2t+1-f$ witnesses of each type. Essentially, in addition to the witness in Algorithm~\ref{alg:single-hotstuff-modified}, we need  another witness holding information about $e_{qc}$ to determine the first time a \qctwo is formed in a higher view. Using the two witnesses, and the fact that the blocks are linked through hashes, culpable nodes can be determined. Finally, the variant from Algorithm~\ref{alg:single-hotstuff-modified} with $e_{qc}$ not being sent as a part of the votes has no forensic support. The lack of information about $e_{qc}$ with witnesses, and the absence of hash-links between blocks does not allow a client to determine \emph{whether a view was the first view} where a higher conflicting \qctwo was formed. 

%\kartik{Sreeram, do you want to take a stab at the $t > 2n/3$ setting?}

%\myparagraph{Future work.} A final consideration is on the generality of our results. Our work has focused on three protocols, two of which are in the partially synchronous setting and one in the asynchronous setting. In all cases, we observed that, ignoring simple modifications, all these protocols have strong forensic support. Based on these results, a natural question is: what are the requirements to make any protocol have strong forensic support? As an example, all of the protocols we considered used digital signatures. Whether we can achieve any guarantees for protocols relying only on authenticated channels is an open question. Moreover, all of our techniques were for protocols tolerating $< 1/3$ faults. Whether we can achieve forensic support for protocols tolerating a larger fraction (e.g., synchronous protocols) is still an open question. %\kartik{I am not sure if we should include this paragraph. Both of these are juicy open questions that we should work on straightaway!}

\ignore{
{\bf Para 1}. In this paper we have focused on Validated Byzantine Agreement, a core consensus formalism. In blockchain applications, this core protocol is adapted to serve consensus for a sequential setting. {\em Discuss chained VBA protocols via an example. Give the example of Hotstuff being used in Libra. Now ask how forensics changes in this context (even definition might change?) and point out some basic results (ideally blackbox -- if VBA has a certain forensic support then the chained version in a blockchain also has the following forensic support properties (this should be stated as a proposition). If this para becomes too long it should be a whole section in itself. Note that proofs can be moved to appendix. }
\gerui{In protocols such as Chained HotStuff (Algorithm~3~\cite{yin2019hotstuff}) and Streamlet~\cite{chan2020streamlet}, the consensus protocol decides on a sequence of decision values that are chained by hash pointers. Sometimes, metadata such as  quorum certificates are also put on chain, as in Chained HotStuff. Libra project adopts LibraBFT~\cite{}, a consensus protocol based on Chained HotStuff, as its core consensus protocol. Comparing simplistic single-shot Byzantine agreement to practical chained SMR protocols, a distinctive difference is that in chained SMR protocols, the entire chain and metadata, from genesis to up-to-date chain tip, have to be made available to a replica in order for it to make progress. This strong availability requirement enables a stronger forensics support, where we just require a replica to provide (part of) the chain and metadata rather than a specific witness to provide a specific evidence. Take the HotStuff case in Figure~\ref{fig:hotstuff-case} as an example: in Chained HotStuff we would have the crucial \qctwo of view $e^*$ on chain for $e<e^*\le e'$, thus a client can query (even Byzantine) replicas for the chain between $e$ and $e'$ and find that \qctwo somewhere on the chain. Generally speaking, if a protocol has forensic support and all quorum certificates are put on chain, then a client can query the chain from replicas and identify culprits exclusively on chain.}

{\bf Para 2}. Emphasize that we needed a minor change to Hotstuff. Its a trivial change, no difference in complexity but makes a crucial difference for forensic capability. (note: how come David's paper is claiming some forensics support for Hotstuff directly? Is their result wrong? Not worth pointing it out in paper, but good for us to know internally.) Ask if there is a way to bring this modification systematically to any BFT protocol to improve forensic support without changing complexity or security properties. {Kartik: any ideas here? I feel you might have something very smart to say here. } 

{\bf Para 3}. What happens when $t> 2f/3$? Note that in synchronous setting, one can securely design consensus against 99\% adversarial resistance. Compare with polygraph here. 


{\bf Para 4}. Forensic support of other VBA protocols. Point out that we covered different network conditions (partially synchronous, asynchronous) and classical/efficient protocols in both settings and find that (with minor implementation level modifications) they already have strong forensic support. Two questions are natural: (1)  whether all VBA protocols also have strong forensic support  (with potentially minor implementatino level modifications)? (2) how about VBA protocols that dont use digital signatures -- but instead rely on authenticated channels? (3) how about VBA protocols in synchronous setting where t is strictly smaller than 50\% (eg: 40\%)? (are there even examples of such protocols???). 
}

